Derivative-Free Policy Optimization for Linear Risk-Sensitive and Robust Control Design: Implicit Regularization and Sample Complexity

Direct policy search serves as one of the workhorses in modern reinforcement learning (RL), and its applications in continuous control tasks have recently attracted increasing attention. In this work, we investigate the convergence theory of policy gradient (PG) methods for learning the linear risk-sensitive and robust controller. In particular, we develop PG methods that can be implemented in a derivative-free fashion by sampling system trajectories, and establish both global convergence and sample complexity results in the solutions of two fundamental settings in risk-sensitive and robust control: the finite-horizon linear exponential quadratic Gaussian, and the finite-horizon linear-quadratic disturbance attenuation problems. As a by-product, our results also provide the first sample complexity for the global convergence of PG methods on solving zero-sum linear-quadratic dynamic games, a nonconvex-nonconcave minimax optimization problem that serves as a baseline setting in multi-agent reinforcement learning (MARL) with continuous spaces. One feature of our algorithms is that during the learning phase, a certain level of robustness/risk-sensitivity of the controller is preserved, which we termed as the implicit regularization property, and is an essential requirement in safety-critical control systems.

==> Mixed Design Arxiv v3/Introduction.tex <==
Recent years have witnessed the rapid development of reinforcement learning (RL) methods in handling continuous control tasks \cite{schulman2015high, lillicrap2015continuous, recht2019tour}. Central to the success of RL are policy optimization (PO) methods, including policy gradient (PG) \cite{sutton2000policy, kakade2002natural, zhang2019global}, actor-critic \cite{konda2000actor, bhatnagar2009natural}, and other variants \cite{schulman2017proximal, schulman2015trust}. Progress reported in the literature has clearly shown an increasing interest in understanding theoretical properties of PO methods for relatively simple baseline problems such as various linear control problems
\cite{fazel2018global, tu2019gap, bu2019LQR, zhang2019policy, zhang2019policymixed, mohammadi2019convergence, furieri2019learning, malik2020derivative, jansch2020convergence,fatkhullin2020optimizing}. However, the theory of model-free PO methods on \emph{risk-sensitive/robust} control remains underdeveloped in the literature.  Since risk-sensitivity and robustness are important issues for designing  safety-critical systems, it is natural to bring up the questions of whether and how model-free PO methods would converge for these continuous control tasks.

Our work in this paper is motivated by the above concern, and
studies the sample complexity of model-free PG methods on two important baseline problems in risk-sensitive/robust control, namely the linear exponential quadratic Gaussian (LEQG), and the linear quadratic (LQ) disturbance attenuation problems. The former covers a fundamental setting in risk-sensitive control, and the latter is an important baseline for robust control. Based on the well-known equivalence between these problems and LQ dynamic games \cite{jacobson1973optimal, glover1988state, basar1991dynamic, bacsar2008h, bacsar1998dynamic}, we develop a \emph{unified} PO perspective for both. 
A common feature for the above two problems is that their optimization landscapes are by nature more challenging than that of the linear quadratic regulator (LQR) problem, and existing proof techniques for model-free PG methods \cite{fazel2018global, mohammadi2019convergence, furieri2019learning, malik2020derivative} are no longer effective due to lack of coercivity of the objective functions. Specifically, when applying PG methods to LQR, the feasible set for the resultant constrained optimization problem  is the set of all linear state-feedback controllers that \emph{stabilize} the closed-loop dynamics. The objective function of LQR is coercive on this feasible set and serves as a barrier function itself \cite{bu2019LQR}, guaranteeing for the PG iterates to stay in the feasible set and converge to the globally optimal controller. For the LEQG and LQ disturbance attenuation problems, the risk-sensitivity/robustness conditions have reshaped the feasible set in a way that the objective function becomes non-coercive, i.e. the objective value can remain finite while approaching the boundary. The objective is no longer a barrier function, and new proof techniques are needed to show that model-free PG iterates will stay in the feasible set. This is significant for safety-critical control systems with model uncertainty, as the iterates' feasibility here is equivalent to \emph{risk-sensitivity/robustness} of the controller (cf. Remark \ref{remark:ir}), and the  failure to preserve robustness during learning can cause catastrophic effects, e.g., destabilizing the system in face of disturbances.

The most relevant result was developed in \cite{zhang2019policymixed}, which proposes implicit regularization (IR) arguments to show the convergence of several PG methods on the mixed $\cH_2/\cH_{\infty}$ control design problem (which can be viewed as the infinite-horizon variant of the LQ disturbance attenuation problem studied in this paper). The main finding there is that two specific PG search directions (with perfect model information)  are automatically biased towards the interior of the robustness-related feasible set.
In \cite{zhang2019policymixed},  it is emphasized that IR is a feature of both the \emph{problem} and the \emph{algorithm}, contrasting to that the stability-preserving nature of PG methods for LQR problems is based on the barrier function property of the objective and hence is \emph{algorithm-agnostic}. Although the idea of IR is relevant to PO problems with non-coercive objective functions,  the arguments in \cite{zhang2019policymixed} only apply to the setting with a \emph{known} model, since they rely on a specialized perturbation technique which may potentially generate arbitrarily small ``margins". However, in the model-free setting, a uniform margin is required for provable tolerance of statistical errors. 
 
In this paper, for the LEQG and LQ disturbance attenuation problems, we overcome the above margin issue and obtain the first IR result in the model-free setting. This enables the first model-free PG method that provably solves these control problems with a finite {number of} samples. We highlight our contributions as follows. 

\paragraph{Contributions.} 
We provide the first sample complexity results for model-free PG methods for solving linear control problems with risk-sensitivity/robustness concerns  (the LEQG and LQ disturbance attenuation problems), which was viewed as an important open problem in the seminal work \cite{fazel2018global}. From the robust control perspective, one feature of our algorithms is that, during the learning process, a certain level of \emph{robustness/risk-sensitivity} of the controller is proved to be preserved. This has  generalized the results in \cite{zhang2019policymixed} with a known model, and has thus enabled the finite-sample convergence guarantees of PO methods for risk-sensitive/robust control design. Our algorithms and sample complexity results also address two-player zero-sum LQ dynamic games in the finite-horizon time-varying setting, which are among the first sample complexity results for the global convergence of policy-based methods for competitive multi-agent RL. Second, in the context of minimax optimization,  our {results address a class of {nonconvex-nonconcave minimax} constrained optimization problems, using \emph{zeroth-order} multi-step gradient descent-ascent methods. Finally, part of our results provide the sample complexity analysis for PG methods that solve the finite-horizon time-varying LQR problem with system noises and a possibly \emph{indefinite} state-weighting matrix. 

\subsection{Related Work}
\noindent\textbf{Risk-Sensitive/Robust Control and Dynamic Games. } $\cH_{\infty}$-robust control has been one of the most fundamental research fields in control theory, addressing worst-case controller design for linear plants in the presence of unknown disturbances and uncertainties. Frequency-domain and time-domain/state-space formulations of the $\cH_{\infty}$-robust control problem were first introduced in \cite{zames1981feedback} and \cite{doyle1989state}, respectively. Based on the time-domain approach, the precise equivalence relationships between controllers in the disturbance attenuation (which belongs to a class of $\cH_{\infty}$-robust control) problem, risk-sensitive linear control, and zero-sum LQ dynamic games have been studied extensively \cite{jacobson1973optimal, glover1988state, basar1991dynamic, basar1990minimax, bacsar1998dynamic, bacsar2008h}. Specifically, \cite{jacobson1973optimal} first demonstrated the equivalence of the controllers between LEQG and zero-sum LQ (differential) games; \cite{glover1988state} studied the relationship between the mixed $\cH_2/\cH_{\infty}$ design problem, a sub-problem of the $\cH_{\infty}$-robust control problem, and LEQG; \cite{basar1991dynamic, basar1990minimax} investigated the disturbance attenuation problem through a dynamic games approach, for both finite- and infinite-horizons, time-invariant and -varying, deterministic and stochastic settings. We refer the readers to \cite{bacsar1998dynamic, bacsar2008h} for comprehensive studies of $\cH_{\infty}$-robust control, dynamic game theory, risk-sensitive control, and also their precise interconnections.
 
\vspace{0.5em}\noindent\textbf{Policy Optimization for LQ Control. }
Applying PG methods to LQ control problems has been investigated in both control and learning communities extensively.  In contrast to the early work on this topic \cite{rautert1997computational, maartensson2009gradient}, the recent study focuses more on theoretical aspects such as global convergence and sample complexity of these PG methods~\cite{fazel2018global, tu2019gap, bu2019LQR, zhang2019policy, bu2019global, mohammadi2019convergence, zhang2019policymixed,  gravell2019learning, malik2020derivative, bu2020global, mohammadi2020linear}.  Specifically, \cite{fazel2018global} was the first work to show the global convergence of PG methods for the LQR problem. Initial sample complexity results for the {derivative}-free PG methods based on zeroth-order optimization techniques were also reported in \cite{fazel2018global}. Subsequently, \cite{bu2019LQR} characterized the optimization landscape of the LQR in detail,  and provided an initial extension toward the distributive LQR. Building upon these works, \cite{malik2020derivative} enhanced the sample complexity result by adopting a two-point zeroth-order optimization method, in contrast to the single-point method adopted in \cite{fazel2018global}. The sample complexity result of the two-point method was further improved recently in both continuous- \cite{mohammadi2019convergence} and discrete-time LQR \cite{mohammadi2020linear}. Moreover, \cite{bu2020global} studied the global convergence of PG methods for the LQR where both the state and control weighting matrices are indefinite, but without addressing the {derivative}-free setting; \cite{zhang2019policy, bu2019global} derived global convergence of PG methods for zero-sum LQ dynamic games, also pointing to the need to investigate the indefinite LQR. 
{The most relevant works that addressed LQ control with \emph{robustness/risk-sensitivity concerns} using policy optimization methods were  \cite{gravell2019learning,roulet2019convergence,zhang2019policymixed}. The work in \cite{gravell2019learning}  considered LQR with multiplicative noises, which enjoys a similar landscape as standard LQR. The work in \cite{roulet2019convergence} studied  finite-horizon risk-sensitive nonlinear control, and established stationary-point convergence when using iterative LEQG and performing optimization over control actions directly.  \cite{zhang2019policymixed} examined the mixed $\cH_2/\cH_{\infty}$ control design problem, a class of $\cH_\infty$-robust control problems, with a different landscape from LQR. However, no sample complexity results were provided in either \cite{roulet2019convergence} or \cite{zhang2019policymixed}.} Very recently,  \cite{hambly2020policy} has also studied the convergence of policy gradient method for finite-horizon LQR problems. Interestingly, the landscape analysis independently developed in \cite{hambly2020policy} matches some of our findings for the inner-loop subproblem of zero-sum LQ dynamic games, while we consider a more general setting with time-varying system dynamics and a possibly indefinite state-weighting matrix. Other recent results on PO for LQ control include \cite{li2019distributed, furieri2019learning, tu2019gap, jansch2020convergence, jansch2020policy, fatkhullin2020optimizing}. 

\vspace{0.5em}\noindent\textbf{Nonconvex-Nonconcave Minimax Optimization \& MARL. }Solving minimax problems using PG methods, especially gradient descent-ascent (GDA), has been one of the most popular sub-fields in the optimization community recently. Convergence of the first-order GDA algorithm (and its variants)  has been studied  in  \cite{daskalakis2018limit, hsieh2019finding, jin2019minimax, vlatakis2019poincare} for general nonconvex-nonconcave objectives, in \cite{yang2020global} for the setting with an additional two-sided Polyak-\L{}ojasiewicz (PL) condition, and in \cite{diakonikolas2020efficient} for the setting under the weak Minty variational inequality condition. In fact, \cite{daskalakis2020complexity} has  shown  very recently the computational hardness of solving nonconvex-nonconcave constrained minimax problems with first-order methods. To the best of our knowledge, \emph{zeroth-order/derivative-free}  methods, as studied in our paper, have not yet been investigated  for nonconvex-nonconcave minimax optimization problems. On the other hand, in the multi-agent RL (MARL) regime, policy optimization for solving zero-sum Markov/dynamic games naturally leads to a nonconvex-nonconcave minimax problem \cite{zhang2019policy,zhang2019multi,daskalakis2020independent}, whose convergence guarantee has remained open \cite{zhang2019multi} until very recently, except for the aforementioned LQ setting \cite{zhang2019policy, bu2019global}. In particular, \cite{daskalakis2020independent} has established the first non-asymptotic global convergence of independent policy gradient methods for tabular (finite-state-action) zero-sum Markov games, where GDA with two-timescale stepsizes is used.  
In stark contrast to these works,  the crucial global \emph{smoothness} assumption (or property that automatically holds in the tabular MARL setting) on the objective therein does not hold in our control setting with \emph{unbounded} and \emph{continuous} spaces. A careful characterization of the iterate trajectory is thus required in order to establish global convergence and sample complexity results.

\vspace{0.5em}\noindent\textbf{Risk-Sensitive/Robust RL. }  Risk-sensitivity/robustness to model uncertainty/misspecification in RL has attracted significant research efforts, following the frameworks of robust adversarial RL (RARL) and robust Markov decision process (RMDP). Tracing back to \cite{morimoto2005robust}, early works on RARL exploited the same game-theoretic perspective as in $\cH_{\infty}$-robust control, by modeling the uncertainty as a fictitious adversary against the nominal agent. This worst-case (minimax) design concept then enabled actor-critic type algorithms with exceptional empirical performance, but rather sparse theoretical footprints \cite{pinto2017robust}. Very recently, theoretical investigations on the convergence and stability of RARL have been carried out in \cite{zhang2020rarl} within the LQ setting. In parallel, the RMDP framework has been proposed in \cite{nilim2005robust, iyengar2005robust}, and the robustness of RL algorithms under such framework has been further studied in \cite{lim2013reinforcement, lim2019kernel, mankowitz2019robust} for the \emph{finite} MDP settings, in contrast to our continuous control tasks. Other recent advances on risk-sensitive/robust RL/MDP include \cite{fei2020risk, zhang2021robust}. 

\subsection{Notations}
For a square matrix $X$ of proper dimension, we use $\Tr(X)$ to denote its trace. We also use $\|X\|$ and $\|X\|_{F}$ to denote, respectively, the operator norm and the Frobenius norm of $X$. If $X$ is further symmetric,  we use $X > 0$ to denote that $X$ is positive definite. Similarly, $X\geq 0$, $X\leq 0$, and $X <0$ are used to denote $X$ being positive semi-definite, negative semi-definite, and negative definite, respectively. Further, again for a symmetric matrix $X$, $\lambda_{\min}(X)$ and $\lambda_{\max}(X)$ are used to denote, respectively, the smallest and the largest eigenvalues of $X$. Moreover, we use $\langle X, Y \rangle:= \Tr(X^{\top}Y)$ to denote the standard matrix inner product and use $diag(X_0, \cdots, X_N)$ to denote the block-diagonal matrix with $X_0, \cdots, X_N$ on the diagonal block entries. In the case where $X_0\hspace{-0.1em}=\hspace{-0.1em}X_1\hspace{-0.1em}=\hspace{-0.1em}\cdots\hspace{-0.1em}=\hspace{-0.1em}X_N\hspace{-0.1em}=\hspace{-0.1em}X$, we further denote it as $diag(X^N)$.  We use $x\sim \cN(\mu,\Sigma)$ to denote a Gaussian random variable with mean $\mu$ and covariance $\Sigma$ and use $\|v\|$ to denote the Euclidean norm of a vector $v$. Lastly, we use $\bI$ and $\bm{0}$ to denote the identity and zero matrices with appropriate dimensions.



==> Mixed Design Arxiv v3/LEQG.tex <==
In this section, we first introduce two classic settings in risk-sensitive and robust control, namely LEQG, and LQ disturbance attenuation. We then discuss, in \S\ref{sec:mix}, the challenges one confronts when attempting to address the above two problems directly using derivative-free PG methods by sampling system trajectories. Fortunately, solving zero-sum LQ (stochastic) dynamic games, a benchmark setting in MARL, via derivative-free PG methods by sampling system trajectories provides a workaround to address these problems all in a unified way, due to the well-known equivalence relationships between zero-sum LQ dynamic games and the two aforementioned classes of problems \cite{bacsar2008h}, which we will also discuss in \S\ref{sec:game}. 

\subsection{Linear Exponential Quadratic Gaussian}\label{sec:leqg}
We first consider a fundamental setting of risk-sensitive optimal control, known as the LEQG problem \cite{jacobson1973optimal, whittle1981risk, whittle1990risk}, in the finite-horizon setting. The time-varying (linear)  systems dynamics are described by: 
\begin{align*}
	&x_{t+1} = A_tx_t + B_tu_t + w_t, \quad t\in\{0,\cdots,N-1\},
\end{align*} 
where $x_t \in \RR^{m}$ represents the system state; $u_t \in \RR^{d}$ is the control input; $w_t \in \RR^{m}$ is an independent (across time) Gaussian random noise drawn from $w_t\sim \cN(\bm{0}, W)$ for some $W>0$; the initial state $x_0 \sim \cN(\bm{0}, X_0)$ is a Gaussian random vector for some $X_0 > 0$, independent of the sequence $\{w_t\}$; and $A_t$, $B_t$ are time-varying system matrices with appropriate dimensions. The objective function is given by
\begin{align*}
	\cJ\big(\{u_t\}\big) :=  \frac{2}{\beta}\log\EE\exp\Big[\frac{\beta}{2}\big(\sum^{N-1}_{t=0}(x_t^{\top}Q_tx_t + u_t^{\top}R_tu_t) + x_N^{\top}Q_Nx_N\big)\Big],
\end{align*}
where $Q_t \geq 0$ and $R_t > 0$, for all $t \in \{0, \cdots, N-1\}$, and $Q_N \geq 0$ are symmetric weighting matrices; and $\beta> 0$ is a parameter capturing the degree of risk-sensitivity, which is upper-bounded by some $\beta^* > 0$ \cite{glover1988state, whittle1990risk, nishimura2021rat}. 

The goal in the LEQG problem is to find the $\cJ$-minimizing optimal control policy $\mu^*_t: (\RR^{m}\times\RR^d)^t \times \RR^m \rightarrow \RR^d$ that maps, at time $t$, the history of state-control pairs up to time $t$ and the current state $x_t$ to the control $u_t$, this being so for all $t \in\{0, \cdots, N-1\}$. It has been shown in \cite{jacobson1973optimal} that $\mu_t^*$ has a linear state-feedback form $\mu^*_t(x_t) = -K_t^*x_t$, where $K^*_t \in \RR^{d\times m}$, for all $t\in\{0, \cdots, N-1\}$. Therefore, it suffices to search $K^*_t$ in the matrix space $\RR^{d \times m}$ for all $t\in\{0, \cdots, N-1\}$, without losing any optimality. The resulting policy optimization problem is then represented as  (by a slight abuse of notation with regard to $\cJ$):
\begin{align}\label{eqn:leqg_objective}
	\min_{\{K_t\}}~\cJ\big(\{K_t\}\big) := \frac{2}{\beta}\log\EE\exp\Big[\frac{\beta}{2}\big(\sum^{N-1}_{t=0}\big(x_t^{\top}(Q_t + K_t^{\top}R_tK_t)x_t\big) + x_N^{\top}Q_Nx_N\big)\Big].
\end{align}
To characterize the solution to \eqref{eqn:leqg_objective}, we first introduce the following time-varying Riccati difference equation (RDE):
\begin{align}\label{eqn:RDE_LEQG}
	P_{K_t} = Q_t + K_t^{\top}R_tK_t + (A_t-B_tK_t)^{\top}\tilde{P}_{K_{t+1}}(A_t-B_tK_t), \quad t\in\{0, \cdots, N-1\}, \quad P_{K_N} = Q_N,
\end{align}
where $\tilde{P}_{K_{t+1}}:= P_{K_{t+1}} + \beta P_{K_{t+1}}(W^{-1}- \beta P_{K_{t+1}})^{-1}P_{K_{t+1}}$. Then, \eqref{eqn:leqg_objective} can be expressed by the solution to \eqref{eqn:RDE_LEQG} and the exact PG can be analyzed, as follows, with its proof being deferred to \S\ref{proof:pg_leqg}.

\begin{lemma}(Closed-Form Objective Function and PG) \label{lemma:pg_leqg} For any sequence of $\{K_t\}$ such that \eqref{eqn:RDE_LEQG} generates a sequence of positive semi-definite (p.s.d.) sequence $\{P_{K_{t}}\}$ satisfying $X_0^{-1} - \beta P_{K_0} > 0$ and $W^{-1}\hspace{-0.15em}-\hspace{-0.12em}\beta P_{K_{t}}\hspace{-0.05em} >\hspace{-0.05em}0$, for all $t \in \{1, \cdots, N\}$, the objective function $\cJ\big(\{K_t\}\big)$ can be expressed as
\begin{align}\label{eqn:LEQG_obj_closed}
	\cJ\big(\{K_t\}\big) = -\frac{1}{\beta}\log\det(\bI - \beta P_{K_{0}}X_0) -\frac{1}{\beta}\sum_{t=1}^{N}\log\det(\bI - \beta P_{K_{t}}W).
\end{align}
As $\beta \rightarrow 0$, \eqref{eqn:LEQG_obj_closed} reduces to $\tr(P_{K_0}X_0) + \sum_{t=1}^{N}\tr(P_{K_{t}}W)$, which is the objective function of the \emph{finite-horizon} linear-quadratic-Gaussian (LQG) problem. Moreover, the PG of \eqref{eqn:LEQG_obj_closed} at time $t$ has the form:
	\begin{align}\label{eqn:LEQG_PG}
		\nabla_{K_t}\cJ\big(\{K_t\}\big) := \frac{\partial \cJ\big(\{K_t\}\big)}{\partial K_t} = 2\big[(R_t+B^{\top}_t\tilde{P}_{K_{t+1}}B_t)K_t - B_t^{\top}\tilde{P}_{K_{t+1}}A_t\big]\Sigma_{K_t}, \quad t\in\{0, \cdots, N-1\},
	\end{align}
where
\begin{align*}
	\Sigma_{K_t} &:= \prod^{t-1}_{i=0}\big[(\bI- \beta P_{K_{i+1}}W)^{-\top}(A_{i} -B_{i}K_{i})\big]\cdot X_0^{\frac{1}{2}}(\bI - \beta X_0^{\frac{1}{2}}P_{K_{0}}X_0^{\frac{1}{2}})^{-1}X_0^{\frac{1}{2}} \cdot\prod^{t-1}_{i=0}\big[(A_{i} -B_{i}K_{i})^{\top}(\bI-\beta P_{K_{i+1}}W)^{-1}\big]\\
	&\hspace{1em} + \sum_{\tau = 1}^{t}\bigg\{\prod^{t-1}_{i=\tau}\big[(\bI-\beta P_{K_{i+1}}W)^{-\top}(A_{i} -B_{i}K_{i})\big]\cdot W^{\frac{1}{2}}(\bI - \beta W^{\frac{1}{2}}P_{K_{\tau}}W^{\frac{1}{2}})^{-1}W^{\frac{1}{2}} \cdot\prod^{t-1}_{i=\tau}\big[(A_{i} -B_{i}K_{i})^{\top}(\bI-\beta P_{K_{i+1}}W)^{-1}\big]\bigg\}.
\end{align*}
\end{lemma}
 


==> Mixed Design Arxiv v3/auxiliary.tex <==
\subsection{Hessians} \label{sec:Hessian}
\xznote{consider not using this... looks stupid, see how Zhengyang proves smoothness}
\begin{lemma}(Hessian of The Inner Loop Problem)
For $X \in \RR^{mN\times n(N+1)}$, and with $(\bP'_{\bL})[X]$ representing the action of differential of the mapping 
$\bL \rightarrow \bP_{\bL}$, the Hessian of the inner loop problem is expressed as
\begin{align}\label{eqn:exact_hessian_L}
	\nabla^2 \cG(\bL)[X, X] = 2\big\langle \bF_{\bL}X\Sigma_{\bL} , X\big\rangle - 4 \big\langle (\bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL})\Sigma_{\bL}, X\big\rangle
\end{align}	
\begin{proof}
	Let $\bE_{\bL}'$ and $\Sigma_{\bL}'$ denote the derivatives with respect to $\bL$ of, respectively, $\bE_{\bL}$ and $\Sigma_{\bL}$. Then, the Hessian of the inner loop problem can be characterized as $\nabla^2\cG(\bL) = 2\bE_{\bL}'\Sigma_{\bL} + 2\bE_{\bL}\Sigma_{\bL}'$, and for $X \in \RR^{mN\times n(N+1)}$, the action of $\nabla^2\cG(\bL)[X, X]$ is given by 
	\begin{align*}
	\nabla^2\cG(\bL)[X, X] &= 2\Big\langle \big((\bR^w + \bD^T\bP_{\bL}\bD)X - \bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL}\big)\Sigma_{\bL}, X\Big\rangle + 2 \Big\langle \bE_{\bL}\big(\Sigma_{\bL}'[X]\big), X\Big\rangle,
%		\frac{d(P_t)}{d(K_t)} = 2(RK_t-B^TP_{t+1}(A-BK_t))
	\end{align*}
 where
	\begin{align*}
		\bP_{\bL}'[X] &= \tilde{\bA}^T_{\bL}(\bP_{\bL}'[X])\tilde{\bA}_{\bL} + 2X^T\bE_{\bL} \\
		\Sigma_{\bL}'[X] &= \tilde{\bA}_{\bL}(\Sigma_{\bL}'[X])\tilde{\bA}^T_{\bL} - \bD X\Sigma_{\bL}\tilde{\bA}^T_{\bL} - \tilde{\bA}_{\bL}\Sigma_{\bL} X^T\bD.
	\end{align*}
	Note that $\bP_{\bL}'[X]$ and $\Sigma_{\bL}'[X]$ can be solved by
	\begin{align}\label{eqn:pk_gradient}
		\bP_{\bL}'[X] &= \sum^N_{i = 0} \big(\tilde{\bA}^T_{\bL}\big)^i\big(2X^T\bE_{\bL}\big)\big(\tilde{\bA}_{\bL}\big)^i \\
		\Sigma_{\bL}'[X] &= \sum^N_{i = 0} \big(\tilde{\bA}_{\bL}\big)^i\big(- \bD X\Sigma_{\bL}\tilde{\bA}^T_{\bL} - \tilde{\bA}_{\bL}\Sigma_{\bL} X^T\bD\big)\big(\tilde{\bA}^T_{\bL}\big)^i.
	\end{align}
	Therefore, the action of the Hessian of the inner loop problem can be represented as
	\begin{align*}
		\nabla^2\cG(\bL)[X, X] &= 2\big\langle (\bR^w + \bD^T\bP_{\bL}\bD)X\Sigma_{\bL} , X\big\rangle - 4 \big\langle (\bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL})\Sigma_{\bL}, X\big\rangle \\
		&= 2\big\langle \bF_{\bL}X\Sigma_{\bL} , X\big\rangle - 4 \big\langle (\bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL})\Sigma_{\bL}, X\big\rangle.
	\end{align*}
	This completes the proof of \eqref{eqn:exact_hessian_L}.
\end{proof}
	
\end{lemma}
\begin{lemma}(Hessian of The Outer Loop Problem)
For $X \in \RR^{mN\times d(N+1)}$, and with $(\bE'_{\bK, \bL(\bK)})[X]$ representing the action of differential of the mapping $\bK \rightarrow \bE_{\bK}$, the Hessian of the outer loop problem is expressed as
	\begin{align}\label{eqn:exact_hessian_K}
		\nabla^2\cG(\bK)[X, X] &= 2\big\langle \bE_{\bK}'[X]\Sigma_{\bK} , X\big\rangle + 2 \big\langle \bE_{\bK}\Sigma_{\bK}'[X], X\big\rangle.
	\end{align}
For ease of expositions, we further define : $\Sigma := \Sigma_{\bK}$, $\bP:=\bP_{\bK}$, $\Lambda := \bR^w - \bD^T\bP_{\bK}\bD$, and $\tilde{\bP} := \tilde{\bP}_{\bK}$. Then, $\bE'[X]$ is defined as follows
 \small
 \begin{align}
 	\hspace{-1em}\bE_{\bK}'[X] &= \bF_{\bK} X  - \bB^T\bP'[X]\bA_{\bK} \nonumber\\
 	&\hspace{1em} + \bK\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB + \bK\bD^T\bP\bB\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} + \bK\bD^T\bP\bB\Lambda^{-1}\bB^T\bP'[X]\bD \nonumber\\
 	&\hspace{1em} -\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB\bA - \bD^T\bP\bB\bA\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} - \bD^T\bP\bB\bA\Lambda^{-1}\bB^T\bP'[X]\bD,\label{eqn:E'}
 \end{align}
 \normalsize
 where the definitions of $\bP'[X]$ and $\Sigma'[X]$ are represented, respectively, as
 \begin{align}
		\bP'[X] &= \bA_{\bK}^T(\bP'[X])\bA_{\bK} + 2X^T\bE_{\bK} \label{eqn:pk'}\\
		\Sigma'[X] &= \bA_{\bK}(\Sigma'[X])\bA_{\bK}^T - \bB X\Sigma\bA_{\bK}^T - \bA_{\bK}\Sigma X^T\bB. \label{eqn:sigmak'}
\end{align}
\end{lemma}

\begin{proof}
Let $\bE_{\bK}'$ and $\Sigma_{\bK}'$ denote the derivatives with respect to $\bK$ of, respectively, $\bE_{\bK}$ and $\Sigma_{\bK}$. Then, by the gradient form reported in Lemma \ref{lemma:exact_PG_K}, the Hessian can be characterized as $\nabla^2\cG(\bK) = 2\bE_{\bK}'\Sigma_{\bK} + 2\bE_{\bK}\Sigma_{\bK}'$, and for $X \in \RR^{mN\times d(N+1)}$, the action of $\nabla^2\cG(\bK)[X, X]$ is given by 
	\begin{align*}
	\nabla^2\cG(\bK)[X, X] &= 2\big\langle \bE_{\bK}'[X]\Sigma_{\bK} , X\big\rangle + 2 \big\langle \bE_{\bK}\Sigma_{\bK}'[X], X\big\rangle.
%	&= 2\Big\langle \big((\bR^u+ \bB^T\tilde{\bP}_{\bK, \bL(\bK)}\bB)X - \bB^T(\tilde{\bP}_{\bK, \bL(\bK)}'[X])(\bA-\bB\bK)\big)\Sigma_{\bK, \bL(\bK)} , X\Big\rangle + 2 \Big\langle \bE_{\bK, \bL(\bK)}\big(\Sigma_{\bK, \bL(\bK)}'[X]\big), X\Big\rangle,
%		\frac{d(P_t)}{d(K_t)} = 2(RK_t-B^TP_{t+1}(A-BK_t))
	\end{align*}
 To further simplify the notations, we let $\bP:=\bP_{\bK}$, $\Lambda := \bR^w - \bD^T\bP_{\bK}\bD$, and $\tilde{\bP} := \tilde{\bP}_{\bK}$. Then, 
 \small
 \begin{align*}
 	\bE_{\bK}'[X] &= \bF_{\bK} X  - \bB^T\bP'[X]\bA_{\bK} \nonumber\\
 	&\hspace{1em} + \bK\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB + \bK\bD^T\bP\bB\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} + \bK\bD^T\bP\bB\Lambda^{-1}\bB^T\bP'[X]\bD \nonumber\\
 	&\hspace{1em} -\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB\bA - \bD^T\bP\bB\bA\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} - \bD^T\bP\bB\bA\Lambda^{-1}\bB^T\bP'[X]\bD,
 \end{align*}
 \normalsize
 where
 \begin{align*}
		\bP'[X] &= \bA_{\bK}^T(\bP'[X])\bA_{\bK} + 2X^T\bE_{\bK} \\
		\Sigma'[X] &= \bA_{\bK}(\Sigma'[X])\bA_{\bK}^T - \bB X\Sigma\bA_{\bK}^T - \bA_{\bK}\Sigma X^T\bB.
\end{align*}
	Note that $\bP'[X]$ and $\Sigma'[X]$ can be solved by the iterative equations
	\begin{align*}
		\bP'[X] &= \sum^N_{i = 0} \big( \bA_{\bK}^T\big)^i\big(2X^T\bE_{\bK}\big)\big( \bA_{\bK}\big)^i \nonumber\\
		\Sigma'[X] &= \sum^N_{i = 0} \big(\bA_{\bK}\big)^i\big(- \bB X\Sigma\bA_{\bK}^T - \bA_{\bK}\Sigma X^T\bB\big)\big(\bA_{\bK}^T\big)^i. 
	\end{align*}
	Therefore, the action of the Hessian can be represented as
	\begin{align*}
		\nabla^2\cG(\bK)[X, X] &= 2\big\langle \bE_{\bK}'[X]\Sigma , X\big\rangle + 2 \big\langle \bE_{\bK}\Sigma'[X], X\big\rangle,
	\end{align*}
	where $\bE_{\bK}'[X]$ and $\Sigma'[X]$ follow the definitions in \eqref{eqn:E'} and \eqref{eqn:sigmak'}, respectively. This completes the proof of \eqref{eqn:exact_hessian_K}.
\end{proof}

\subsection{Auxiliary Bounds: The Inner Loop Problem}\label{sec:bounds_L}
\begin{lemma}
	For a fixed outer loop control gain matrix $\bK$ and for any $\bL \in \cS_{\bL}(a)$, there exist positive auxiliary constants reported in the left column of Table \ref{table:L}, such that the bounds in the right column of Table \ref{table:L} hold.
\end{lemma}
\begin{table}[!h]

\begin{tabular*}{\textwidth}{
  @{\extracolsep{\fill}}
  l
  >{$\displaystyle}c<{\vphantom{\sum_{1}{N}}$}
  >{\refstepcounter{equation}(\theequation)}r
  @{}
}
\toprule
\textbf{Auxiliary Constants} & \multicolumn{1}{c}{\textbf{Auxiliary Bounds: The Inner Loop Problem}} & \multicolumn{1}{c}{} \\
\midrule
$c_{\iota_1} := c_{\bP_{\bL}, a}$  &
  	\|\bP_{\bL}\| \leq  c_{\iota_1} &
  \label{bound:P_L}
\\
$c_{\iota_2} := sNC_m$ & 
  \|\Sigma_{\bL}\| \leq  c_{\iota_2} & \label{bound:sigma_L}
\\
$c_{\iota_3} :=$\small $\sqrt{(\|\bR^w\| + \|\bD\|^2c_{\iota_1})(a - \cG(\bL^*)))}$\normalsize &
  \|\bE_{\bL}\| \leq c_{\iota_3} & \label{bound:E_L}
\\
 $c_{\iota_4} := \frac{c_{\iota_3}+\|\bB\|\|\tilde{\bA}\|c_{\iota_1}}{\lambda_{\min}(\bR^w)}$&
  \|\nabla\cG(\bL)\| \leq c_{\iota_2}c_{\iota_3} & \label{bound:grad_L}
\\
& 
  \|\bL\| \leq c_{\iota_4} & \label{bound:L}
\\
&
  \|\cT_{\bL}\| \leq c_{\iota_2} & \label{bound:TL}
\\
\bottomrule
\end{tabular*}
\caption{Auxiliary constants and bounds for the Inner loop problem.}\label{table:L}
\end{table}

\begin{proof}
	First, due to the finite-horizon setting that is considered in this paper, mappings $\bL \rightarrow \bP_{\bL}$ is continuous for a fixed outer loop control gain matrix $\bK$. Thus, there exist uniform upper bounds such that for $\bL \in \cS_{\bL}(a)$,
	\begin{align*}
		\|\bP_{\bL}\| \leq c_{\bP_{\bL}, a} = c_{\iota_1}.
	\end{align*}
	This proves \eqref{bound:P_L}. Next, because that $\Sigma_{\bL}$ is the solution of the Lyapunov equation
	\begin{align*}
		\Sigma_{\bL} = \tilde{\bA}_{\bL}\Sigma_{\bL}\tilde{\bA}_{\bL}^T + \Sigma_0,
	\end{align*} 
	where $\Sigma_0 = \EE[\bm{\xi}\bm{\xi}^T]$ and $\|\bm{\xi}\|^2 \leq sC_m$ almost surely due to the assumption on the distribution $\cD$. Since $\Sigma_{\bL}$ can be solved iteratively via 
	\begin{align*}
		\Sigma_{\bL} = \sum^{N}_{t=0}\big(\tilde{\bA}_{\bL}\big)^{t}\Sigma_{0} \big((\tilde{\bA}_{\bL})^T\big)^t,
	\end{align*}
	we can bound $\|\Sigma_{\bL}\|$ by $\|\Sigma_{\bL}\| \leq sNC_m = c_{\iota_1}$. This proves \eqref{bound:sigma_L}. Next, we prove \eqref{bound:E_L} by deriving a lower bound that provides counterparts of the results in Lemma \ref{lemma:gd_L}. Specifically, under the assumption that $\cG(\bL') \geq \cG(\bL^*)$, we have
	\begin{align*}
		\cG(\bL) - \cG(\bL^*) &\geq \cG(\bL) - \cG(\bL') \geq \Tr\big(\Sigma_{\bL'} \bE^T_{\bL}\bF^{-1}_{\bL}\bE_{\bL} \big) \\
			&\geq \frac{\lambda_{\min}(\Sigma_{\bL'})}{\|\bF_{\bL}\|}\Tr\big(\bE^T_{\bL}\bE_{\bL} \big) \geq \frac{1}{\|\bF_{\bL}\|}\Tr\big(\bE^T_{\bL}\bE_{\bL} \big).
	\end{align*}
	The last inequality is because of $\Sigma_{\bL'} \geq \Sigma_0 = \textbf{I}$. By utilizing \eqref{bound:P_L}, it leads to 
	\begin{align*}
		\Tr\big(\bE^T_{\bL}\bE_{\bL} \big) \leq \|\bF_{\bL}\|(\cG(\bL) - \cG(\bL^*)) \leq (\|\bR^w\| + \|\bD\|^2c_{\iota_1})(a - \cG(\bL^*)) = c_{\iota_3}^2.
	\end{align*}
Then, \eqref{bound:E_L} can be concluded. Furthermore, invoking Lemma 25 of \cite{fazel2018global} and applying \eqref{bound:sigma_L} yields
\begin{align*}
	\|\nabla\cG(\bL)\|^2 \leq \Tr(\Sigma_{\bL}\bE^T_{\bL}\bE_{\bL}\Sigma_{\bL}) \leq \|\Sigma_{\bL}\|^2\Tr(\bE^T_{\bL}\bE_{\bL}) \leq \big(c_{\iota_2}c_{\iota_3} \big)^2.
\end{align*}
Taking square-root of both sides proves \eqref{bound:grad_L}. Next, Lemma 25 of \cite{fazel2018global} suggests that
\begin{align*}
	\|\bL\| \leq \frac{\sqrt{(\|\bR^w\| + \|\bD\|^2c_{\iota_1})(a - \cG(\bL^*))}}{\lambda_{\min}(\bR^w)} + \frac{\|\bD\|\|\tilde{\bA}\|c_{\iota_1}}{\lambda_{\min}(\bR^w)} = \frac{c_{\iota_3}+\|\bB\|\|\tilde{\bA}\|c_{\iota_1}}{\lambda_{\min}(\bR^w)} = c_{\iota_4}, 
\end{align*}
yielding \eqref{bound:L}. Lastly, combining the results from Lemma 17 of \cite{fazel2018global} with \eqref{bound:sigma_L} yields \eqref{bound:TL} as follows
	\begin{align*}
		\|\cT_{\bL}\| \leq \|\Sigma_{\bL}\| \leq c_{\iota_2}.
	\end{align*}
	This completes the proof.
\end{proof}


\subsection{Auxiliary Bounds: The Outer Loop Problem}\label{sec:bounds_K}
\begin{lemma}
	For $\bK \in \cS_{\bK}(a)$, there exist positive auxiliary constants reported in the left column of Table \ref{table:K}, such that the bounds in the right column of Table \ref{table:K} hold.
\end{lemma}

\begin{table}[!h]

\begin{tabular*}{\textwidth}{
  @{\extracolsep{\fill}}
  l
  >{$\displaystyle}c<{\vphantom{\sum_{1}{N}}$}
  >{\refstepcounter{equation}(\theequation)}r
  @{}
}
\toprule
\textbf{Auxiliary Constants} & \multicolumn{1}{c}{\textbf{Auxiliary Bounds: The Outer Loop Problem}} & \multicolumn{1}{c}{} \\
\midrule
$c_{\kappa_1} := c_{\bP_{\bK}, a}$  &
  	\|\bP_{\bK}\| \leq  c_{\kappa_1} &
  \label{bound:P_K}
\\
$c_{\kappa_2} := sNC_m$ & 
  \|\Sigma_{\bK}\| \leq  c_{\kappa_2} & \label{bound:sigma_K}
\\
$c_{\kappa_3} := c_{\kappa_1} + \|\bR^w\|\|\bD\|^2c^2_{\kappa_1}$ &
  \|\tilde{\bP}_{\bK}\| \leq c_{\kappa_3} & \label{bound:barP_K}
\\
$c_{\kappa_4} :=$\small $\sqrt{(\|\bR^u\| + \|\bB\|^2c_{\kappa_3})(a - \cG(\bK^*))}$\normalsize &
  \|\bE_{\bK}\| \leq c_{\kappa_4} & \label{bound:E_K}
\\
 $c_{\kappa_5} := \frac{c_{\kappa_4}+\|\bB\|\|\bA\|c_{\kappa_3}}{\lambda_{\min}(\bR^u)}$&
  \|\nabla\cG(\bK)\| \leq c_{\kappa_2}c_{\kappa_4} & \label{bound:grad_K}
\\
$c_{\kappa_6} :=$ \small$2\|\bB\|c_{\kappa_2}c_{\kappa_4}(\|\bA\| + \|\bB\|c_{\kappa_5})$\normalsize& 
  \|\bK\| \leq c_{\kappa_5} & \label{bound:K}
\\
\hspace{2em}\small$+(4 + 2\|\bR^w\|\|\bD\|^2c_{\kappa_1})\|\bR^w\|\|\bB\|^2\|\bD\|^2$\normalsize&
  \|\cT_{\bK}\| \leq c_{\kappa_2} & \label{bound:TK}
\\
\hspace{2em}\small$c_{\kappa_1}c_{\kappa_2}c_{\kappa_4}(c_{\kappa_5}+\|\bA\|) + \|\bR^u\| + \|\bB\|^2c_{\kappa_3}$\normalsize&
  \|\bE'_{\bK}\| \leq c_{\kappa_6} & \label{bound:EK'}
\\
\bottomrule
\end{tabular*}
\caption{Auxiliary constants and bounds for the outer loop problem.}\label{table:K}
\end{table}


\begin{proof}
First, due to the finite-horizon setting that is considered in this paper, mappings $\bK \rightarrow \bP_{\bK}$ is continuous. Thus, there exist an uniform upper bound such that for $\bK \in \cS_{\bK}(a)$,
	\begin{align*}
		\|\bP_{\bK}\| \leq c_{\bP_{\bK}, a} = c_{\kappa_1}.
    \end{align*}
	This proves \eqref{bound:P_K}. Next, because that $\Sigma_{\bK}$ is the solution of the Lyapunov equation
	\begin{align*}
		\Sigma_{\bK} = \bA_{\bK, \bL}\Sigma_{\bK} \bA_{\bK, \bL}^T + \Sigma_0,
	\end{align*} 
	where $\Sigma_0 = \EE[\bm{\xi}\bm{\xi}^T]$ and $\|\bm{\xi}\|^2 \leq sC_m$ almost surely due to the assumption on the distribution $\cD$. Since $\Sigma_{\bK}$ can be solved iteratively via 
	\begin{align*}
		\Sigma_{\bK} = \sum^{N}_{t=0}\big(\bA_{\bK, \bL}\big)^{t}\Sigma_{0} \big(\bA_{\bK, \bL}^T\big)^t,
	\end{align*}
	we can bound $\|\Sigma_{\bK}\|$ by $\|\Sigma_{\bK}\| \leq sNC_m = c_{\kappa_1}$. This proves \eqref{bound:sigma_K}. Furthermore, by the definition of $\tilde{\bP}_{\bK}$, we can prove \eqref{bound:barP_K} by
	\begin{align*}
		\|\tilde{\bP}_{\bK}\| \leq c_{\kappa_1} + \|\bR^w - \bD^T\bP_{\bK}\bD\|\|\bD\|^2c^2_{\kappa_1} \leq c_{\kappa_1} + \|\bR^w\|\|\bD\|^2c^2_{\kappa_1} := c_{\kappa_3}.
	\end{align*}
	Subsequently, we consider $\bK' = \bK - \bF_{\bK}^{-1}\bE_{\bK}$, which is the Gauss-Newton update \eqref{eqn:gn_K} with stepsize $1/2$. Under the assumption that $\cG(\bK^*) \leq \cG(\bK')$, we have
	\begin{align*}
		\cG(\bK) - \cG(\bK^*) &\geq \cG(\bK) - \cG(\bK') \geq \Tr(\bE^T_{\bK}\bF_{\bK}^{-1}\bE_{\bK}) \geq \frac{1}{\|\bF_{\bK}\|}\Tr(\bE^T_{\bK}\bE_{\bK}).
	\end{align*}
	This yields
	\begin{align*}
		\Tr(\bE^T_{\bK}\bE_{\bK}) &\leq \|\bF_{\bK}\|(\cG(\bK) - \cG(\bK^*)) \leq (\|\bR^u\| + \|\bB\|^2c_{\kappa_3})(a - \cG(\bK^*)) = c_{\kappa_4}^2.
	\end{align*}
	Therefore, we prove \eqref{bound:E_K}. Also, by invoking Lemma 25 of \cite{fazel2018global}, we can derive that
	\begin{align*}
		\|\nabla\cG(\bK)\|^2 &\leq \Tr(\Sigma_{\bK}\bE^T_{\bK}\bE_{\bK}\Sigma_{\bK}) \leq \|\Sigma_{\bK}\|^2 \Tr(\bE^T_{\bK}\bE_{\bK}) \leq (c_{\kappa_2}c_{\kappa_4})^2.
	\end{align*}
	Taking square root of both sides proves \eqref{bound:grad_K}. Next, Lemma 25 of \cite{fazel2018global} suggests that
\begin{align*}
	\|\bK\| \leq \frac{\sqrt{(\|\bR^u\| + \|\bB\|^2c_{\kappa_3})(a - \cG(\bK^*))}}{\lambda_{\min}(\bR^u)} + \frac{\|\bB\|\|\bA\|c_{\kappa_3}}{\lambda_{\min}(\bR^u)} = \frac{c_{\kappa_4}+\|\bB\|\|\bA\|c_{\kappa_3}}{\lambda_{\min}(\bR^u)} = c_{\kappa_5}, 
\end{align*}
yielding \eqref{bound:K}. Furthermore,  combining Lemma 17 of \cite{fazel2018global} with \eqref{bound:sigma_K} yields \eqref{bound:TK} as follows
	\begin{align*}
		\|\cT_{\bK}\| \leq \|\Sigma_{\bK}\| \leq c_{\kappa_2}.
	\end{align*}
Lastly, we focus on proving the upper bound for $\|\bE'_{\bK}\|$. To start with, by the definition of $\bP_{\bK}'$ in \eqref{eqn:pk'}, we can show that
\begin{align*}
	\|\bP_{\bK}'\| \leq 2\|\cT_{\bK}\|\|\bE_{\bK}\| \leq 2c_{\kappa_2}c_{\kappa_4}.
\end{align*}
Then, by the definition of $\bE'_{\bK}$ in \eqref{eqn:E'}, we can show that
\begin{align*}
	\|\bE'_{\bK}\| &\leq \|\bR^u\| + \|\bB\|^2c_{\kappa_3} + 2\|\bB\|c_{\kappa_2}c_{\kappa_4}(\|\bA\| + \|\bB\|c_{\kappa_5}) \\
	&\hspace{1em} + 4\|\bR^w\|\|\bB\|^2\|\bD\|^2c_{\kappa_1}c_{\kappa_2}c_{\kappa_4}c_{\kappa_5} + 2\|\bR^w\|^2\|\bB\|^2\|\bD\|^4c^2_{\kappa_1}c_{\kappa_2}c_{\kappa_4}c_{\kappa_5}\\
	&\hspace{1em} + 4\|\bR^w\|\|\bA\|\|\bB\|^2\|\bD\|^2c_{\kappa_1}c_{\kappa_2}c_{\kappa_4} + 2\|\bR^w\|^2\|\bA\|\|\bB\|^2\|\bD\|^4c^2_{\kappa_1}c_{\kappa_2}c_{\kappa_4} \\
	&= \|\bR^u\| + \|\bB\|^2c_{\kappa_3} + 2\|\bB\|c_{\kappa_2}c_{\kappa_4}(\|\bA\| + \|\bB\|c_{\kappa_5})\\
	&\hspace{1em} + (4 + 2\|\bR^w\|\|\bD\|^2c_{\kappa_1})\|\bR^w\|\|\bB\|^2\|\bD\|^2c_{\kappa_1}c_{\kappa_2}c_{\kappa_4}(c_{\kappa_5}+\|\bA\|) = c_{\kappa_6}.
\end{align*}
This completes the proof of \eqref{bound:EK'}
\end{proof}

%\subsection{Proof of Theorem \ref{theorem:free_pg_L}}
% \begin{proof}
% 	For ease of notation, we define $\Delta_l = \cG(\bL_l) - \cG(\bL^*)$ as the optimality gap between the control gain matrix $\bL_l$ at iteration $l$ and the optimal control gain matrix $\bL^*$. Also, we define
% 	\begin{align*}
% 		G_{\infty} := \sup_{\bL}~ \|\nabla\cG(\bL)\|, \quad G_2 := \sup_{\bL}~ \EE~\Big[\big\|\nabla\cG(\bL) - \EE~\big[\nabla\cG(\bL) \mid \bL\big]\big\|^2\Big]
% 	\end{align*}
% 	as the uniform bounds on the gradient norm and its variance, respectively.  Suppose that the algorithm parameters are chosen to satisfy \eqref{eqn:one_point_req}, we first focus on proving that for any iteration index $l$, inequality
% \begin{align}\label{eqn:delta_bound}
% 	\EE_l[\Delta_{l+1}] \leq (1-\frac{\eta c_g}{4})\Delta_l + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta c_g \frac{\epsilon_{\bL}\delta}{20}
% \end{align}
% holds, where $\EE_l[\Delta_{l}]$ denotes the expectation of the optimality gap at iteration $l$. From page 24 of \cite{malik2020derivative}, we can apply Markov's inequality to obtain
% 	\begin{align*}
% 		\EE_l[\Delta_{l+1} - \Delta_l] \leq - \frac{\eta c_g}{2}\Delta_l + \frac{\eta c_g}{4}\Delta_l + 4\frac{\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta^2\psi_{\bL}^3r_{\bL}^2,
% 	\end{align*}
% 	where $\theta_{\bL} = \min\{\frac{1}{2\psi_{\bL}}, \frac{1}{l_{\bL}}\}$. Since \eqref{eqn:one_point_req} is satisfied, we can derive that $\frac{4\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$ and $\eta^2\psi_{\bL}^3r_{\bL}^2 \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$. This completes the proof of \eqref{eqn:delta_bound}. Subsequently, we want to show that if \eqref{eqn:one_point_req} is satisfied, then we will have 
% 	\begin{align}\label{eqn:intermediate_E}
% 		\EE[\Delta_{\cL}] \leq \epsilon_{\bL}\delta.
% 	\end{align}
% 	with probability $1$. Suppose $\eta \leq \frac{\epsilon_{\bL} c_g\delta}{40\psi_{\bL} G_2}$, we have
% 	\begin{align*}
% 		\EE [\Delta_{l+1}] &\leq \Big(1-\frac{\eta c_g}{4}\Big)^{l+1}\Delta_0 + \Big(\frac{\psi_{\bL}\eta^2G_2}{2} + \frac{\eta c_g \epsilon_{\bL}\delta}{20}\Big)\sum^{l}_{i=0}\Big(1 - \frac{\eta c_g}{4}\Big)^i \\
% 		&\leq \Big(1-\frac{\eta c_g}{4}\Big)^{l+1}\Delta_0 + \frac{2\psi_{\bL}\eta G_2}{c_g} + \frac{\epsilon_{\bL}\delta}{5} \\
% 		& \leq \Big(1-\frac{\eta c_g}{4}\Big)^{l+1}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4}.
%  	\end{align*}
%  	Let $\cL = l+1$, we can verify that if $\cL = \frac{4}{\eta c_g}\log(\frac{4\Delta_0}{3\delta\epsilon_{\bL}})$, then
%  	\begin{align*}
%  		\Big(1-\frac{\eta c_g}{4}\Big)^{\cL}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4} \leq \epsilon_{\bL}\delta.
%  	\end{align*}
%  	This leads to $\EE[\Delta_{\cL}] \leq \epsilon_{\bL}\delta$.  Moreover, applying Markov's inequality leads to
% 	\begin{align*}
% 		P\{\Delta_\cL \geq \epsilon_{\bL}\} \leq \frac{1}{\epsilon_{\bL}}\EE[\Delta_{\cL}] \leq \delta,
% 	\end{align*}
% 	which implies $P\{\Delta_\cL \leq \epsilon_{\bL}\} > 1- \delta$. Lastly, we provide bounds for $G_2$ and $G_{\infty}$. By definition of the estimated cost function, their exists an absolute constant $c_1$ such that 
% 	\begin{align*}
% 		\cG(\bL + U, \bm{\xi}) = \bm{\xi}^T\bP_{\bL + U}\bm{\xi} \leq sC_m \EE_{\bm{\xi}} [\bm{\xi}^T\bm{\xi}]~ \|\bP_{\bL + U}\| \leq sC_mc_{1}.
% 	\end{align*}
% 	Therefore, as $\|U\|_F = r_{\bL}$, we can prove the following bound
% 	\begin{align*}
% 		G_{\infty} = \frac{\tilde{d}_{\bL}}{r_{\bL}}~\sup_{\bL+U}~ \overline{\cG} \leq \frac{sC_m\tilde{d}_{\bL}c_{1}}{r_{\bL}}, \quad G_2 \leq G^2_{\infty} \leq \Big(\frac{sC_m\tilde{d}_{\bL}c_{1}}{r_{\bL}}\Big)^2.
% 	\end{align*}
% 	Substitute the bounds into the requirements of $\eta$ completes the proof of the theorem. 
% \end{proof}
 
% \begin{lemma}
% 	For an initial control gain matrix $\bK_0 \in \cK$, there exists a smoothing radius 
% 	\begin{align}
% 		r_{\bK} \leq \min \Big\{ \bB_{\bK}, \frac{\lambda_{\min}(\bR^w - \bD^T\bP_{\bK_0}\bD)}{\|\bD\|_F^2\bB_{\bP}} \Big\}
% 	\end{align} 
% 	such that $\bK_0 + r_{\bK}U_i \in \cK$, $\|U_i\|_F = 1$.
% \end{lemma}
% \begin{proof}
% 	For $\bK_0$ initialized within the set $\cK$, we have $\lambda_{\min}(\bR^w - \bD^T\bP_{\bK_0}\bD) :=X > 0$. Then, suppose $\bK' = \bK_0 + r_{\bK}U$, where $\|U\|_F = 1$, Lemma \ref{lemma:riccati_perturb} suggests that if 
% 	\begin{align*}
% 		\|\bK' - \bK_0\|_F = r_{\bK} \leq \min \Big\{ \bB_{\bK}, \frac{X}{\|\bD\|_F^2\bB_{\bP}} \Big\}, 
% 	\end{align*}
% 	then $\|\bP_{\bK'} - \bP_{\bK_0}\|_F \leq \frac{X}{\|\bD\|_F^2}$ holds, which leads to the condition
% 	\begin{align*}
% 		\|\bD^T(\bP_{\bK'} - \bP_{\bK_0})\bD\| \leq \|\bD^T(\bP_{\bK'} - \bP_{\bK_0})\bD\|_F \leq \|\bD\|_F^2\|\bP_{\bK'} - \bP_{\bK_0}\|_F \leq  X.
% 	\end{align*}
% 	This condition is sufficient to derive 
% 	\begin{align*}
% 		\bD^T(\bP_{\bK'} - \bP_{\bK_0})\bD \leq X\bI \Rightarrow \bD^T\bP_{\bK'}\bD \leq \bD^T\bP_{\bK_0}\bD +X\bI\Rightarrow \bR^w - \bD^T\bP_{\bK'}\bD >0.
% 	\end{align*}
% 	Therefore, $\bK' \in \cK$ is guaranteed, which completes the proof.
% \end{proof}
% 
% \begin{lemma}(Riccati Perturbation)\label{lemma:riccati_perturb}
% 	For any control gain matrix $\bK, \bK' \in \cK$, there exists some constant $\cB_{\bK} > 0$ such that if $\|\bK' - \bK\|_F \leq \cB_{\bK}$, the inequlity
% 	\begin{align}
% 		\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \cB_{\bP}\|\bK'-\bK\|_F
% 	\end{align}
% 	holds for some constant $\cB_{\bP}>0$.
% \end{lemma}
%% \xzedit{Whether Sun98 can be applied. Here, the inner loop player solves a Riccati equation with indefinite Q matrix. but for a given $\bK$, $\bP_{\bK} > 0$.}
% \begin{proof}
% 	The proof mostly follows from Proposition B.1 of \cite{zhang2019policy}. First of all, for a given $\bK \in \cK$, there exists $\bP_{\bK} \geq 0$ that solves the Riccati equation for the inner loop minimization problem with transition matrix $\tilde{\bA}_{\bK} = \bA-\bB\bK$ and state-weighting matrix $\tilde{\bQ} = -\bQ - \bK^T\bR^u\bK$. Recall that $\bL(\bK) = (-\bR^w + \bD\bP_{\bK}\bD)^{-1}\bD^T\bP_{\bK}\tilde{\bA}_{\bK}$, we have
% 	\begin{align*}
% 		\tilde{\bA}_{\bK} - \bD\bL(\bK) = \tilde{\bA}_{\bK} + \bD(\bR^w - \bD^T\bP_{\bK}\bD)^{-1}\bD^T\bP_{\bK}\tilde{\bA}_{\bK} = [\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\tilde{\bA}_{\bK},
% 	\end{align*}
% 	where the last equality comes from the matrix inversion lemma. Then, we let $\Delta = \bK'-\bK$ and follow page 44 of \cite{zhang2019policy} to define the following quantities
% 	\begin{align*}
% 		&\delta = \|\tilde{\bA}_{\bK'} - \tilde{\bA}_{\bK}\| = \|\bB\Delta\|_F, \quad f = \|[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\|_F, \quad g = \|\bD(\bR^w)^{-1}\bD\|_F \\
% 		&\phi = \|[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\tilde{\bA}_{\bK}\|_F, \quad \gamma = f\delta(2\phi + f\delta), \quad \psi = \|\bP_{\bK}[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\|_F \\
% 		&T_{\bK} = \bI - \big[\tilde{\bA}_{\bK} - \bD\bL(\bK)\big]^T\otimes\big[\tilde{\bA}_{\bK} - \bD\bL(\bK)\big]^T, \quad l = \|T_{\bK}^{-1}\|^{-1}_F, \quad H = \bP_{\bK}[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\tilde{\bA}_{\bK} \\
% 		&p = \big\|T_{\bK}^{-1}\big[\bI \otimes H^T + (H^T \otimes \bI)\Pi\big]\big\|_F, \quad \epsilon = \frac{1}{l}\big\|\Delta^T\bR^u\bK + \bK^T\bR^u\Delta + \Delta^T\bR^u\Delta\big\|_F + \big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \\
% 		&\alpha = f(\|\tilde{\bA}_{\bK}\|_F + \|\bB\Delta\|_F), \quad \theta = \frac{l}{\phi + \sqrt{\phi^2 + l}},
% 	\end{align*}
% 	where $\Pi$ is the vec-perturbation matrix. Here, $l$ is finite and uniformly bounded above zero because $\tilde{\bA}_{\bK} - \bD\bL(\bK)$ is actually concatenation of blocks. Then, we require the following sufficient conditions to hold \cite{sun1998perturbation, zhang2019policy}
% 	\begin{align}\label{eqn:perturb_conditions}
% 		1-fg\xi_* \geq 0, \quad \frac{f\delta+\phi fg\xi_*}{1-fg\xi_*} \leq \theta
% 	\end{align}
% 	where $\xi_* = (2l\epsilon)\cdot(l/2 + lfg\epsilon)^{-1}$. Additionally, we require
% 	\begin{align}\label{eqn:gamma}
% 		\gamma = f\delta(2\phi + f\delta) &\leq f\|\bB\Delta\|_F(2\phi+2l+f\|\bB\Delta\|_F) \nonumber\\
% 		&\leq 2f(\phi+l)\|\bB\|_F\|\Delta\|_F + f^2\|\bB\|_F^2\|\Delta\|_F^2 \leq l/2
% 	\end{align}
% 	and 
% 	\begin{align}\label{eqn:epsilon}
% 		\epsilon &= \frac{1}{l}\big\|\Delta^T\bR^u\bK + \bK^T\bR^u\Delta + \Delta^T\bR^u\Delta\big\|_F + \big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \nonumber\\
% 		&\leq \frac{1}{l}\big(2\|\bR^u\bK\|_F\|\Delta\|_F + \|\bR^u\|_F\|\Delta\|_F^2\big) + \big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \leq \frac{(l/2)^2}{2lfg(l+2a)} = \frac{l}{8fg(l+2a)}.
% 	\end{align}
% 	Then, as $\gamma \leq l/2$, we can further have
% 	\begin{align}
% 		\frac{(l/2)^2}{2lfg(l+2a)} \leq \frac{(l-\gamma)^2}{lfg(l-\gamma+2\alpha + \sqrt{(l-\gamma+2\alpha)^2-(l-\gamma)^2})}.
% 	\end{align}
% 	This implies the condition (4.41) of \cite{sun1998perturbation} holds. Therefore, Theorem 4.1 of \cite{sun1998perturbation} suggests that 
% 	\begin{align}\label{eqn:pk_bound}
% 		\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \xi_* &= \frac{2l\epsilon}{l/2 + lfg\epsilon} \leq 4\epsilon = \frac{4}{l}\big\|\Delta^T\bR^u\bK + \bK^T\bR^u\Delta + \Delta^T\bR^u\Delta\big\|_F+ 4\big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \nonumber\\
% 		&\leq \frac{8}{l}\|\bR^u\bK\|_F\|\Delta\|_F + \frac{4}{l}\|\bR^u\|_F\|\Delta\|_F^2 + 4p\|\bB\|_F\|\Delta\|_F +4\frac{\psi}{l}\|\bB\|_F^2\|\Delta\|_F^2
%    \end{align}
%    Then, following the proof of Proposition 1 in \cite{zhang2019policy}, we can have the sufficient conditions of \eqref{eqn:perturb_conditions}, \eqref{eqn:gamma}, and \eqref{eqn:epsilon} such that \eqref{eqn:pk_bound} is satisfied. This sufficient condition can be represented as
%%    \begin{align}
%%    	fg\frac{2\epsilon}{1/2 + fg\epsilon} \leq \Rightarrow fg\epsilon \leq 1/2, \quad f\delta + (\phi+\theta)fg\xi_* \leq \theta
%%    \end{align}
%%    where one sufficient condition for the second one to hold is 
%%    \begin{align}\label{eqn:condition1}
%%    	f\delta + 4(\phi+\theta)fg\epsilon \leq \theta,
%%    \end{align}
%%    as $\xi_* \leq 2\epsilon/(1/2) = 4\epsilon$. Since $f\delta\geq 0$ and $fg\epsilon \geq 0$, \eqref{eqn:condition1} implies that $fg\epsilon \leq 1/2$. For \eqref{eqn:condition1} to hold, we can let
%%    \begin{align}
%%    	f\|\bB\|\|\Delta\| + 4(\phi+\theta)fg\big(\frac{2}{l}\|\bR^u\bK\|\|\Delta\| + \frac{1}{l}\|\bR^u\|\|\Delta\|^2 + p\|\bB\|\|\Delta\| + \frac{\psi}{l}\|\bB\|^2\|\Delta\|^2\big) \leq \theta,
%%    \end{align}
%%    which can be satisfied by choosing $\|\Delta\|$ such that
%%    \begin{align}
%%    	\hspace{-0.5em}\|\Delta\| \leq \min\Big\{\frac{\|\bB\| + 4(\phi+\theta)g(2\|\bR^u\bK\|/l + p\|\bB\|)}{4(\phi+\theta)g(\|\bR^u\|/l + \psi\|\bB\|^2/l)}, \frac{\theta}{2f\|\bB\|+8f(\phi+\theta)g(2\|\bR^u\bK\|/l + p\|\bB\|)}\Big\}
%%    \end{align}
%%    Subsequently, \eqref{eqn:gamma} gives
%%    \begin{align}
%%    	2f(\phi + l)\|\bB\|\|\Delta\| + f^2\|\bB\|^2\|\Delta\|^2 \leq l/2,
%%    \end{align}
%%    which can be satisfied by choosing $\|\Delta\|$ such that
%%     \begin{align}
%%    	\|\Delta\| \leq \min\Big\{\frac{2(\phi+l)}{f\|\bB\|}, \frac{l}{8f(\phi+l)\|\bB\|}\Big\}
%%    \end{align}
%%    \xzedit{maybe should just cite the result}
%%    The three conditions can be satisfied by choosing
%    \begin{align}
%    	\hspace{-0.5em}\|\Delta\|_F \leq \min\Big\{1, \frac{2\|\bR^u\bK\|_F + (p+1)l\|\bB\|_F}{\|\bR^u\|_F + \psi\|\bB\|_F^2}, \frac{l}{16fg[l+2f(\|\tilde{\bA}_{\bK}\|_F + \|\bB\|_F)](\|\bR^u\bK\|_F/l + 2(p+1)\|\bB\|_F)}\Big\}
%    \end{align}
%    Under this condition, the perturbation of the Riccati equation can be bounded by
%    \begin{align}
%    	\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \Big[\frac{\|\bB\|_F}{(\psi+\theta)g} + \frac{16\|\bR^u\bK\|_F}{l} + 8p\|\bB\|_F\Big] \cdot\|\Delta\|_F
%    \end{align}
%    Therefore, there exists some $\cB_{\bK} >0$ and $\cB_{\bP} = \frac{\|\bB\|_F}{(\psi+\theta)g} + \frac{16\|\bR^u\bK\|_F}{l} + 8p\|\bB\|_F$ such that $\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \cB_{\bP}\|\bK'-\bK\|_F$ for $\bK', \bK \in \cK$ and $\|\bK' - \bK\|_F \leq \cB_{\bK}$. This completes the proof.
% \end{proof}
 
% \begin{lemma}(Local Lipschitz and Smooth)
% 	For $\bK, \bK' \in \cK$ and let the inequality  \xznote{Do we actually need smoothness}
% 	\begin{align}\label{eqn:lipschitz_bound}
% 		\|\bK' - \bK\|_F \leq \cB_{\bK}
% 	\end{align}
% 	holds. Then, we have
% 	\begin{align}\label{eqn:out_lipschitz}
% 		|\cG(\bK') - \cG(\bK)| &\leq l_{\bK}\|\bK'-\bK\|_F \\
% 		\|\nabla\cG(\bK') -\nabla\cG(\bK)\|_F &\leq \psi_{\bK}\|\bK'-\bK\|_F \label{eqn:out_smooth} 
% 	\end{align}
% \end{lemma}
% \begin{proof}
% 	By definition, 
% 	\begin{align}
% 		|\cG(\bK') - \cG(\bK)| = \Tr(\bP_{\bK'}) - \Tr(\bP_{\bK}) \leq s\|\bP_{\bK'} - \bP_{\bK}\| \leq s\|\bP_{\bK'} - \bP_{\bK}\|_F.
% 	\end{align}
% 	Applying Lemma \ref{lemma:riccati_perturb} and the condition \eqref{eqn:lipschitz_bound} yields
% 	\begin{align}
% 		\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \bB_{\bP}\|\bK'-\bK\|_F.
% 	\end{align}
% 	Therefore, substituting $l_{\bK} = s\cB_{\bP}$ completes the proof of \eqref{eqn:out_lipschitz}. Next, we focus on showing \eqref{eqn:out_smooth}. First, we invoke Lemma 13 of \cite{fazel2018global} to obtain
% 	\begin{align}
% 		\|\bP_{\bK}\| \leq \cG(\bK).
% 	\end{align}
% 	Next, because that $\Sigma_{\bK}$ is the solution of the Lyapunov equation
%	\begin{align*}
%		\Sigma_{\bK} = \bA_{\bK, \bL}\Sigma_{\bK} \bA_{\bK, \bL}^T + \Sigma_0,
%	\end{align*} 
%	where $\Sigma_0 = \EE[\bm{\xi}\bm{\xi}^T]$ and $\|\bm{\xi}\|^2 \leq sC_m$ almost surely due to the assumption on the distribution $\cD$. Since $\Sigma_{\bK}$ can be solved iteratively via 
%	\begin{align*}
%		\Sigma_{\bK} = \sum^{N}_{t=0}\big(\bA_{\bK, \bL}\big)^{t}\Sigma_{0} \big(\bA_{\bK, \bL}^T\big)^t,
%	\end{align*}
%	we can bound $\|\Sigma_{\bK}\|$ by $\|\Sigma_{\bK}\| \leq sNC_m$. Subsequently, by the gradient formula in Lemma \ref{lemma:exact_PG_K} and suppose \eqref{eqn:lipschitz_bound} is enforced, we have
%	\begin{align}
%		\|\nabla\cG(\bK') - \nabla\cG(\bK)\|_F &= \|(\bE_{\bK'} - \bE_{\bK})\Sigma_{\bK'} + \bE_{\bK}(\Sigma_{\bK'} - \Sigma_{\bK})\|_F \\
%		&\leq \|\bE_{\bK'} - \bE_{\bK}\|_F\|\Sigma_{\bK'}\| + \|\bE_{\bK}\|_F\|\Sigma_{\bK'} - \Sigma_{\bK}\| \\
%		&\leq 
%	\end{align}
%	
%	\begin{align*}
%		\|\bE_{\bK'} - \bE_{\bK}\|_F &= 2\|(\bR^u + \bB^T\tilde{\bP}_{\bK'}\bB)\bK -\bB^T\tilde{\bP}_{\bK'}\bA - (\bR^u + \bB^T\tilde{\bP}_{\bK}\bB)\bK + \bB^T\tilde{\bP}_{\bK}\bA\|_F \\
%		&\hspace{-2em}\leq 2\|\bR^u(\bK'-\bK) + \bB^T(\tilde{\bP}_{\bK'} - \tilde{\bP}_{\bK})\bB\bK' + \bB^T\tilde{\bP}_{\bK}\bB(\bK'-\bK) - \bB^T(\tilde{\bP}_{\bK'} -\tilde{\bP}_{\bK})\bA\|_F\\
%		&\hspace{-2em}\leq 2\|\bR^u\|_F\|\bK'-\bK\|_F + 2\|\bB^T(\tilde{\bP}_{\bK'}- \tilde{\bP}_{\bK})\bB\bK'\|_F + 2\|\bB^T\tilde{\bP}_{\bK}\bB(\bK'-\bK)\|_F + 2\|\bB^T(\tilde{\bP}_{\bK'} -\tilde{\bP}_{\bK})\bA\|_F
%	\end{align*}
%	\begin{align*}
%		\|\tilde{\bP}_{\bK'}- \tilde{\bP}_{\bK}\|_F &= \|\bP_{\bK'} - \bP_{\bK} + \bP_{\bK'}\bD(\bR^w - \bD^T\bP_{\bK'}\bD)^{-1}\bD^T\bP_{\bK'}  - \bP_{\bK}\bD(\bR^w - \bD^T\bP_{\bK}\bD)^{-1}\bD^T\bP_{\bK}\|_F\\
%		&\leq \|\bP_{\bK'} - \bP_{\bK}\|_F + \|\|_F
%	\end{align*}
% \end{proof}

 
 % Backup
% \begin{proof}
% 	For the ease of notation, we first define the set $\cS_{\bL_{10}} := \big\{\bL \mid \cG(\bL) - \cG(\bL^*) \leq 10\delta^{-1}\Delta_0\big\}$, where $\Delta_l = \cG(\bL_l) - \cG(\bL^*)$ is the optimality gap between the control gain matrix $\bL_l$ at iteration $l$ and the optimal control gain matrix $\bL^*$. Also, we define
% 	\begin{align*}
% 		G_{\infty} := \sup_{\bL \in \cS_{\bL_{10}}} \|\nabla\cG(\bL)\|, \quad G_2 := \sup_{\bL \in \cS_{\bL_{10}}} \EE~\Big[\big\|\nabla\cG(\bL) - \EE~\big[\nabla\cG(\bL) \mid \bL\big]\big\|^2\Big]
% 	\end{align*}
% 	as the uniform bounds on the gradient norm and its variance, respectively. Subsequently, let $\iota := \min\big\{l\mid \Delta_{l} > 10\delta^{-1}\Delta_0\big\}$ to denote the first iteration index where the iterates exits the sublevel set $\cS_{\bL_{10}}$. Then, we provide the following helper lemma with its proof deferred for smoother reading.
% \begin{lemma}\label{lemma:Deltabound}
% Let the algorithm parameters are chosen to satisfy \eqref{eqn:one_point_req}. Then, for any iteration index $l$ such that $\bL_l \in \cS_{\bL_{10}}$, we have
% \begin{align*}
% 	\EE_l[\Delta_{l+1}] \leq (1-\frac{\eta c_g}{4})\Delta_l + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta c_g \frac{\epsilon_{\bL}\delta}{20},
% \end{align*}
% where $\EE_l[\Delta_{l}]$ denotes the expectation of the optimality gap at iteration $l$. 
% \end{lemma}
%
% With the helper lemma above, we first show that if \eqref{eqn:one_point_req} is satisfied, then we will have 
% 	\begin{align}\label{eqn:intermediate_E}
% 		\EE[\Delta_{\cL} 1_{\iota > \cL}] \leq \frac{\epsilon_{\bL}\delta}{2}.
% 	\end{align}
% 	and $\iota > \cL$ with probability greater than $1-\frac{\delta}{2}$. To start with, we separate the proof into two cases. In the case where $\iota > \cL$, Lemma \ref{lemma:Deltabound} can be applied to to bound $\EE_l[\Delta_{l+1}]$. In the case where $\iota \leq \cL$, it is straightforward to see that $\EE_{l}[\Delta_{l+1}]1_{\iota > \cL} = 0$. Combining these two case with $\eta \leq \frac{\epsilon_{\bL} c_g\delta}{40\psi_{\bL} G_2}$ yields
% 	\begin{align*}
% 		\EE [\Delta_{l+1}1_{\iota > l+1}] &\leq \Big(1-\frac{\eta}{ c_g}\Big)^{l+1}\Delta_0 + \Big(\frac{\psi_{\bL}\eta^2G_2}{2} + \frac{\eta c_g \epsilon_{\bL}\delta}{20}\Big)\sum^{l}_{i=0}\Big(1 - \frac{\eta c_g}{4}\Big)^i \\
% 		&\leq \Big(1-\frac{\eta}{ c_g}\Big)^{l+1}\Delta_0 + \frac{2\psi_{\bL}\eta G_2}{c_g} + \frac{\epsilon_{\bL}\delta}{5} \\
% 		& \leq \Big(1-\frac{\eta}{ c_g}\Big)^{l+1}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4}.
%  	\end{align*}
%  	Let $\cL = l+1$, we can verify that if $\cL = \frac{4}{\eta c_g}\log(\frac{4\Delta_0}{\delta\epsilon_{\bL}})$, then
%  	\begin{align*}
%  		\Big(1-\frac{\eta}{ c_g}\Big)^{\cL}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4} \leq \frac{\epsilon_{\bL}\delta}{2}.
%  	\end{align*}
%  	This leads to $\EE[\Delta_{\cL} 1_{\iota > \cL}] \leq \frac{\epsilon_{\bL}\delta}{2}$. It remains to show that the event $\iota \leq \cL$ happens with a probability lower than $\frac{\delta}{2}$. Then, for $l \in [\cL]$, we denote the stopped process
% 	\begin{align*}
% 		Y_l = \Delta_{\min(\iota, l)} + (\cL - l)\big(\frac{\eta^2\psi_{\bL}}{2}G_2 + \frac{\eta c_g\epsilon_{\bL}\delta}{20}\big).
% 	\end{align*}
% 	Following from \cite{malik2020derivative}, the stopped process sequence $Y_l$ is a super-martingale such that
% 	 \begin{align*}
% 		\EE_l[Y_{l+1}] \leq Y_{l}.
% 	\end{align*}
% 	Then, if $\epsilon_{\bL}$ is small enough to satisfy $\epsilon_{\bL} \log(\frac{4\Delta_0}{\delta\epsilon_{\bL}}) \leq \frac{16}{\delta}\Delta_0$, we can obtain
% 	\begin{align*}
% 		P \big\{\max_{l \in [\cL]} Y_l \geq 10\delta^{-1}\Delta_0\big\} &\leq \frac{\EE[Y_0]}{10\delta^{-1}\Delta_0} \\
% 		& = \frac{1}{10\delta^{-1}\Delta_0}\bigg(\Delta_0 + \cL\Big(\frac{\psi_{\bL}\eta^2}{2}G_2 + \frac{\eta\epsilon_{\bL} c_g \delta}{20}\Big)\bigg) \\
% 		& \leq \frac{1}{10\delta^{-1}\Delta_0}\bigg(\Delta_0 + \frac{2}{c_g}\log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big)\psi_{\bL}\eta G_2 + \log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big)\frac{\epsilon_{\bL}\delta}{5}\bigg)\\
% 		& \leq \frac{1}{10\delta^{-1}\Delta_0}\bigg(\Delta_0 + \frac{\delta\epsilon_{\bL}}{20}\log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big) + \frac{\epsilon_{\bL}\delta}{5}\log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big)\bigg) \\
% 		&\leq \frac{\delta}{10\Delta_0}(5\Delta_0) = \frac{\delta}{2}.
% 	\end{align*}
% 	This completes the proof of \eqref{eqn:intermediate_E}. Moreover, this leads to
% 	\begin{align*}
% 		P\{\Delta_\cL \geq \epsilon_{\bL}\} &\leq P\{\Delta_{\cL}1_{\iota>\cL} \geq \epsilon_{\bL}\} + P\{1_{\iota \leq \cL}\}  \leq \frac{1}{\epsilon_{\bL}}\EE[\Delta_{\cL}1_{\iota>\cL}] + P\{1_{\iota \leq \cL}\} \leq \delta,
% 	\end{align*}
% 	which implies $P\{\Delta_\cL \leq \epsilon_{\bL}\} > 1- \delta$. Lastly, we provide bounds for $G_2$ and $G_{\infty}$. By definition of the cost function, if $r \leq \frac{10\delta^{-1}\cG(\bL_0)}{l_{\bL}}$ and $\|U\|_F = r_{\bL}$, then we will have
% 	\begin{align*}
% 		\cG(\bL + U, \bm{\xi}) = \bm{\xi}^T\bP_{\bL + U}\bm{\xi} \leq sC_m \EE_{\bm{\xi}} [\bm{\xi}^T\bP_{\bL + U}\bm{\xi}] &= sC_m\cG(\bL + U)\leq 20\delta^{-1}sC_m\cG(\bL_0).
% 	\end{align*}
% 	Therefore, 
% 	\begin{align*}
% 		G_{\infty} = \frac{\tilde{d}_{\bL}}{r_{\bL}}\sup_{\bL+U \in \cS_{\bL_{10}}} \overline{\cG} \leq \frac{20\delta^{-1}\tilde{d}_{\bL}sC_m}{r_{\bL}}\cG(\bL_0), \quad G_2 \leq G^2_{\infty} \leq \Big(\frac{20\delta^{-1}\tilde{d}_{\bL}sC_m}{r_{\bL}}\cG(\bL_0)\Big)^2.
% 	\end{align*}
% 	Substitute the bounds into the requirements of $\eta$ completes the proof of the theorem. Lastly, we focus on proving the helper Lemma \eqref{lemma:Deltabound}.
% 	From page 24 of \cite{malik2020derivative}, we have
% 	\begin{align*}
% 		\EE_l[\Delta_{l+1} - \Delta_l] \leq - \frac{\eta c_g}{2}\Delta_l + \frac{\eta c_g}{4}\Delta_l + 4\frac{\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta^2\psi_{\bL}^3r_{\bL}^2,
% 	\end{align*}
% 	where $\theta_{\bL} = \min\{\frac{1}{2\psi_{\bL}}, \frac{1}{\lambda}\}$. Since \eqref{eqn:one_point_req} is satisfied, we can derive that $\frac{4\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$ and $\eta^2\psi_{\bL}^3r_{\bL}^2 \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$. This completes the proof.
% \end{proof}


==> Mixed Design Arxiv v3/formulation.tex <==
For ease of analysis, we first present the following compact notations for the game.
\small
\begin{align}
&\bx = \big[x^{\top}_0, \cdots, x^{\top}_{N}\big]^{\top}, ~~~\ \bu = \big[u^{\top}_0, \cdots, u^{\top}_{N-1}\big]^{\top}, ~~~\ \bw = \big[w^{\top}_0, \cdots, w^{\top}_{N-1}\big]^{\top}, ~~~\ \bm{\xi} = \big[x^{\top}_0, ~\xi^{\top}_0, \cdots, \xi^{\top}_{N-1}\big]^{\top}, ~~~\ \bQ = \big[diag(Q_0, \cdots, Q_N)\big],\nonumber\\
&\bA = \begin{bmatrix} \bm{0}_{m\times mN} &  \bm{0}_{m\times m} \\ diag(A_0, \cdots, A_{N-1}) & \bm{0}_{mN\times m}\end{bmatrix}, \
\bB = \begin{bmatrix} \bm{0}_{m\times dN} \\ diag(B_0, \cdots, B_{N-1}) \end{bmatrix}, \ \bD = \begin{bmatrix} \bm{0}_{m\times nN} \\ diag(D_0, \cdots, D_{N-1}) \end{bmatrix}, \  \bR^u = \big[diag(R^u_0, \cdots, R^u_{N-1})\big], \nonumber \\
&\bR^w = \big[diag(R^w_0, \cdots, R^w_{N-1})\big], \qquad \bK = \begin{bmatrix} diag(K_0, \cdots, K_{N-1}) & \bm{0}_{dN\times m} \end{bmatrix}, \qquad \bL = \begin{bmatrix} diag(L_0, \cdots, L_{N-1}) & \bm{0}_{nN\times m} \end{bmatrix}. \label{eqn:KL_form}
\end{align}
\normalsize
We re-derive the earlier game formulation with linear state-feedback policies for the players using compact notations in \S\ref{sec:compact_forms} and show that they are equivalent to the recursive ones in \S\ref{sec:game}. Now, using the compact notations, we develop PG methods with access to the \emph{exact} policy gradient that provably converges to the Nash equilibrium of the game, $(\bK^*, \bL^*) \in \cS(d, m, N) \times \cS(n, m, N)$, where $\cS(d, m, N)$ and $\cS(n, m, N)$ are the subspaces that we confine our searches of $\bK$ and $\bL$ to, respectively. In particular, we only search over $\bK \in \RR^{Nd \times (N+1)m}$ and $\bL \in \RR^{Nn \times (N+1)m}$, and $\bK, \bL$ satisfy the sparsity patterns shown in \eqref{eqn:KL_form}, as they suffice to attain the Nash equilibrium. The degrees of freedom of  $\cS(d, m, N)$ and $\cS(n, m, N)$ are $d\times m\times N $ and $n\times m \times N$, respectively. Then, for any pair of gains $(\bK, \bL)$, the objective function $\cG(\bK, \bL)$ is given by
\begin{align}\label{eqn:ckl}
	\cG(\bK, \bL) = \EE_{\bm{\xi}}\big[\bm{\xi}^{\top}\bP_{\bK, \bL}\bm{\xi}\big] = \Tr\big(\bP_{\bK, \bL}\Sigma_0\big) = \Tr\big((\bQ + \bK^{\top}\bR^u\bK - \bL^{\top}\bR^w\bL)\Sigma_{\bK, \bL}\big), 
\end{align} 
where $\bP_{\bK, \bL}\hspace{-0.2em}:=\hspace{-0.15em}diag(P_{K_0, L_0}, \cdots, P_{K_N, L_N})$ and $P_{K_t, L_t}$ is the solution to the recursive Lyapunov equation
\begin{align}\label{eqn:pkl_recursive}
	P_{K_t, L_t} = (A_t -B_tK_t -D_tL_t)^{\top}P_{K_{t+1}, L_{t+1}}(A_t-B_tK_t-D_tL_t) + Q_t + K_t^{\top}R^u_tK_t -L_t^{\top}R^w_tL_t, \ t \in \{0, \cdots, N-1\}
\end{align}
with $P_{K_N, L_N}:= \hspace{-0.1em}Q_N$. Moreover, $\bP_{\bK, \bL}$ and $\Sigma_{\bK, \bL} := \EE_{x_0, \xi_0, \cdots, \xi_{N-1}}\left[diag(x_0x_0^{\top}, \cdots, x_Nx_N^{\top})\right]$ are the solutions to the recursive Lyapunov equations in the compact form
\begin{align}
	\label{eqn:bpkl}
	\bP_{\bK, \bL} &= (\bA -\bB\bK -\bD\bL)^{\top}\bP_{\bK, \bL}(\bA-\bB\bK-\bD\bL) + \bQ + \bK^{\top}\bR^u\bK -\bL^{\top}\bR^w\bL \\
	\Sigma_{\bK, \bL} &= (\bA -\bB\bK-\bD\bL)\Sigma_{\bK, \bL}(\bA -\bB\bK-\bD\bL)^{\top} + \Sigma_0,\label{eqn:sigmaKL}
\end{align}
where $\Sigma_0 := \EE_{x_0, \xi_0, \cdots, \xi_{N-1}}\left[diag(x_0x_0^{\top}, \xi_0\xi_0^{\top}, \cdots, \xi_{N-1}\xi_{N-1}^{\top})\right] > 0$ is full-rank because $x_0, \xi_0, \cdots, \xi_{N-1}$ are drawn independently from distribution $\cD$ that has a positive-definite covariance. The solutions to \eqref{eqn:bpkl} and \eqref{eqn:sigmaKL} always exist and are unique because they are essentially recursive formulas in blocks. Since $\|x_0\|, \|\xi_t\| \leq \vartheta$ almost surely, for all $t\in \{0, \cdots, N-1\}$, $\big\|diag(x_0x_0^{\top}, \xi_0\xi_0^{\top}, \cdots, \xi_{N-1}\xi_{N-1}^{\top})\big\|_F \leq c_0 :=(N+1)\vartheta^2$ almost surely. Moreover, we define $d_{\Sigma}:=m^2(N+1)$ and $\phi:=\lambda_{\min}(\Sigma_0) > 0$ that will be useful in our analysis.

Our goal is to solve the minimax optimization problem $\min_{\bK}\max_{\bL} \cG(\bK, \bL)$ such that $\cG(\bK^*, \bL) \leq \cG(\bK^*, \bL^*) \leq \cG(\bK, \bL^*)$ for any $\bK$ and $\bL$, where $(\bK^*, \bL^*)$  is the saddle-point (equivalently, Nash equilibrium) solution. In the following lemmas, we show that $\cG(\bK, \bL)$ is \emph{nonconvex-nonconcave}, and also provide explicit forms of the PGs of $\cG(\bK, \bL)$. Lastly, we show that the stationary point of $\cG(\bK, \bL)$ captures the Nash equilibrium of the game under standard regularity conditions. Proofs of the two lemmas are deferred to   \S\ref{proof:nonconvex_nonconcave} and \S\ref{proof:station}, respectively.

\begin{lemma}(Nonconvexity-Nonconcavity)\label{lemma:nonconvex_nonconcave}
	There exist zero-sum LQ dynamic games such that the objective function $\cG(\bK, \bL)$ is nonconcave in $\bL$ for a fixed $\bK$, and nonconvex in $\bK$ for a fixed $\bL$.
\end{lemma}

\begin{lemma}({PG} \& Stationary Point Property)\label{lemma:station}
The policy gradients of $\cG(\bK, \bL)$ can be computed as
\begin{align}  
	 \nabla_{\bK}\cG(\bK, \bL) & = 2\bF_{\bK, \bL}\Sigma_{\bK, \bL} := 2\big[(\bR^u + \bB^{\top}\bP_{\bK, \bL}\bB)\bK - \bB^{\top}\bP_{\bK, \bL}(\bA-\bD\bL)\big] \Sigma_{\bK, \bL}, \label{eqn:nabla_K}\\
	 \nabla_{\bL}\cG(\bK, \bL) & = 2\bE_{\bK, \bL}\Sigma_{\bK, \bL} := 2\big[(-\bR^w + \bD^{\top}\bP_{\bK, \bL}\bD)\bL - \bD^{\top}\bP_{\bK, \bL}(\bA-\bB\bK)\big] \Sigma_{\bK, \bL}. \label{eqn:nabla_L}
\end{align}	
Also, if at some stationary point $(\bK,\bL)$ of $\cG(\bK, \bL)$ (i.e., where  $\nabla_{\bK}\cG(\bK, \bL)=\bm{0}$ and $\nabla_{\bL}\cG(\bK, \bL) = \bm{0}$), it holds that $\bP_{\bK,\bL}\geq 0$ and $\bR^w - \bD^{\top}\bP_{\bK, \bL}\bD > 0$, then this stationary point $(\bK,\bL)$ is the unique Nash equilibrium of the game.
\end{lemma}

\subsection{Double-Loop Scheme}\label{sec:double_loop_scheme}
We start by introducing our  \emph{double-loop} update scheme.  Specifically, we first fix an outer-loop control gain matrix $\bK$, and solve for the optimal $\bL$ by maximizing the objective $\cG(\bK,\cdot)$ over $\bL\in \cS(n, m, N)$. We denote the inner-loop solution for a fixed  $\bK$, if exists, by $\bL(\bK)$. After obtaining the inner-loop solution, the outer-loop $\bK$ is then updated to minimize the objective $\cG(\bK, \bL(\bK))$ over $\bK\in\cS(d, m, N)$}. For each fixed $\bK$, the inner-loop is an \emph{indefinite}  LQR problem where the state-weighting matrix, i.e., $-\bQ-\bK^{\top}\bR^u\bK$, is not p.s.d. Our goal is to find, via PG methods, the optimal linear state-feedback controller $\bw(\bK) = -\bL(\bK)\bx$, which suffices to attain the optimal performance for the inner loop, whenever the objective function $\cG(\bK,\cdot)$ admits a finite upper bound value (depending on the choice of the outer-loop $\bK$). We formally state the precise condition for the solution to the inner-loop maximization problem to be \emph{well-defined} as follows, with its proof being deferred to \S\ref{proof:assumption_L}. 

\begin{lemma}\label{lemma:assumption_L}(Inner-Loop Well-Definedness Condition)
For the Riccati equation
		\begin{align}\label{eqn:DARE_black_L}
			\bP_{\bK, \bL(\bK)} = \bQ + \bK^{\top}\bR^u\bK + (\bA-\bB\bK)^{\top}\big(\bP_{\bK, \bL(\bK)}+\bP_{\bK, \bL(\bK)}\bD(\bR^w - \bD^{\top}\bP_{\bK, \bL(\bK)}\bD)^{-1}\bD^{\top}\bP_{\bK, \bL(\bK)}\big)(\bA-\bB\bK),
\end{align}
we define the feasible set of control gain matrices $\bK$ to be
	\begin{align}\label{eqn:set_ck}
		\cK := \big\{\bK \in \cS(d, m, N) \mid \eqref{eqn:DARE_black_L} \text{ admits a solution } \bP_{\bK, \bL(\bK)}\geq 0, \text{~and } \bR^w - \bD^{\top}\bP_{\bK, \bL(\bK)}\bD > 0\big\}.
    \end{align}
  Then, $\bK \in \cK$ is \emph{sufficient} for the inner-loop solution $\bL(\bK)$ to be well defined. Also, $\bL(\bK)$ is unique, and takes the form of:
\begin{align}\label{eqn:l_k}
	\bL(\bK) = (-\bR^w + \bD^{\top}\bP_{\bK, \bL(\bK)}\bD)^{-1}\bD^{\top}\bP_{\bK, \bL(\bK)}(\bA-\bB\bK).
\end{align}
Moreover, $\bK \in \cK$ is also \emph{almost necessary}, in that if $\bK \notin \overline{\cK}$, where 
  \begin{align}\label{eqn:set_ckbar}
  	\overline{\cK} := \big\{\bK \in \cS(d, m, N) \mid \eqref{eqn:DARE_black_L} \text{ admits a solution } \bP_{\bK, \bL(\bK)}\geq 0, \text{~and } \bR^w - \bD^{\top}\bP_{\bK, \bL(\bK)}\bD \geq 0\big\},
  \end{align}
  then the solution to the inner loop is not well defined, i.e., the objective $\cG(\bK, \cdot)$ could be driven to arbitrarily large values. Lastly, the solution to \eqref{eqn:DARE_black_L} satisfies $\bP_{\bK, \bL(\bK)} \geq \bP_{\bK, \bL}$ in the p.s.d. sense for all $\bL$.
\end{lemma} 
We note that the set $\cK$ is nonempty due to Assumption \ref{assumption_game_recursive} (as $\bK^*$ must lie in $\cK$), but it might be \emph{unbounded}. Also, every control gain matrix $\bK\in\cK$ for the outer-loop minimizing player in the game is equivalent to a control gain matrix that attains a $\gamma$-level of disturbance in the original disturbance attenuation problem  (cf. Lemma \ref{lemma:equivalent}). Then, by Lemma \ref{lemma:nonconvex_nonconcave}, the inner loop for a fixed $\bK \in \cK$ is a nonconcave optimization problem in terms of $\bL$, represented as $\max_{\bL}\cG(\bK, \bL)$. By Lemma \ref{lemma:assumption_L}, the inner loop always admits a unique maximizing solution for any $\bK\in\cK$. Thus,  the function $\max_{\bL}\cG(\bK, \bL)$ is differentiable with respect to $\bK$ and $\nabla_{\bK}\{\max_{\bL}\cG(\bK, \bL)\} = \nabla_{\bK}\cG(\bK, \bL(\bK))$ according to a variant of Danskin's theorem \cite{bernhard1995theorem}. The outer loop is then a nonconvex (as we will show in Lemma \ref{lemma:landscape_K}) constrained optimization problem in terms of $\bK$, which can be written as $\min_{\bK\in\cK}\cG(\bK, \bL(\bK))$. Note that restricting our search to $\cK$ does not lead to any loss of optimality because Assumption \ref{assumption_game_recursive} ensures that $\bK^*$ lies in $\cK$. Then, the policy gradient of the outer loop can be derived by substituting \eqref{eqn:l_k} into \eqref{eqn:nabla_K}, resulting in $\nabla_{\bK}\cG(\bK, \bL(\bK)) = 2\bF_{\bK, \bL(\bK)}\Sigma_{\bK, \bL(\bK)}$, where $\Sigma_{\bK, \bL(\bK)}$ follows from \eqref{eqn:sigmaKL} and
\begin{align}
	\bF_{\bK, \bL(\bK)} := (\bR^u + \bB^{\top}\tilde{\bP}_{\bK, \bL(\bK)}\bB)\bK - \bB^{\top}\tilde{\bP}_{\bK, \bL(\bK)}\bA, \quad \label{eqn:tilde_pk}
	\tilde{\bP}_{\bK, \bL(\bK)} := \bP_{\bK, \bL(\bK)} + \bP_{\bK, \bL(\bK)}\bD(\bR^w - \bD^{\top}\bP_{\bK, \bL(\bK)}\bD)^{-1}\bD^{\top}\bP_{\bK, \bL(\bK)}.
\end{align}
Lastly, we comment, in the next remark,  on the double-loop scheme we study, and compare it with other possible update schemes, such as alternating/simultaneous updates, that may also be candidates to solve this minimax optimization problem. 

\begin{remark}(Double-Loop Scheme)\label{remark:double}
	Our double-loop scheme, which has also  been used before in \cite{zhang2019policy,bu2019global},  is pertinent to the descent-multi-step-ascent scheme \cite{nouiehed2019solving} and the gradient descent-ascent (GDA) scheme with two-timescale stepsizes  \cite{jin2019minimax,lin2019gradient,fiez2020gradient} for solving nonconvex-(non)concave minimax optimization problems, with the number of multi-steps of ascent going to infinity, or the ratio between the fast and slow  stepsizes going to infinity (the $\tau$-GDA scheme with $\tau\to\infty$ \cite{jin2019minimax,fiez2020gradient}). Another variant is the alternating GDA (AGDA) scheme, which has been investigated in \cite{yang2020global} to address nonconvex-nonconcave problems with two-sided PL condition. However, unlike this literature,  one key condition for establishing convergence, the  \emph{global smoothness} of the objective function, does not hold in our control setting with \emph{unbounded} decision spaces and objective functions. In fact, as per Lemma \ref{lemma:assumption_L}, a non-judicious choice of $\bK$ may lead to an  undefined inner-loop maximization problem with unbounded objective. Hence, one has to carefully control the  update-rule here, to ensure that the iterates do not yield unbounded/undefined values along iterations. As we will show in \S\ref{sec:alternate}, it is not hard to construct cases where descent-multi-step-ascent/AGDA/$\tau$-GDA diverges even with infinitesimal stepsizes, similar to the negative results reported in the infinite-horizon setting in \cite{zhang2020rarl}. These results suggest that it seems challenging to provably show that other candidate update schemes converge to the global NE in  zero-sum LQ games, except the double-loop one, as we will show next. 
\end{remark}

\subsection{Optimization Landscape}\label{sec:landscape}
 
For a fixed $\bK$, the optimization landscape of the inner-loop subproblem is summarized in the following lemma, with its proof being deferred to \S\ref{proof:landscape_L}. 
\begin{lemma}(Inner-Loop Landscape)\label{lemma:landscape_L}
	There exists $\bK \in \cK$ such that $\cG(\bK, \bL)$ is nonconcave in $\bL$. For a fixed $\bK \in \cK$, $\cG(\bK, \bL)$ is coercive (i.e., $\cG(\bK, \bL) \rightarrow - \infty$ as $\|\bL\|_F \rightarrow \infty$), and the superlevel set 
	\small
\begin{align}\label{eqn:levelset_L}
		\cL_{\bK}(a) := \big\{\bL\in \cS(n, m, N) \mid \cG(\bK, \bL) \geq a\big\}
\end{align}  
\normalsize
is compact for any $a$ such that $\cL_{\bK}(a) \neq \varnothing$. Moreover, there exist some $l_{\bK, \bL}, \psi_{\bK, \bL}, \rho_{\bK, \bL} > 0$ such that $\cG(\bK,\bL)$ is $(l_{\bK, \bL}, \rho_{\bK, \bL})$ locally Lipschitz and $(\psi_{\bK, \bL}, \rho_{\bK, \bL})$ locally smooth at $(\bK, \bL)$. In other words, given any $\bL$, we have 
\begin{align*}
	\forall \bL' \text{ ~s.t.~  } \|\bL'-\bL\|_F\leq \rho_{\bK, \bL}, \quad |\cG(\bK, \bL') - \cG(\bK, \bL)| \leq l_{\bK, \bL}\cdot\|\bL' - \bL\|_F, \quad \|\nabla_{\bL}\cG(\bK, \bL') - \nabla_{\bL}\cG(\bK, \bL)\|_F \leq \psi_{\bK, \bL}\cdot\|\bL' - \bL\|_F.
\end{align*}
Also, there exist some $l_{\bK, a}, \psi_{\bK, a}> 0$ such that for any $\bL, \bL' \in \cL_{\bK}(a)$, we have
\begin{align*}
	|\cG(\bK, \bL') - \cG(\bK, \bL)| \leq l_{\bK, a}\cdot\|\bL' - \bL\|_F, \quad \|\nabla_{\bL}\cG(\bK, \bL') - \nabla_{\bL}\cG(\bK, \bL)\|_F \leq \psi_{\bK, a}\cdot\|\bL' - \bL\|_F.
\end{align*}
Lastly, the objective function $\cG(\bK, \bL)$ is $\mu_{\bK}$-PL for some $\mu_{\bK}>0$, such that $\tr (\nabla_{\bL}\cG(\bK, \bL)^{\top}\nabla_{\bL}\cG(\bK, \bL)) \geq \mu_{\bK} (\cG(\bK, \bL(\bK)) - \cG(\bK, \bL))$, where $\bL(\bK)$ is as defined in \eqref{eqn:l_k}. The PL constant $\mu_{\bK}$ depends only on $\bK$ and the problem parameters.
 \end{lemma}

The optimization landscape of the inner loop is similar to that of the standard infinite-horizon LQR problem studied in \cite{fazel2018global, bu2019LQR, malik2020derivative}. We note that in our finite-horizon setting, independent process noises (together with the random initial state) with positive-definite covariances are essential for $\Sigma_{\bK,\bL}$ to be full-rank (in contrast to only requiring a random initial state with positive-definite covariance in \cite{fazel2018global}). The full-rankness of $\Sigma_{\bK,\bL}$ further guarantees that the stationary point of the inner-loop objective function $\cG(\bK, \bL)$ is also the unique optimal solution, as suggested in Lemma \ref{lemma:station}. Furthermore, it also ensures that the inner-loop objective function $\cG(\bK, \bL)$ is PL, as shown in Lemma \ref{lemma:landscape_L}. These two properties together are the key enablers to establish  the global convergence of our double-loop method, despite the problem being nonconvex-nonconcave. 

Subsequently, we analyze the optimization landscape of the outer loop in the following lemma (proved in \S\ref{proof:landscape_K}),  subject to the feasible set $\cK$ defined by \eqref{eqn:set_ck}. Note that the set $\cK$ is critical, as by Lemma \ref{lemma:assumption_L}, it is a sufficient and almost necessary condition to ensure that the solution to the associated inner-loop subproblem is well defined. More importantly, from a robust control perspective, such a set $\cK$ represents the set of control gains that enjoy a certain level of \emph{robustness}, which share the same vein as the $\cH_{\infty}$-norm constraint for the infinite-horizon LTI setting  \cite{zhang2019policymixed}. Indeed,  they both enforce the gain matrix to \emph{attenuate} a prescribed level of disturbance. This level of robustness also corresponds to the level of \emph{risk-sensitivity} of the controllers in LEQG problems. For more discussion of both the finite- and infinite-horizon discrete-time disturbance attenuation problem, we refer the reader to \cite{doyle1989state, whittle1990risk, bacsar2008h}.

\begin{lemma}(Outer-Loop Landscape)\label{lemma:landscape_K}
 There exist zero-sum LQ dynamic games such that $\cG(\bK, \bL(\bK))$ is nonconvex and noncoercive on $\cK$. Specifically, as $\bK$ approaches $\partial\cK$, $\cG(\bK, \bL(\bK))$ does not necessarily approach $+\infty$. Moreover, the stationary point of $\cG(\bK, \bL(\bK))$ in $\cK$, denoted as $(\bK^*, \bL(\bK^*))$, is unique and constitutes the unique Nash equilibrium of the game.
 \end{lemma}

\begin{figure}[t]
\begin{minipage}{.48\textwidth}
\centering
\includegraphics[width=1\textwidth]{plots/landscape.png}
\caption{\textit{Left:} Optimization landscape of LQR, where the dashed line represents the boundary of the stabilizing controller set. \textit{Right:} Optimization landscape of the outer loop, with the dashed line representing the boundary of $\cK$. The solid lines represent the contour lines of the objective function, $K$ denotes the control gain of one iterate, and $\bigstar$ is the global minimizer.}
\label{fig:landscape}
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{plots/ir_plot.png}
\caption{Illustrating the proof idea for Theorem \ref{theorem:ir_K}. Starting with any $\bK \hspace{-0.1em} \in \hspace{-0.1em} \cK$ that induces a $\bP_{\bK, \bL(\bK)}$, denote the gain matrix after one step of the updates \eqref{eqn:npg_K} or \eqref{eqn:gn_K} as $\bK'$. We construct an iterative argument backward in time to find a constant stepsize such that $P_{K'_t, L(K'_t)} \hspace{-0.1em}\geq\hspace{-0.1em} 0$ exists and satisfies $P_{K'_t, L(K'_t)} \hspace{-0.1em}\leq\hspace{-0.1em} P_{K_t, L(K_t)}$ for all $t$. Specifically, for any $t \in \{0, \hspace{-0.1em}\cdots\hspace{-0.1em}, N\hspace{-0.1em}-\hspace{-0.1em}1\}$, a $K'_t$ satisfying \textcolor{mysquare}{$\blacksquare$} also satisfies \textcolor{mytriangle}{\large$\blacktriangle$\normalsize}. Moreover, \textcolor{mybigcube}{$\blacklozenge$} is automatically enforced by Assumption \ref{assumption_game_recursive}. Combined, $\bK' \hspace{-0.1em}\in  \hspace{-0.1em}\cK$ is guaranteed.}
\label{fig:proof1}
\end{minipage}
\end{figure}

Lack of the coercivity brings up challenges for convergence analysis, as a decrease in the value of the objective function cannot ensure feasibility of the updated gain matrix, in contrast to the standard LQR problem \cite{fazel2018global,bu2019LQR}. We illustrate the difficult landscape of the outer loop in Figure \ref{fig:landscape}. To address this challenge, we will show next that the natural PG (NPG) and Gauss-Newton (GN) updates, these two specific policy search directions, can  automatically preserve the feasibility of the iterates on-the-fly, which was referred to as the {implicit regularization} property in \cite{zhang2019policymixed} for infinite-horizon LTI systems. 
	
\subsection{Update Rules and Global Convergence}\label{sec:double_update}
	In this section, we introduce three PG-based update rules. We use $l, k \geq 0$ to represent the iteration indices of the inner- and outer-loop updates, respectively, and we additionally define 
	\begin{align}\label{eqn:gh_def}
		\bH_{\bK, \bL} := \bR^w - \bD^{\top}\bP_{\bK, \bL}\bD, \quad \bG_{\bK, \bL(\bK)} := \bR^u + \bB^{\top}\tilde{\bP}_{\bK, \bL(\bK)}\bB,
	\end{align}
 where $\tilde{\bP}_{\bK, \bL(\bK)}$ is defined in \eqref{eqn:tilde_pk}. The update rules, motivated by \cite{fazel2018global, bu2019LQR, zhang2019policymixed}, can be written as follows:
 
 \vspace{-0.9em}
\hspace{-2.55em}
\begin{minipage}[b]{0.5\linewidth}
 \centering\begin{align}
 	\text{PG: } \quad \bL_{l+1} &= \bL_l + \eta\nabla_{\bL}\cG(\bK_k, \bL_l), \label{eqn:pg_L}\\
 	\text{NPG: } \quad  \bL_{l+1} &= \bL_l + \eta\nabla_{\bL}\cG(\bK_k, \bL_l)\Sigma^{-1}_{\bK_k, \bL_l}, \label{eqn:npg_L} \\
 	\text{GN: } \quad  \bL_{l+1} &=  \bL_l + \eta\bH_{\bK_k, \bL_l}^{-1}\nabla_{\bL}\cG(\bK_k, \bL_l)\Sigma^{-1}_{\bK_k, \bL_l},\label{eqn:gn_L}
 \end{align}
\end{minipage}
\hspace{0.5em}
\begin{minipage}[b]{0.5\linewidth}
\centering
\begin{align}
	\bK_{k+1} &= \bK_k - \alpha\nabla_{\bK}\cG(\bK_k, \bL(\bK_k)), \label{eqn:pg_K}\\
	\bK_{k+1} &= \bK_k - \alpha\nabla_{\bK}\cG(\bK_k, \bL(\bK_k))\Sigma^{-1}_{\bK_k, \bL(\bK_k)}, \label{eqn:npg_K} \\
	\bK_{k+1} &= \bK_k - \alpha\bG_{\bK_k, \bL(\bK_k)}^{-1}\nabla_{\bK}\cG(\bK_k, \bL(\bK_k))\Sigma^{-1}_{\bK_k, \bL(\bK_k)},\label{eqn:gn_K}
\end{align}
\end{minipage}
where $\eta, \alpha >0$ are constant stepsizes for the inner loop and the outer loop, respectively. For a fixed $\bK \in \cK$, we have $\bH_{\bK, \bL_l}$ invertible for any $l \geq 0$. This is because $\bH_{\bK, \bL} \geq \bH_{\bK, \bL(\bK)} >0$ for all $\bL$. Also, we have $\bG_{\bK_k, \bL(\bK_k)}$ invertible for any $\bK_k \in \cK$, due to $\bG_{\bK_k, \bL(\bK_k)} \geq \bR^u$ in the p.s.d. sense at such iterations. We note that the PG \eqref{eqn:pg_L}, \eqref{eqn:pg_K} and NPG \eqref{eqn:npg_L}, \eqref{eqn:npg_K} updates can be estimated using samples, as shown in \cite{fazel2018global,malik2020derivative}. To prove the global convergence of our algorithms to the Nash equilibrium, we first present the convergence results for three inner-loop PG updates.

\begin{theorem}(Inner-Loop Global Convergence)\label{theorem:conv_L}
For a fixed $\bK\in \cK$ and an arbitrary $\bL_0$ that induces a finite $\cG(\bK, \bL_0)$, we define a superlevel set $\cL_{\bK}(a)$ as in \eqref{eqn:levelset_L}, where $a < \cG(\bK, \bL_0)$ is an arbitrary constant. Then, for $l \geq 0$, the iterates $\bL_l$ following \eqref{eqn:pg_L}-\eqref{eqn:gn_L} with stepsizes satisfying 
\begin{align*}
	\text{PG: } \ \eta \leq \frac{1}{\psi_{\bK, a}},\quad \text{Natural PG: } \ \eta \leq \frac{1}{2\|\bH_{\bK, \bL_0}\|}, \quad\text{Gauss-Newton: } \ \eta \leq \frac{1}{2},
\end{align*} 
converge to $\bL(\bK)$ at globally linear rates, where $\psi_{\bK, a}$ is the smoothness constant of the objective over $\cL_{\bK}(a)$, and $\bH_{\bK, \bL}$ is as defined in \eqref{eqn:gh_def}. Moreover, with $\eta = 1/2$, GN \eqref{eqn:gn_L} converges to $\bL(\bK)$ with a locally Q-quadratic rate.
\end{theorem}
The proof of Theorem \ref{theorem:conv_L} is deferred to \S\ref{proof:conv_L}. For the outer loop, we require the iterates of $\bK$ to stay within $\cK$ in order for the solution to the associated inner-loop subproblem to be well defined. To meet this requirement, we introduce the \emph{implicit regularization} property for the NPG \eqref{eqn:npg_K} and GN \eqref{eqn:gn_K} updates in Theorem \ref{theorem:ir_K}, with its proof being provided in \S\ref{proof:ir_K}.   

\begin{theorem}(Implicit Regularization)\label{theorem:ir_K}
	{Let $\bK_0 \in \cK$ and let the stepsizes satisfy
	\begin{align*}
		\text{Natural PG: }  \alpha \leq 1/\|\bG_{\bK_0, \bL(\bK_0)}\|, \quad \text{Gauss-Newton: }\alpha &\leq 1.
	\end{align*}
	Then, the iterates $\bK_k \in\cK$ for all $k \geq 0$. In other words, the sequence of solutions to the Riccati equation \eqref{eqn:DARE_black_L}, $\{\bP_{\bK_k, \bL(\bK_k)}\}$, exists, and for all $k \geq 0$, $\bP_{\bK_k, \bL(\bK_k)}$ always satisfies the conditions in \eqref{eqn:set_ck}. Furthermore, the sequence $\{\bP_{\bK_k, \bL(\bK_k)}\}$ is monotonically non-increasing and bounded below by $\bP_{\bK^*, \bL(\bK^*)}$, in the p.s.d. sense.}
\end{theorem}
We note that one key step of the proof for Theorem \ref{theorem:ir_K} is to ensure the \emph{existence} of a solution to \eqref{eqn:DARE_black_L} along the iterations, by carefully controlling the sizes of update steps along certain descent directions. We provide an illustration of the proof idea in Figure \ref{fig:proof1}. Specifically, the implicit regularization property holds  for NPG and GN directions because they can ensure \emph{matrix-wise} decrease of $\bP_{\bK_k,\bL(\bK_k)}$ (more than just that of the objective value $\cG(\bK,\bL(\bK))$), while other descent directions (e.g., vanilla PG) can only decrease  $\cG(\bK,\bL(\bK))$, which is a \emph{scalar-wise} decrease and is not sufficient  to ensure that the next iterate stays  in $\cK$. Note that the intuition for implicit regularization here is thus more explicit than that in \cite{zhang2019policymixed} for infinite-horizon LTI settings, where some linear matrix inequalities have to be delicately designed. We highlight the importance of the implicit regularization property as follows.
\begin{remark}(Preserving the Robustness of $\bK_0$)\label{remark:ir}
Suppose that the initial control gain matrix satisfies $\bK_0 \in \cK$. Then Lemma \ref{lemma:equivalent} shows that $\bK_0$ is the control gain matrix that attains a $\gamma$-level of disturbance attenuation. By the implicit regularization property in Theorem \ref{theorem:ir_K}, every iterate $\bK_k\in\cK$ for all $k\geq 0$ following the NPG \eqref{eqn:npg_K} or the GN \eqref{eqn:gn_K} update rules will thus preserve this $\gamma$-level of disturbance attenuation throughout the policy optimization (learning) process. Theorem \ref{theorem:ir_K} thus provides some provable robustness guarantees for two specific policy search directions, \eqref{eqn:npg_K} and \eqref{eqn:gn_K}, which is important for safety-critical control systems in the presence of adversarial disturbances, since otherwise, the system performance index can be driven to arbitrarily large values.  
\end{remark}	
Based on Theorem \ref{theorem:ir_K},  we now establish the convergence result for the outer loop.

\begin{theorem}(Outer-Loop Global Convergence)\label{theorem:Mbased_conv_K}
	Let $\bK_0 \in \cK$ and let the stepsizes satisfy
\begin{align*}
	\text{Natural PG: }  \alpha \leq 1/(2\|\bG_{\bK_0, \bL(\bK_0)}\|), \quad \text{Gauss-Newton: }  \alpha \leq 1/2,
\end{align*}
where $\bG_{\bK, \bL(\bK)}$ is as defined in \eqref{eqn:gh_def}. Then, the sequence of average natural gradient norm squares $\{k^{-1}\sum^{k-1}_{\kappa = 0}\|\bF_{\bK_\kappa, \bL(\bK_\kappa)}\|^2_F\}$, $k\geq 1$, converges to $\bm{0}$ with $\cO(1/k)$ rate. Moreover, this convergence is towards the unique Nash equilibrium. Lastly, the NPG \eqref{eqn:npg_K} and GN \eqref{eqn:gn_K} updates enjoy locally linear and Q-quadratic rates, respectively,  around the Nash equilibrium. 
\end{theorem}
The proof of Theorem \ref{theorem:Mbased_conv_K} is deferred to \S\ref{proof:Mbased_conv_K}.  In the derivative-free setting where PGs are estimated through samples of system trajectories, if we can uniformly control the estimation bias using a fixed number of samples per iterate, then Theorems  \ref{theorem:conv_L} and \ref{theorem:Mbased_conv_K} together imply that the global convergence to the Nash equilibrium also holds. We will substantiate this in the next section. 


==> Mixed Design Arxiv v3/game.tex <==
\subsection{An Equivalent Dynamic Game Formulation}\label{sec:game} 
Lastly, and more importantly, we describe an equivalent dynamic game formulation to the LEQG and the LQ disturbance attenuation problems introduced above. Under certain conditions to be introduced in Lemma \ref{lemma:equivalent}, the saddle-point gain matrix of the minimizing player in the dynamic game (if exists) also addresses the LEQG and the LQ disturbance attenuation problem, providing an alternative route to overcome the challenges reported in Remark \ref{rmk:challenge_LEQG_atten}. Specifically, we consider a zero-sum LQ stochastic dynamic game (henceforth, game) model with closed-loop perfect-state information pattern, which can also be viewed as a benchmark setting of MARL for two competing agents 
\cite{shapley1953stochastic, littman1994markov,zhang2019policy, bu2019global, zhang2020model}, as the role played by LQR for  single-agent RL \cite{recht2019tour}. The linear time-varying system dynamics follow
\begin{align}\label{eqn:sto_game_dynamics}
	x_{t+1} = A_tx_t + B_tu_t + D_tw_t + \xi_t, \quad t\in\{0,\cdots,N-1\},
\end{align}
where $x_t \in \RR^{m}$ is the system state, $u_t:=\mu_{u, t}(h_{u, t}) \in \RR^{d}$ (resp., $w_t:=\mu_{w, t}(h_{w, t}) \in \RR^{n}$) is the control input of the minimizing (resp., maximizing) player\footnote{Hereafter we will use player and agent interchangeably.} and $\mu_{u, t}: (\RR^{m}\times\RR^d)^t \times \RR^m \rightarrow \RR^d$ (resp., $\mu_{w, t}: (\RR^{m}\times\RR^n)^t \times \RR^m \rightarrow \RR^n$) is the control policy that maps, at time $t$, the history of state-control pairs up to time $t$, and state at time $t$, denoted as $h_{u, t}:=\{x_0, \cdots, x_{t}, u_{0}, \cdots, u_{t-1}\}$ (resp., $h_{w, t}:=\{x_0, \cdots, x_{t}, w_{0}, \cdots, w_{t-1}\}$), to the control $u_t$ (resp., $w_t$). The independent process noises are denoted by $\xi_t \sim \cD$ and $A_t$, $B_t$, $D_t$ are system matrices with proper  dimensions. Further, we assume $x_0 \sim \cD$ to be independent of the process noises, and the distribution $\cD$ has zero mean and a positive-definite covariance. We also assume that $\|x_0\|, \|\xi_t\| \leq \vartheta$, for all $t\in \{0, \cdots, N-1\}$, almost surely, for some constant $\vartheta$\footnote{{The assumption on the boundedness of distribution is only for ease of analysis \cite{malik2020derivative, furieri2019learning}. Extensions to sub-Gaussian distributions are standard and do not affect the sample complexity result, as noted by \cite{malik2020derivative}.}}. The goal of the minimizing (resp. maximizing) player is to minimize (resp. maximize) a quadratic objective function, namely to solve the zero-sum game 
\begin{align}\label{eqn:game_value_uw}
	\inf_{\{u_t\}}~\sup_{\{w_t\}}~ \EE_{x_0, \xi_0, \cdots, \xi_{N-1}}\bigg[\sum^{N-1}_{t=0} \big(x_t^{\top}Q_tx_t + u_t^{\top}R^u_tu_t - w^{\top}_tR^w_tw_t\big) + x_N^{\top}Q_Nx_N\bigg],
\end{align}
where $Q_t \geq 0$, $R^u_t, R^w_t >0$ are symmetric weighting matrices and the system transitions follow \eqref{eqn:sto_game_dynamics}. Whenever the solution to \eqref{eqn:game_value_uw} exists such that the $\inf$ and $\sup$ operators in \eqref{eqn:game_value_uw} are interchangeable, then the value \eqref{eqn:game_value_uw} is the \emph{value} of the game, and the corresponding policies of the players are known as saddle-point policies. To characterize the solution to \eqref{eqn:game_value_uw}, we first introduce the following time-varying generalized RDE (GRDE):
	\begin{align}\label{eqn:RDE_recursive}
		P^*_t = Q_t + A^{\top}_tP^*_{t+1}\Lambda^{-1}_{t}A_t, \quad t \in \{0, \cdots, N-1\},
	\end{align}
	where $\Lambda_{t}:=\bI + \big(B_t(R^u_t)^{-1}B^{\top}_t - D_t(R^w_t)^{-1}D_t^{\top}\big)P^*_{t+1}$ and $P^*_N = Q_N$. For the stochastic game with closed-loop perfect-state information pattern that we considered, we already know from \cite{bacsar1998dynamic} that whenever a saddle point exists, the saddle-point control policies are linear state-feedback (i.e., $\mu^*_{u, t}(h_{u, t}) = -K^*_tx_t$ and $\mu^*_{w, t}(h_{w, t})= -L^*_tx_t$), and the gain matrices $K^*_t$ and $L^*_t$, for $t \in\{0, \cdots, N-1\}$, are unique and can be expressed by

\vspace{-0.5em}
\hspace{-2.5em}
\begin{minipage}[b]{0.5\linewidth}
 \centering\begin{align}
K^*_t &= (R^u_t)^{-1}B_t^{\top}P^*_{t+1}\Lambda_{t}^{-1}A_t, \label{eqn:optimalK_r}
 \end{align}
\end{minipage}
\hspace{0.4em}
\begin{minipage}[b]{0.5\linewidth}
\centering
\begin{align}
L^*_t &= -(R^w_t)^{-1}D_t^{\top}P^*_{t+1}\Lambda_{t}^{-1}A_t,\label{eqn:optimalL_r}
\end{align}
\end{minipage}

\noindent where $P^*_{t+1}$, $t \in \{0, \cdots, N-1\}$, is the sequence of p.s.d. matrices generated by  \eqref{eqn:RDE_recursive}. We next introduce a standard assumption that suffices to ensure the existence of the value of the game, following from Theorem 3.2 of \cite{bacsar2008h} and Theorem 6.7 of \cite{bacsar1998dynamic}.

\begin{assumption}\label{assumption_game_recursive}
$R^w_t - D^{\top}_tP^*_{t+1}D_t > 0$, for all $t\in\{0, \cdots, N-1\}$, where $P^*_{t+1} \geq 0$ is generated by \eqref{eqn:RDE_recursive}.
\end{assumption}
Under Assumption \ref{assumption_game_recursive}, the value in \eqref{eqn:game_value_uw} is attained by the controller sequence $\big(\{-K^*_tx^*_t\}, \{-L^*_tx^*_t\}\big)$, where $K^*_t$ and $L^*_t$ are given in \eqref{eqn:optimalK_r} and \eqref{eqn:optimalL_r}, respectively, and $x^*_{t+1}$ is the corresponding state trajectory generated by $x^*_{t+1} = \Lambda^{-1}_tA_tx^*_t + \xi_t$, for $t \in \{0, \cdots, N-1\}$ and with $x_0^* = x_0$ \cite{bacsar2008h}. Thus, the solution to \eqref{eqn:game_value_uw} can be found by searching $K^*_t$ and $L^*_t$ in $\RR^{d\times m} \times \RR^{n \times m}$, for all $t \in \{0, \cdots, N-1\}$. The resulting minimax policy optimization problem is
\begin{align}\label{eqn:game_value}
	\min_{\{K_t\}}~\max_{\{L_t\}} ~\cG\big(\{K_t\}, \{L_t\}\big) := \EE_{x_0, \xi_0, \cdots, \xi_{N-1}}\bigg[\sum^{N-1}_{t=0} x_t^{\top}\big(Q_t + K_t^{\top}R^u_tK_t - L^{\top}_tR^w_tL_t)x_t + x_N^{\top}Q_Nx_N\bigg],
\end{align}
subject to the system transition $x_{t+1} = (A_t-B_tK_t-D_tL_t)x_t +\xi_t$, for $t\in\{0, \cdots, N-1\}$. Some further notes regarding Assumption \ref{assumption_game_recursive} are provided in the remark below.
\begin{remark} (Unique Feedback Nash (Saddle-point) Equilibrium)
	By \cite{bacsar2008h, bacsar1998dynamic}, Assumption \ref{assumption_game_recursive} is sufficient to guarantee the \emph{existence} of feedback Nash (equivalently, saddle-point) equilibrium in zero-sum LQ dynamic games (game), under which it is also unique. Besides sufficiency, Assumption \ref{assumption_game_recursive} is also ``almost necessary", and ``quite tight" as noted in Remark 6.8 of \cite{bacsar1998dynamic}. In particular, if the sequence of matrices $R^w_t - D^{\top}_tP^*_{t+1}D_t$ for $t \in \{0, \cdots, N-1\}$ in Assumption \ref{assumption_game_recursive} admits any negative eigenvalues, then the upper value of the game becomes unbounded. In the context of LEQG and LQ disturbance attenuation (LQDA), suppose we set the system parameters of LEQG, LQDA, and game according to Lemma \ref{lemma:equivalent}, and in particular set $\beta^{-1}\bI$ in LEQG,  $\gamma^2\bI$ in LQDA, and $\bR^w$ in the game to be the same. Then these three problems are equivalent as far as their optimum solutions go (which is what we seek). Due to this equivalence, Assumption \ref{assumption_game_recursive} is a sufficient and ``almost necessary" condition for the existence of a solution to the equivalent LEQG/LQDA. Specifically, if the sequence of matrices $R^w_t - D^{\top}_tP^*_{t+1}D_t$ for $t \in \{0, \cdots, N-1\}$ in Assumption \ref{assumption_game_recursive} admits any negative eigenvalues, then no state-feedback controller can achieve a $\gamma$-level of disturbance attenuation in the equivalent LQDA, and no state-feedback controller can achieve a $\beta$-degree of risk-sensitivity in the equivalent LEQG. 	
\end{remark}
Lastly, we formally state the well-known equivalence conditions between LEQG, LQ disturbance attenuation, and zero-sum LQ stochastic dynamic games in the following lemma, and provide a short proof in \S\ref{proof:equivalent}.

\begin{lemma}(Connections)\label{lemma:equivalent}
	For any fixed $\gamma > \gamma^*$ in the LQ disturbance attenuation problem, we can introduce an equivalent LEQG problem and an equivalent zero-sum LQ dynamic game. Specifically, if we set $\beta^{-1}\bI, R_t, C_t^{\top}C_t, W$ in LEQG, $\gamma^2\bI, R_t, C_t^{\top}C_t, D_tD_t^{\top}$ in the LQ disturbance attenuation problem, and $R^w_t, R^u_t, Q_t, D_tD_t^{\top}$ in the game to be the same, for all $t \in \{0, \cdots, N-1\}$, then the optimal gain matrices in LEQG, the gain matrix in the LQ disturbance attenuation problem, and the saddle-point gain matrix for the minimizing player in the game are the same.
\end{lemma}


 By the above connections and Remark \ref{rmk:challenge_LEQG_atten}, we will hereafter focus on the stochastic zero-sum LQ dynamic game  between a minimizing controller and a maximizing disturbance, using PG methods with exact gradient accesses in \S\ref{sec:1st}, and derivative-free PG methods by sampling system trajectories in \S\ref{sec:0order}. As a result, the minimizing controller we obtain solves all three classes of problems introduced above altogether.  


==> Mixed Design Arxiv v3/landscape.tex <==

\xznote{note that it is different from LQR, don't overclaim}


%Moreover, we can show that whenever $\bK \in \cK$, the cost function of the outer loop is smooth.
% 
% \begin{lemma}(``Smoothness'')\label{lemma:smooth_K} For $\bK \in \cK$, the cost function $\cG(\bK, \bL(\bK))$ of the outer loop is $\psi_2$-smooth. That is,
% \begin{align*}
% 	\|\nabla_{\bK}\cG(\bK', \bL(\bK')) - \nabla_{\bK}\cG(\bK, \bL(\bK))\|_F &\leq \psi_2 \|\bK'-\bK\|_F, \ \forall \bK \in \cK, 
% \end{align*}
% where $\psi_2$ is an absolute constant.
% \end{lemma}
 

%By Lemma \ref{assumption_game}, for any fixed $\bK_i \in \overline{\cK}$, the maximization problem in terms of $\bL$ is a well-defined indefinite LQR that is $\psi_i$-smooth and $p_i$-PL. Also, for any $\bK \in \overline{\cK}$, the Hessian is a polynomial and $\overline{\cK}$ is compact, there exists a uniform upper bound for the Hessian. Combining the above two conditions yields that there exists a constant parameter $L_1$ such that   
%\begin{align*}
%	\|\nabla_{\bK}\cG(\bK', \bL') - \nabla_{\bK}\cG(\bK, \bL)\| \leq L_1 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bK \in \overline{\cK}	
%\end{align*}
%Similarly, we can show that $\overline{\cL}$ is a compact set and for any fixed $\bL \in \overline{\cL}$, the minimization problem in terms of $\bK$ is a well-defined indefinite LQR that is $\psi_j$-smooth and $p_j$-PL. Thus, we can also derive the condition such that there exists a constant parameter $L_2$  that 
%\begin{align*}
%	\|\nabla_{\bL}\cG(\bK', \bL') - \nabla_{\bL}\cG(\bK, \bL)\| \leq L_2 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bL \in \overline{\cL}.
%\end{align*}
%This proves the two-sided smoothness property, similar to Assumption 1 of \cite{yang2020global}, but restricted to the region where $(\bK, \bL) \in  \overline{\cK} \times \overline{\cL}$.  Finally, invoking Lemma A.2 of \cite{yang2020global} yields that the outer loop is $L$-smooth with $L:=\max\{L_1, L_2\} + \frac{\max\{L_1, L_2\}}{\max_i{p_i}}$ for any $\bK \in \overline{\cK}$.
% \begin{lemma}(Lemma A.3 of \cite{nouiehed2019solving})
% 	Assume that $\{\cG(\bK, \bL) \mid \bK \in \cK\}$ is a class of $\Upsilon$-PL functions in $\bL$, where $\Upsilon$ is an absolute constant. Then, if $\bL(\bK) = \argmax_{\bL}\cG(\bK, \bL)$, we have for any $\bK_1, \bK_2 \in \cK$ and their corresponding $\bL(\bK_1), \bL(\bK_2)$, 
% 	\begin{align*}
% 		\|\bK_1 - \bK_2\| \leq \frac{\textcolor{red}{L}}{2\Upsilon}\|\bL(\bK_1) - \bL(\bK_2)\| 
% 	\end{align*}  
% \end{lemma}
%
%\begin{lemma}(Lemma A.5 of \cite{nouiehed2019solving})
%	For $\bK \in \cK$, the outer loop is $\psi_{2}$-smooth.
%\end{lemma}
%Meisam Lemma A.5: outer loop is smooth, for $\bK \in \cK$.
% \end{proof}
% 
% 
% \begin{lemma}(Two-Sided Smoothness)\label{lemma:two_side_smooth}
% There exists a positive constant $l >0$ such that
% \begin{align*}
% 	\|\nabla_{\bK}\cG(\bK', \bL') - \nabla_{\bK}\cG(\bK, \bL)\| \leq l \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \\
% 	\|\nabla_{\bL}\cG(\bK', \bL') - \nabla_{\bL}\cG(\bK, \bL)\| \leq l \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big],
% \end{align*}	
% holds for all pairs of $(\bK, \bL)$ such that $\bK \in \cK$ and $\bL \in \cL$.
%\end{lemma}
%
%\begin{proof}
%First, define the auxiliary sets 
%\begin{align*}
%	\overline{\cK}:= \{\bK \mid \bR^w-\bD^{\top}\bP_{\bK, \bL(\bK)}\bD \geq \zeta\bI\}, \quad \overline{\cL} := \{\bL \mid \bR^u + \bB^{\top}\bP_{\bK(\bL), \bL}\bB \geq \zeta\bI \}, 
%\end{align*}
%where $\bL(\bK) = \argmax_{\bL}\cG(\bK, \bL)$ and $\bK(\bL) = \argmin_{\bK}\cG(\bK, \bL)$ for whenever $\bL(\bK)$ and $\bK(\bL)$ exist and $\zeta>0$ is a small constant such that $\overline{\cK}$ and $\overline{\cL}$ are nonempty. We first claim that $\overline{\cK}$ is a compact set. First, we show that $\overline{\cK}$ is closed. Since $\bP_{\bK, \bL(\bK)}$ is the unique solution of the Riccati equation
%\begin{align*}
%	\bP_{\bK, \bL(\bK)} = \bQ + \bK^{\top}\bR^u\bK - \bL(\bK)^{\top}\bR^w\bL(\bK) +(\bA-\bB\bK-\bD\bL(\bK))^{\top}\bP_{\bK, \bL(\bK)}(\bA-\bB\bK-\bD\bL(\bK))
%\end{align*}
%where the uniqueness is due to the fact that it is actually an iterative linear equation in terms of the blocks. Thus, $\overline{\cK}$ is closed. Then, it remains to show that $\overline{\cK}$ is bounded. Since $\bQ \geq 0, \bR^u, \bR^w > 0$ and $\bL$ is the control gain matrix of the maximizing player, we have $\bQ + \bK^{\top}\bR^u\bK - \bL(\bK)^{\top}\bR^w\bL(\bK) \geq 0$. This leads to $\bP_{\bK, \bL(\bK)} \geq 0$. Moreover, for any $\bK \in \overline{\cK}$,
%\begin{align*}
%	\bD^{\top}\bP_{\bK, \bL(\bK)}\bD \leq \bR^w \Rightarrow \|\bD^{\top}\bP_{\bK, \bL(\bK)}\bD\| \leq \|\bR^w\| \Rightarrow \|\bP_{\bK, \bL(\bK)}\| \leq C
%\end{align*}
%where $C>0$ is a finite absolute constant. This results in the condition that $\sup_{\bK}\|\bK\| < \infty$. Therefore, the set $\overline{\cK}$ is bounded and thus compact. By Lemma \ref{assumption_game}, for any fixed $\bK_i \in \overline{\cK}$, the maximization problem in terms of $\bL$ is a well-defined indefinite LQR that is $\psi_i$-smooth and $p_i$-PL. Also, for any $\bK \in \overline{\cK}$, the Hessian is a polynomial and $\overline{\cK}$ is compact, there exists a uniform upper bound for the Hessian. Combining the above two conditions yields that there exists a constant parameter $L_1$ such that   
%\begin{align*}
%	\|\nabla_{\bK}\cG(\bK', \bL') - \nabla_{\bK}\cG(\bK, \bL)\| \leq L_1 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bK \in \overline{\cK}	
%\end{align*}
%Similarly, we can show that $\overline{\cL}$ is a compact set and for any fixed $\bL \in \overline{\cL}$, the minimization problem in terms of $\bK$ is a well-defined indefinite LQR that is $\psi_j$-smooth and $p_j$-PL. Thus, we can also derive the condition such that there exists a constant parameter $L_2$  that 
%\begin{align*}
%	\|\nabla_{\bL}\cG(\bK', \bL') - \nabla_{\bL}\cG(\bK, \bL)\| \leq L_2 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bL \in \overline{\cL}.
%\end{align*}
%This proves the two-sided smoothness property, similar to Assumption 1 of \cite{yang2020global}, but restricted to the region where $(\bK, \bL) \in  \overline{\cK} \times \overline{\cL}$.  Finally, invoking Lemma A.2 of \cite{yang2020global} yields that the outer loop is $L$-smooth with $L:=\max\{L_1, L_2\} + \frac{\max\{L_1, L_2\}}{\max_i{p_i}}$ for any $\bK \in \overline{\cK}$.
 
%	We prove the two-sided smoothness property by showing that when fixing either $\bK$ or $\bL$, the cost function of the remaining single-player optimization problem is smooth. That is, there exists constants $l_{\bK}, l_{\bl}$ such that
%	\begin{align}\label{eqn:fixed_L}
%	 	\|\nabla_{\bK}\cG(\bK', \bL) - \nabla_{\bK}\cG(\bK, \bL)\| &\leq l_{\bK} \|\bK'-\bK\|, \\
% 	\|\nabla_{\bL}\cG(\bK, \bL') - \nabla_{\bL}\cG(\bK, \bL)\| &\leq l_{\bL}  \|\bL'-\bL\|, \label{eqn:fixed_K}
%	\end{align}
%	holds for all $\bK$ and $\bL$. If \eqref{eqn:fixed_K} and \eqref{eqn:fixed_L} hold, Lemma \ref{lemma:two_side_smooth} is proved by setting $l = \max(l_{\bK}, l_{\bL})$. Now, we focus on proving \eqref{eqn:fixed_K} and \eqref{eqn:fixed_L}. Notice that for any fixed $\bK$, the maximization problem in terms of $\bL$ is essentially an indefinite LQR with state weighting matrix $-\bQ-\bK^{\top}\bR^u\bK$ and state transition matrix $\bA - \bB\bK$. Similarly, for any fixed $\bL$, the minimization problem in terms of $\bK$ is also an indefinite LQR with state-weighting matrix $\bQ - \bL^{\top}\bR^w\bL$ and state transition matrix $\bA-\bD\bL$. \xznote{expand}Then, we can conclude coerciveness properties and thus compact level sets. This leads to \eqref{eqn:fixed_K} and \eqref{eqn:fixed_L} and thus proves the two-sided smoothness property.


\subsection{Global Convergence}\label{sec:convergence}



 

%	There are a few intuitions behind the initialization process that we would like to point out. Firstly, when initializing with any $\bK_0$,  there exists a finite disturbance attenuation level $\gamma_{\bK_0} > \gamma^*$ associated with the initial controller $\bK_0$. By Lemma \ref{lemma:game-game} and \ref{lemma:game-inf}, we can formulate a corresponding stochastic game parametrized by $\gamma_{\bK_0}$ that is well-defined, in the sense that the upper value of the game is finite. Then, as we shown in Theorem \ref{theorem:ir_K}, this initial disturbance attenuation level is preserved on-the-fly along two PG methods. Finally, Theorem \ref{theorem:Mbased_conv_K} proves that starting with any $\bK_0$, two PG methods converge to the saddle-point policies of the associated game. According to Lemma \ref{lemma:game-game} and \ref{lemma:game-inf}, the saddle point policy of the minimizing player is equivalent to the controller that minimizes the objective \eqref{eqn:ckl} and also attains a the disturbance attenuation level of $\gamma_{\bK_0}$ in the original disturbance attenuation problem. 
%	
%	Further, for any $\tilde{\bK}_0$ that satisfies a prescribed disturbance attenuation level $\gamma_{\tilde{\bK}_0} > \gamma^*$, Theorem \ref{theorem:Mbased_conv_K}, Lemma \ref{lemma:game-game}, and Lemma \ref{lemma:game-inf} demonstrate that two PG methods automatically preserve the a $\gamma_{\tilde{\bK}_0}$-level of disturbance attenuation on-the-fly while converging globally to the saddle point. Lastly, searching for such a feasible initial control gain matrix $\tilde{\bK}_0$ that satisfies $\gamma_{\tilde{\bK}_0} > \gamma^*$ is empirically permissible through a ``robustification'' process without the knowledge of model parameters \cite{zhang2020rarl}. 


==> Mixed Design Arxiv v3/mix.tex <==
\subsection{LQ Disturbance Attenuation}\label{sec:mix}
Second, we introduce the \emph{optimal} LQ disturbance attenuation problem, again for finite-horizon settings, with time-varying (deterministic) dynamical systems described by
\begin{align*}
x_{t+1} = A_tx_t + B_tu_t + D_tw_t, \quad z_t = C_tx_t + E_tu_t, \quad t\in\{0,\cdots,N-1\},
\end{align*}
where $x_t \in \RR^{m}$ is the system state; $u_t \in \RR^{d}$ is the control input; $w_t \in \RR^{n}$ is the (unknown) disturbance input; $z_t \in \RR^{l}$ is the controlled output; $A_t$, $B_t$, $C_t$, $D_t$, $E_t$ are system matrices with appropriate dimensions; and $x_0 \in \RR^{m}$ is unknown. In  addition, we assume that $E_t^{\top} [C_t \ E_t] = [0 \ R_t]$ for some $R_t > 0$ to eliminate the cross-weightings between control input $u$ and system state $x$, which provides no loss of generality, and is standard in the literature  \cite{glover1988state, bacsar2008h}. As shown in \S 3.5.1 of \cite{bacsar2008h}, a simple procedure can transform the general problem into a form where there are no coupling terms between $u$ and $x$, satisfying the above ``normalization” assumption that we have made. Subsequently, we introduce the $\ell^2$-norms of the vectors $\omega:=\big[x_0^{\top}C_0^{\top}, w_0^{\top}, \cdots, w_{N-1}^{\top}\big]^{\top}$ and $z := \big[z_0^{\top}, \cdots, z_{N-1}^{\top}, x_N^{\top}Q_N^{1/2}\big]^{\top}$ as $\|\omega\| := \big\{x_0^{\top}C^{\top}_0C_0x_0 + \sum^{N-1}_{t=0}\|w_t\|^2\big\}^{1/2}$ and $\|z\| =\big\{\cC\big(\{u_t\}, \{w_t\}\big)\big\}^{1/2} := \big\{x_N^{\top}Q_Nx_N + \sum^{N-1}_{t=0}\|z_t\|^2\big\}^{1/2}$, where $Q_N \geq 0$ is symmetric, and $\|\cdot\|$ in the two expressions denote appropriate Euclidean norms. Then, the robustness of a designed controller can be guaranteed by a constraint on the ratio between $\|z\|$ and $\|\omega\|$. Specifically, the goal of the optimal LQ disturbance attenuation problem is to find the optimal control policy $\mu^*_t : (\RR^{m}\times\RR^d)^t \times \RR^m \rightarrow \RR^d$ that maps, at time $t$, the history of state-control pairs until time $t$ and the current state $x_t$, denoted as $h_{t}:=\{x_0, \cdots, x_{t}, u_{0}, \cdots, u_{t-1}\}$, to the control $u_t$, such that
\begin{align}\label{equ:optimal_DA}
	\gamma^* = \inf_{\{\mu_t\}}~\sup_{x_0, \{w_t\}} ~\frac{\big\{\cC\big(\{
\mu_t(h_t)\}, \{w_t\}\big)\big\}^{1/2}}{\|\omega\|} = \sup_{x_0, \{w_t\}} ~\frac{\big\{\cC\big(\{
\mu^*_t(h_t)\}, \{w_t\}\big)\big\}^{1/2}}{\|\omega\|},
\end{align}
where $\gamma^* = \sqrt{(\beta^*)^{-1}} >0$ is the \emph{optimal} (\emph{minimax}) level of disturbance attenuation at the output \cite{glover1988state, bacsar2008h}, and recall that $\beta^*$ is the upper bound for the risk-sensitivity parameter in LEQG. It is known that under closed-loop perfect-state information pattern, the existence of a sequence $\{\mu^*_t\}$, $t\in\{0, \cdots, N-1\}$, is always guaranteed and $\mu^*_t$ is linear state-feedback, i.e., $\mu^*(h_t) = -K^*_tx_t$ (\cite{bacsar2008h}; Theorem 3.5). Thus, it suffices to search for $K_t^* \in \RR^{d\times m}$, for all $t \in \{0, \cdots, N-1\}$, to achieve the optimal attenuation.

The problem \eqref{equ:optimal_DA} can be challenging to solve to the optimum  \cite{bacsar2008h}. Moreover, in practice, due to the inevitable uncertainty in modeling the system, the robust controller that achieves the optimal attenuation level can be too sensitive to the model uncertainty to use. Hence, a reasonable surrogate of the optimal LQ disturbance attenuation problem is the following: Given a $\gamma > \gamma^*$, find a control policy $\mu_t = -K_tx_t$, for all $t \in \{0, \cdots, N-1\}$, that solves
\small
\begin{align}\label{eqn:mixed_LQ}
	\min_{\{\mu_{t}\}}~\cJ\big(\{
\mu_t(x_t)\}\big):= \EE_{\{\xi_t\}}\bigg[\sum_{t=0}^{N-1}\big(x^{\top}_tQ_tx_t + u^{\top}_tR_tu_t\big) + x_N^{\top}Q_Nx_N\bigg] \quad \text{s.t.} \  \sup_{x_0, \{w_t\}} ~\frac{\big\{\cC\big(\{
\mu_t(x_t)\}, \{w_t\}\big)\big\}^{1/2}}{\|\omega\|} < \gamma,
\end{align}
\normalsize
where $Q_t := C_t^{\top}C_t$ for $t\in\{0, \cdots, N-1\}$,  $\cJ\big(\{\mu_t(x_t)\}\big)$ is the LQG cost of the system $x_{t+1} = A_tx_t + B_tu_t + D_t\xi_t$,  and $\xi_t \sim \cN(\bm{0}, \bI)$ is independent Gaussian noise with unit intensity \cite{mustafa1991lqg}. Note that the LQ disturbance attenuation problem in \eqref{eqn:mixed_LQ}, and particularly with $x_0=\bm{0}$, is also called the mixed $\cH_2/\cH_{\infty}$ problem \cite{doyle1989state, mustafa1991lqg, kaminer1993mixed, zhang2019policymixed}, when the system is time-invariant, and the horizon of the problem $N$ is $\infty$. To solve \eqref{eqn:mixed_LQ} using policy optimization methods, we introduce the time-varying RDE:
\begin{align}\label{eqn:RDE_DA}
	P_{K_t} = Q_t + K_t^{\top}R_tK_t + (A_t-B_tK_t)^{\top}\tilde{P}_{K_{t+1}}(A_t-B_tK_t), \quad t\in\{0, \cdots, N-1\}, \quad P_{K_N} = Q_N,
\end{align}
where $\tilde{P}_{K_{t+1}}:= P_{K_{t+1}} + P_{K_{t+1}}(\gamma^2\bI - D_t^{\top} P_{K_{t+1}}D_t)^{-1}P_{K_{t+1}}$. Then, two upper bounds of $\cJ$ and their corresponding PGs can be expressed in terms of solutions to \eqref{eqn:RDE_DA} (if exist) \cite{mustafa1991lqg}. In particular, \eqref{eqn:DA_obj_1} below is closely related to the objective function of LEQG in \eqref{eqn:leqg_objective}, and \eqref{eqn:DA_obj_2} is connected to the objective function of zero-sum LQ dynamic games to be introduced shortly.
 
\begin{lemma}(Closed-Forms for the Objective Function and PGs) \label{lemma:pg_mix} For any sequence of control gains $\{K_t\}$ such that \eqref{eqn:RDE_DA} generates a sequence of p.s.d. solutions $\{P_{K_{t+1}}\}$ satisfying $\gamma^2\bI - D_t^{\top} P_{K_{t+1}}D_t >0$, for all $t \in \{0, \cdots, N-1\}$, and $\gamma^2\bI - P_{K_0} >0$, then two common upper bounds of the objective function $\cJ$ in \eqref{eqn:mixed_LQ} are:
\begin{align}
	\overline{\cJ}\big(\{K_t\}\big) &= -\gamma^{2}\log\det(\bI - \gamma^{-2} P_{K_{0}}) -\gamma^{2}\sum_{t=1}^{N}\log\det(\bI - \gamma^{-2} P_{K_{t}}D_{t-1}D^{\top}_{t-1}),\label{eqn:DA_obj_1} \\
	\overline{\cJ}\big(\{K_t\}\big) &= \tr(P_{K_0}) + \sum_{t = 1}^{N}\tr(P_{K_{t}}D_{t-1}D_{t-1}^{\top}).\label{eqn:DA_obj_2}
\end{align}
The PGs of \eqref{eqn:DA_obj_1} and \eqref{eqn:DA_obj_2} at time $t$ can be expressed as 
	\begin{align}\label{eqn:DA_PG}
		\nabla_{K_t}\overline{\cJ}\big(\{K_t\}\big) := \frac{\partial \overline{\cJ}\big(\{K_t\}\big)}{\partial K_t}= 2\big[(R_t+B^{\top}_t\tilde{P}_{K_{t+1}}B_t)K_t - B_t^{\top}\tilde{P}_{K_{t+1}}A_t\big]\Sigma_{K_t}, \quad t\in\{0, \cdots, N-1\},
	\end{align}
	where $\Sigma_t$, $t \in \{0, \cdots, N-1\}$, for the PGs of \eqref{eqn:DA_obj_1} and \eqref{eqn:DA_obj_2} are expressed, respectively, as
	\small
	\begin{align*}
	\Sigma_{K_t} &:= \prod^{t-1}_{i=0}\big[(\bI- \gamma^{-2}P_{K_{i+1}}D_iD_i^{\top})^{-\top}(A_{i} -B_{i}K_{i})\big]\cdot (\bI - \gamma^{-2} P_{K_{0}})^{-1}\cdot\prod^{t-1}_{i=0}\big[(A_{i} -B_{i}K_{i})^{\top}(\bI-\gamma^{-2} P_{K_{i+1}}D_iD_i^{\top})^{-1}\big] \\
	&+\sum_{\tau = 1}^{t}\bigg\{\prod^{t-1}_{i=\tau}\big[(\bI-\gamma^{-2} P_{K_{i+1}}D_iD_i^{\top})^{-\top}(A_{i} -B_{i}K_{i})\big]\cdot D_{\tau-1}(\bI - \gamma^{-2} D_{\tau-1}^{\top}P_{K_{\tau}}D_{\tau-1})^{-1}D_{\tau-1}^{\top}\cdot\prod^{t-1}_{i=\tau}\big[(A_{i} -B_{i}K_{i})^{\top}(\bI- \gamma^{-2}P_{K_{i+1}}D_iD_i^{\top})^{-1}\big]\bigg\},\\
	\Sigma_{K_t} &:= \prod^{t-1}_{i=0}\big[(\bI- \gamma^{-2}P_{K_{i+1}}D_iD_i^{\top})^{-\top}(A_{i} -B_{i}K_{i})(A_{i} -B_{i}K_{i})^{\top}(\bI-\gamma^{-2} P_{K_{i+1}}D_iD_i^{\top})^{-1}\big] \\
	&+ \sum_{\tau = 1}^{t}\bigg\{\prod^{t-1}_{i=\tau}\big[(\bI-\gamma^{-2} P_{K_{i+1}}D_iD_i^{\top})^{-\top}(A_{i} -B_{i}K_{i})\big]\cdot D_{\tau-1}D_{\tau-1}^{\top}\cdot\prod^{t-1}_{i=\tau}\big[(A_{i} -B_{i}K_{i})^{\top}(\bI-\gamma^{-2} P_{K_{i+1}}D_iD_i^{\top})^{-1}\big]\bigg\}.
	\end{align*} 
	\normalsize 
\end{lemma}
The proof of Lemma \ref{lemma:pg_mix} is deferred to \S\ref{proof:pg_mix}. Before moving on to the next section, we provide a remark regarding the challenges of addressing LEQG or the LQ disturbance attenuation problem directly using derivative-free PG methods.

\begin{remark}\label{rmk:challenge_LEQG_atten}
 It seems tempting to tackle LEQG or the LQ disturbance attenuation problem directly using derivative-free PG methods, e.g., vanilla PG or natural PG methods by sampling the system trajectories as in \cite{fazel2018global}. However, there are several challenges. First, when attempting to sample the LEQG objective \eqref{eqn:leqg_objective} using system trajectories (and then to estimate PGs), the bias of gradient estimates can be difficult to control uniformly with a fixed sample size per iterate, as the $\log$ function is not globally Lipschitz\footnote{One workaround for mitigating this bias might be to remove the $\log$ operator in the objective {\scriptsize \eqref{eqn:leqg_objective}}, and only minimize the terms after the $\EE\exp(\cdot)$ function. However, it is not clear yet if derivative-free methods provably converge for this objective, as $\exp$ function is neither globally smooth nor Lipschitz. We have left this direction in our future work, as our goal in the present work is to provide a unified way to solve all three classes of problems.}. Moreover, for the vanilla PG method, even with exact PG accesses, the iterates may not preserve a certain level of risk-sensitivity/disturbance attenuation, i.e., remain feasible, along the iterations, which can make the disturbance input drive the cost to arbitrarily large values (see the numerical examples in \cite{zhang2019policymixed} for the infinite-horizon LTI setting). This failure will only be exacerbated in the derivative-free setting with accesses to only noisy PG estimates.  Lastly, developing a derivative-free natural PG method (which we will show in  \S\ref{sec:double_update} that it can preserve a prescribed attenuation level along the iterations) is also challenging, because the expressions of $\Sigma_{K_t}$ in Lemmas \ref{lemma:pg_leqg} and \ref{lemma:pg_mix} cannot be sampled from system trajectories directly. Therefore, the game-theoretic approach to be introduced next is rather one workaround. 
\end{remark}	 

==> Mixed Design Arxiv v3/mixfree.tex <==
\xznote{need perturbation analaysis for K, Pk, L(K), and SigmaK.}
In this section, we analyze the sample complexity of random search algorithms for the outer loop problem. 





\begin{theorem}
	Let the stepsize and smoothing radius to satisfy $\alpha = \cO(M^{-2/3})$ and $r_{\bK} = \cO(M^{-1/6})$ and run the algorithm for $M = \cO(\epsilon_{\bK}^{-3}\Lambda^{-3})$ iterations. Then, the random search algorithm reaches the stationary point, such that $\|\nabla\cG(\bK_{M})\|^2 \leq \epsilon_{\bK}$, with probability greater than $1-\Lambda$. $\epsilon_{\bK} >0$ is the desired accuracy level and $\Lambda \in (0, 1)$.  
\end{theorem}
\begin{proof}
	Following from \cite{nesterov2017random}, the following properties holds for Gaussian-smoothed version of function $\cG(\bK)$, denoted as $\cG_{r_{\bK}}(\bK) := \EE[\cG(\bK+r_{\bK}U)]$,
	\begin{align}
		|\cG_{r_{\bK}}(\bK) - \cG(\bK)| &\leq r_{\bK}^2\psi_{\bK}\tilde{d}_{\bK} \label{eqn:cost_bound}\\
		\|\nabla\cG_{r_{\bK}}(\bK) - \nabla\cG(\bK)\| &\leq r_{\bK}\psi_{\bK}(\tilde{d}_{\bK} + 3)^{3/2} \label{eqn:grad_bound}
	\end{align}
	Also, the noisy gradient estimate $\overline{\nabla}\cG_{r_{\bK}}(\bK)$ satisfies that for all $\bK_k$,
	\begin{align}\label{eqn:unbiased_est}
		\EE~[\overline{\nabla}\cG_{r_{\bK}}(\bK_k)] = \nabla\cG_{r_{\bK}}(\bK_k)
	\end{align}
	where the expectation is taken over both the random process noise $\bm{\xi}$ and the Gaussian smoothing on the control gain matrix, $U$. Let the function $\cG_{r_{\bK}}(\bK, \bm{\xi}) \in C^{1, 1}$ with Lipschitz constant $\psi_{\bK}(\bm{\xi})$, we assume $\psi_{\bK}(\bm{\xi}) \leq \psi_{\bK}$. Then, we have
	\begin{align}
		\EE~[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2] &\leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + \|\nabla\cG_{r_{\bK}}(\bK_k)\|^2\nonumber\\
		&\leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + 2\|\nabla\cG(\bK_k)\|^2 + 2\|\nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\|\nonumber\\
		&\leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + 2\|\nabla\cG(\bK_k)\|^2 + 2r_{\bK}^2\psi_{\bK}^2(\tilde{d}_{\bK}+3)^3. \label{eqn:step2}
	\end{align}
	Following Lemma 1.2.3 of \cite{nesterov2013introductory}, we can obtain the following inequality
	\begin{align*}
		\cG_{r_{\bK}}(\bK_{k+1}) &\leq \cG_{r_{\bK}}(\bK_{k}) + \big\langle\nabla\cG_{r_{\bK}}(\bK_{k}), \bK_{k+1}-\bK_k \big\rangle + \frac{\psi_{\bK}}{2}\|\bK_{k+1} - \bK_k\|^2 \\
		&= \cG_{r_{\bK}}(\bK_{k}) -\alpha\big\langle\nabla\cG_{r_{\bK}}(\bK_{k}), \overline{\nabla}\cG_{r_{\bK}}(\bK_{k}) \big\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2 \\
		&=\cG_{r_{\bK}}(\bK_{k}) -\alpha\big\langle\nabla\cG_{r_{\bK}}(\bK_{k}), \overline{\nabla}\cG_{r_{\bK}}(\bK_{k})-\nabla\cG_{r_{\bK}}(\bK_{k}) \big\rangle -\alpha\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2 + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2
	\end{align*}
	By \eqref{eqn:unbiased_est},  we take expectation on both sides and rearrange terms. This leads to
	\begin{align*}
		\alpha\EE\big[\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big] \leq \EE\big[\cG_{r_{\bK}}(\bK_{k})\big] - \EE\big[\cG_{r_{\bK}}(\bK_{k+1})\big] + \frac{\psi_{\bK}\alpha^2}{2}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big]
	\end{align*}
	Summing the above inequality from 0 to $M-1$ and dividing both sides by $\alpha$ yields
	\begin{align}
		\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big] \leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \EE\big[\cG_{r_{\bK}}(\bK_{M})\big]}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] \nonumber\\
		\leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] \label{eqn:step1}
	\end{align}
	where $\cG_{r_{\bK}}(\bK^*)$ is the lower bound of the smoothed function $\cG_{r_{\bK}}(\bK)$, for which the existence is ensured because of the boundness of the original function $\cG(\bK)$ and \eqref{eqn:cost_bound}. Since
	\begin{align}
		\frac{1}{2}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \EE\big[\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big] + \EE\big[\|\nabla\cG(\bK_{k}) - \nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big],
	\end{align}
	we can combine \eqref{eqn:step1} and \eqref{eqn:grad_bound} to obtain
	\begin{align*}
		\frac{1}{2}\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] + r^2_{\bK}\psi^2_{\bK}(\tilde{d}_{\bK} + 3)^{3}M
	\end{align*}
	Also, from \eqref{eqn:step2}, we can derive 
	\begin{align}
		\sum^{M-1}_{k=0}\EE~[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2]  \leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k))M + 2\|\nabla\cG(\bK_k)\|^2M + 2r_{\bK}^2\psi_{\bK}^2(\tilde{d}_{\bK}+3)^3M.
	\end{align}
	Therefore, 
	\begin{align*}
		&\frac{1}{2}\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] + r^2_{\bK}\psi^2_{\bK}(\tilde{d}_{\bK} + 3)^{3}M \\
		&\hspace{1em}\leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} +\frac{\psi_{\bK}\alpha \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k))M}{2} + \psi_{\bK}\alpha\|\nabla\cG(\bK_0)\|^2M + (\psi_{\bK}\alpha+1)r^2_{\bK}\psi^2_{\bK}(\tilde{d}_{\bK} + 3)^{3}M 
	\end{align*}
	\xzedit{As the variance term can be bounded by 
	\begin{align*}
		\Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) \leq \Big(\frac{1}{r_{\bK}}~\sup_{\bK_k}~ (\overline{\cG}_{r_{\bK}}(\bK_k) + \epsilon_{\bL})\Big)^2
	\end{align*}
	almost surely, we can conclude that $\Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) = \cO(r_{\bK}^{-2}\epsilon_{\bL}^2)$}. Then, let the stepsize and the perturbation radius chosen to satisfy the order of $\alpha = \cO(M^{-2/3})$ and $r_{\bK} = \cO(M^{-1/6})$, we have
 	\begin{align}
 		\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \cO(M^{2/3}) + \cO(M^{2/3}\xzedit{\epsilon_{\bL}^2}) + \cO(M^{1/3}) + \cO(M^{2/3}) + \cO(1)
 	\end{align}
 	Dividing both sides by $M$, we can observe when $M = \cO(\epsilon_{\bK}^{-3}\Lambda^{-3})$ \xzedit{and $ \epsilon_{\bL} = o( \sqrt{\epsilon_{\bK}\Lambda})$ almost surely}, $\EE\big[\|\nabla\cG(\bK_{M})\|^2\big] \leq \epsilon_{\bK}\Lambda$. Applying Markov's inequality leads to 
 	\begin{align}
 		P\big\{\|\nabla\cG(\bK_{M})\|^2 \geq \epsilon_{\bK}\big\} \leq \frac{1}{\epsilon_{\bK}}\EE\big[\|\nabla\cG(\bK_{M})\|^2\big] \leq \Lambda.
 	\end{align}
 	This implies $P\big\{\|\nabla\cG(\bK_{M})\|^2 \leq \epsilon_{\bK}\big\} > 1-\Lambda$. The proof is completed.
\end{proof}

\xzedit{The total sample complexity scales as $\cO\big(\frac{1}{\epsilon_{\bK}^{3}\epsilon_{\bL}^2\Lambda^{3}\delta^{2}}\log(\frac{1}{\epsilon_{\bL}\delta})\big)$, where $ \epsilon_{\bL} = o( \sqrt{\epsilon_{\bK}\Lambda})$ almost surely.}
%\begin{proof}
%	For a positive smoothing radius $r_{\bK} > 0$, the smoothed function $\cG_{r_{\bK}}(\bK) := \EE[\cG(\bK+U)]$ with $\|U\|_F = r_{\bK}$ and the expectation is taken with respect to the combined randomness. The estimate of the gradient $\overline{\nabla}\cG_{r_{\bK}}$ at the point $\bK$ is given by $\overline{\nabla}\cG_{r_{\bK}}(\bK) = \frac{\tilde{d}_{\bL}}{r^2_{\bK}}\cG(\bK+U; \bm{\xi})U$, where each of the randomness $\{x_0, \xi_0, \dots, \xi_{N-1}\}$ of the system is sampled independently from the distribution $\cD$. Then, \cite{flaxman2005online, agarwal2010optimal, shamir2017optimal, malik2020derivative} suggests the following properties of the gradient estimate $\overline{\nabla}\cG_{r_{\bK}}$.
%	\begin{itemize}
%		\item $\nabla\cG_{r_{\bK}}(\bK) = \EE[\overline{\nabla}\cG_{r_{\bK}}(\bK)]$
%		\item $\|\nabla\cG_{r_{\bK}}(\bK) - \nabla\cG(\bK)\| \leq \psi_{\bK}r_{\bK}$
%%		\item  \quad $\|\nabla\cG_{r_{\bK}}(\bK)\|^2 \leq \|\nabla\cG(\bK)\|^2 +  \psi_{\bK}^2r_{\bK}^2$.
%	\end{itemize}
%	The proof is omitted for simplicity and we refer the readers to Appendix $C$ of \cite{malik2020derivative} for a complete justification. Since the gradient of the outer loop problem is $\psi_{\bK}$-Lipschitz, we have
%	\begin{align*}
%		\cG(\bK_{k+1}) - \cG(\bK_{k}) &\leq \big\langle \nabla\cG(\bK_k), \cG(\bK_{k+1}) - \cG(\bK_k)\big\rangle + \frac{\psi_{\bK}}{2}\|\cG(\bK_{k+1}) - \cG(\bK_k)\|^2 \\
%		&= - \alpha\big\langle \nabla\cG(\bK_k), \nabla\cG_{r_{\bK}}(\bK_k)\big\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2\\
%		&= -\alpha\|\nabla\cG(\bK_k)\|^2 - \alpha \langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2
%	\end{align*}
%	where the first equality follows from the first property above. Rearranging the terms yields
%	\begin{align*}
%		\alpha\|\nabla\cG(\bK_k)\|^2 &\leq \cG(\bK_{k}) - \cG(\bK_{k+1}) - \alpha \langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2
%	\end{align*}
%%	Then, utilizing the assumption of $\cG(\bK^*) \leq \cG(\bK_{k+1})$ leads to 
%%	\begin{align}
%%		\alpha \|\nabla\cG(\bK_k)\|^2 \leq \big(\cG(\bK_{k}) - \cG(\bK^*)\big) - \alpha \langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2
%%	\end{align}
%	Taking expectation of the randomness up to iteration $k$ on both sides yields
%	\small
%	\begin{align*}
%		\alpha \EE_k~\big[\|\nabla\cG(\bK_k)\|^2\big] \leq \cG(\bK_{k}) - \cG(\bK_{k+1}) - \alpha \EE_{k}~\big[\langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle\big] + \frac{\psi_{\bK}\alpha^2}{2}\EE_{k}~\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2\big]
%	\end{align*}
%	\normalsize
%	Also, similar to equation (3.20) of \cite{ghadimi2013stochastic} and the second to last equation on page 23 of \cite{malik2020derivative}, we can observe the following two conditions
%	\begin{align*}
%		&\EE_{k}~\big[\langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle\big] = 0\\
%		&\EE_{k}~\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2\big] = \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + \EE_{k}~\big[\|\nabla\cG_{r_{\bK}}(\bK_k)\|^2\big] \\
%%		&\hspace{2em} \leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + 2\|\nabla\cG(\bK_k)\|^2 + 2\|\nabla\cG_{r_{\bK}}(\bK_k)- \nabla\cG(\bK_k)\|^2\\
%		&\hspace{2em} \leq G_2 + 2\EE_{k}~\|\nabla\cG(\bK_k)\|^2 + 2(\psi_{\bK}r_{\bK})^2.
%	\end{align*}
%	Therefore, applying the conditions leads to
%	\begin{align*}
%		\alpha \EE_k~\big[\|\nabla\cG(\bK_k)\|^2\big] &\leq \cG(\bK_{k}) - \cG(\bK_{k+1}) + \frac{\psi_{\bK}\alpha^2}{2}\big(G_2 + 2\EE_{k}~\|\nabla\cG(\bK_k)\|^2 + 2(\psi_{\bK}r_{\bK})^2\big) \\
%		(\alpha - \psi_{\bK}\alpha^2)\EE_k~\big[\|\nabla\cG(\bK_k)\|^2\big] & \leq \cG(\bK_{k}) - \cG(\bK_{k+1}) +  \frac{\psi_{\bK}\alpha^2}{2}\big(G_2 + 2(\psi_{\bK}r_{\bK})^2\big)
%	\end{align*}
%	Since $\alpha \leq \frac{1}{2\psi_{\bK}}$, we have $\sum^{\cK}_{k=0}(\alpha - \psi_{\bK}\alpha^2) = \cK\alpha(1-\psi_{\bK}\alpha) \geq \frac{\cK\alpha}{2}$. Then, summing over $\cK$ and dividing both sides by $\sum^{\cK}_{k=0}(\alpha - \psi_{\bK}\alpha^2)$ yields
%	\begin{align*}
%		 (\alpha - \psi_{\bK}\alpha^2)\sum^{\cK}_{k=0}\EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] &\leq \Delta_0  + \frac{\psi_{\bK}\alpha^2}{2}\sum^{\cK}_{k=0}\big(G_2 + 2(\psi_{\bK}r_{\bK})^2\big) \\
%		\Rightarrow \EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] &\leq \frac{2\Delta_0}{\cK\alpha}  + \psi_{\bK}\alpha\big(G_2 + 2(\psi_{\bK}r_{\bK})^2\big)\\
%		 &\leq \frac{2\Delta_0}{\cK\alpha}  + \psi_{\bK}\alpha G_2 + 2\psi^3_{\bK}r_{\bK}^2\alpha\\
%		 &\leq \frac{2\Delta_0}{\cK}\max\big\{2\psi_{\bK}, G_2\psi_{\bK}\sqrt{\cK}\big\}  + \frac{1}{\sqrt{\cK}}  + \frac{1}{\sqrt{\cK}} + \psi^2_{\bK}r_{\bK}^2 
%	\end{align*}
%	where the last inequality follows from the requirements of $\alpha$ in \eqref{eqn:one_point_req_K}. Then, since $r_{\bK} \leq \frac{1}{\psi_{\bK}\sqrt{\cK}}$, 
%	\begin{align*}
%		\frac{2\Delta_0}{\cK}\max\big\{2\psi_{\bK}, G_2\psi_{\bK}\sqrt{\cK}\big\}  + \frac{1}{\sqrt{\cK}} + \psi^2_{\bK}r_{\bK}^2 &\leq \frac{2\Delta_0}{\cK}\big[2\psi_{\bK}+  G_2\psi_{\bK}\sqrt{\cK}\big]  + \frac{1}{\sqrt{\cK}} + \frac{1}{\cK}\\
%		&= \frac{4\Delta_0\psi_{\bK}+1}{\cK} + \frac{G_2\psi_{\bK}}{\sqrt{\cK}} + \frac{1}{\sqrt{\cK}}.
%	\end{align*}
%	Subsequently, we provide a bound for $G_2$. By definition of the estimated cost function, their exists an absolute constant $c_2$ such that \xznote{in two point, G2 is a constant, in one point, G2 is more complicated, and needs to depend on epsilon, thus ck}
% 	\begin{align*}
% 		\cG(\bK + U, \bm{\xi}) = \bm{\xi}^T\bP_{\bK + U}\bm{\xi} \leq s\sigma^2 \EE_{\bm{\xi}} [\bm{\xi}^T\bm{\xi}]~ \|\bP_{\bK + U}\| \leq s\sigma^2c_{2}.
% 	\end{align*}
% 	Therefore, as $\|U\|_F = r_{\bK}$, we can prove the following bound
% 	\begin{align*}
% 		G_{\infty} = \frac{\tilde{d}_{\bK}}{r_{\bK}}~\sup_{\bK+U}~ \overline{\cG} \leq \frac{s\sigma^2\tilde{d}_{\bK}c_{2}}{r_{\bK}}, \quad G_2 \leq G^2_{\infty} \leq \Big(\frac{s\sigma^2\tilde{d}_{\bK}c_{2}}{r_{\bK}}\Big)^2 \leq \Big(\frac{s\sigma^2\tilde{d}_{\bK}c_{2}}{r_{\bK}}\Big)^2
% 	\end{align*}
%	Then, it can be seen that choosing a $\cK$ with the order of $\cO(\epsilon^{2}_{\bK})$. Then, the 
%	 ensures that $\EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] \leq \epsilon_{\bK}\Lambda$. Then, applying Markov's inequality yields 
%	\begin{align}
%		P\big\{\|\nabla\cG(\bK_{\cK})\|^2 \geq \epsilon_{\bK}\big\} \leq \frac{1}{\epsilon_{\bK}}\EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] \leq \Lambda.
%	\end{align}
%	This implies $P\big\{\|\nabla\cG(\bK_{\cK})\|^2 \leq \epsilon_{\bK}\big\} > 1-\Lambda$.  	Substitute the bounds into the requirements of $\alpha$ completes the proof of the theorem.
%%	Also, as the cost function of the outer loop problem is smooth, we have
%%	\begin{align}
%%		(\theta_{\bK} - \theta_{\bK}^2\psi_{\bK}/2)\|\nabla\cG(\bK_k)\|^2 \leq \cG(\bK_k) - \cG(\bK_k - \theta_{\bK}\nabla\cG(\bK_k)) \leq \cG(\bK_k) - \cG(\bK^*),
%%	\end{align}
%%	for $\theta_{\bK} = \min\{\frac{1}{2\psi_{\bK}}, \frac{1}{l_{\bK}}\}$. Then, define $\Delta_k := \cG(\bK_k) - \cG(\bK^*)$ to be the optimality gap at iteration $k$. Then, 
%%	\begin{align}
%%	\EE_k[\Delta_{k+1} - \Delta_k] &\leq -\alpha\|\nabla\cG(\bK_k)\|^2 + \frac{2\alpha\psi_{\bK}r_{\bK}}{\theta_{\bK}}\Delta^{1/2}_k + \frac{\psi_{\bK}\alpha^2}{2}G_2 +  \psi_{\bK}\alpha^2\big(\|\nabla\cG(\bK_k)\|^2 + (\psi_{\bK}r_{\bK})^2\big) \\
%%	&\leq -\frac{\alpha}{2}\|\nabla\cG(\bK_k)\|^2+ \frac{2\alpha\psi_{\bK}r_{\bK}}{\theta_{\bK}}\Delta^{1/2}_k + \frac{\psi_{\bK}\alpha^2}{2}G_2 + \alpha^2\psi_{\bK}^3r_{\bK}^2 \\
%%	&\leq -\frac{\alpha}{2}\|\nabla\cG(\bK_k)\|^2+\Delta_k + \frac{\alpha^2\psi^2_{\bK}r_{\bK}^2}{\theta^2_{\bK}} + \frac{\psi_{\bK}\alpha^2}{2}G_2 + \alpha^2\psi_{\bK}^3r_{\bK}^2
%%	\end{align}
%%	\xznote{alsdhfliashdgfashdfoah}
%%	where the second inequality follows from $\alpha \leq \frac{1}{2\psi_{\bK}}$ and the last inequality follows from the inequality $2ab \leq a^2+b^2$ for any pair of $(a, b)$. 
%\end{proof}

==> Mixed Design Arxiv v3/modelfree.tex <==
We present the sample complexity of our double-loop algorithm, when the exact PG is not accessible, and can only be estimated through samples of system trajectories. In particular, we propose a zeroth-order NPG (ZO-NPG) algorithm with a (zeroth-order) maximization oracle that approximately solves the inner-loop subproblem (cf. Algorithms \ref{alg:model_free_inner_PG} and \ref{alg:model_free_outer_NPG}). In the following Remark, we comment on how to construct Algorithms \ref{alg:model_free_inner_PG} and \ref{alg:model_free_outer_NPG} when explicit knowledge on the system parameters is not available.

\begin{remark}\label{remark:input}
	When solving LEQG and LQ disturbance attenuation (LQDA) problems using the proposed double-loop derivative-free PG methods (cf. Algorithms \ref{alg:model_free_inner_PG} and \ref{alg:model_free_outer_NPG}), we exploited the equivalence relationships in Lemma \ref{lemma:equivalent} to construct and solve an equivalent zero-sum LQ game. We comment on how to construct such an equivalent game problem in the model-free setting where only oracle-level accesses to the LEQG and LQDA models are available. 
	
	Suppose that one would like to solve the LQDA problem by solving the equivalent zero-sum game; then, the only information needed is oracle-level accesses to the LQDA model (cf. \S\ref{sec:mix}). In particular, for a fixed sequence of gains $K_t$ and any sequence of disturbances $w_t$, we assume that this LQDA oracle can return the $\|z\|$ as defined in \S\ref{sec:mix}. Then, the LQDA oracle with an additionally injected sequence of independent Gaussian noise (with any positive definite covariance matrix) suffices to serve as the oracle for our double-loop derivative-free PG algorithms (for the stochastic game). Therefore, no explicit knowledge on the system parameters ($A_t$, $B_t$, $D_t$, $C_t$, $E_t$, $\gamma$) is needed.
	
	However, if one would like to solve the LEQG problem by solving an equivalent zero-sum game, one will need knowledge of $W$ (to build-up the black-box sampling oracle/simulator, but still, the exact value of $W$ is not revealed to the learning agent) in addition to oracle-level accesses to the original LEQG model (cf. \S\ref{sec:leqg}). Also, explicit knowledge of the parameters ($A_t$, $B_t$, $Q_t$, $R_t$, $\beta$) is not required. We would like to note that the assumption on the knowledge (and/or the availability of the estimate) of $W$ is reasonable for a large family of control applications where system dynamics and disturbance can be studied separately. For example, consider the risk-sensitive control of a wind turbine. The turbine dynamics and the wind information can be gathered separately. One can identify $W$ by looking at the past wind data. Similar situations hold for many aerospace applications where the properties of process noise (e.g. wind gust) can be estimated beforehand.
\end{remark}
 
 
\subsection{Inner-Loop Maximization Oracle}\label{sec:max_oracle}
Sample complexities of zeroth-order PG algorithms for solving standard infinite-horizon LQR have been investigated in both discrete-time \cite{fazel2018global, malik2020derivative,mohammadi2020linear} and continuous-time \cite{mohammadi2019convergence} settings. Our inner-loop maximization oracle extends the sample complexity result to finite-horizon time-varying LQR with system noises and a possibly \emph{indefinite} state-weighting matrix. In particular, we show that zeroth-order PG and NPG with a one-point minibatch estimation scheme enjoy $\tilde{\cO}(\epsilon_1^{-2})$ sample complexities, where $\epsilon_1$ is the desired accuracy level in terms of inner-loop objective values, i.e., $\cG(\bK, \overline{\bL}(\bK)) \geq \cG(\bK, \bL(\bK))-\epsilon_1$ for the $\overline{\bL}(\bK)$ returned by the algorithm. The two specific zeroth-order PG updates are introduced as follows:
\begin{align}
	\text{Zeroth-Order PG: } \quad \bL_{l+1} &= \bL_l + \eta\overline\nabla_{\bL}\cG(\bK, \bL_l) \label{eqn:pg_free_L}, \\
	\text{Zeroth-Order Natural PG: } \quad \bL_{l+1} &= \bL_l + \eta\overline\nabla_{\bL}\cG(\bK, \bL_l)\overline{\Sigma}^{-1}_{\bK, \bL_l}, \label{eqn:npg_free_L} 
\end{align}
where $\eta > 0$ is the stepsize to be chosen, $l \in \{0, \cdots, L-1\}$ is the iteration index, $\overline{\nabla}_{\bL} \cG(\bK, \bL)$ and $\overline{\Sigma}_{\bK, \bL}$ are the noisy estimates of $\nabla_{\bL}\cG(\bK, \bL)$ and $\Sigma_{\bK, \bL}$, respectively, obtained through zeroth-order oracles. The procedure of our inner-loop maximization oracle is presented in Algorithm \ref{alg:model_free_inner_PG} and we formally establish its sample  complexity in the following theorems. 
 
\begin{algorithm}[t]
	\caption{~Inner-Loop Zeroth-Order Maximization Oracle} 
	\label{alg:model_free_inner_PG}
	\begin{algorithmic}[1]
		\STATE Input: gain matrices ($\bK$, $\bL_0$), iteration $L$, batchsize $M_{1}$, problem horizon $N$, distribution $\cD$, smoothing radius $r_1$, dimension $d_1 =mnN$, stepsize $\eta$. 
		\FOR{$l = 0, \cdots, L-1$}
		\FOR{$i = 0, \cdots, M_1-1$}
		\STATE Sample $\bL^i_l = \bL_l + r_1\bU^i_l$, where $\bU^i_l$ is uniformly drawn from $\cS(n,m,N)$ with $\|\bU^i_l\|_F=1$. 
		\STATE Simulate ($\bK, \bL^i_l$) and ($\bK, \bL_l$) for horizon $N$ starting from $x^{i, 0}_{l, 0}, x^{i, 1}_{l, 0}\sim \cD$, and collect the empirical estimates $\overline{\cG}(\bK, \bL^i_l) = \sum_{t=0}^N c^{i, 0}_{l, t}$, $\overline{\Sigma}^i_{\bK, \bL_l} = diag\big[x^{i, 1}_{l, 0}(x^{i, 1}_{l, 0})^{\top}, \cdots, x^{i, 1}_{l, N}(x^{i, 1}_{l, N})^{\top}\big]$, where $\big\{c^{i, 0}_{l, t}\big\}$ is the sequence of stage costs following the trajectory generated by $(\bK, \bL^{i}_l)$ and $\big\{x^{i, 1}_{l, t}\big\}$ is the sequence of states following the trajectory generated by $(\bK, \bL_l)$, for $t\in\{0,\cdots,N\}$, under independently sampled noises $\xi^{i, 0}_{l, t}, \xi^{i, 1}_{l, t} \sim \cD$ for all $t\in\{0,\cdots,N-1\}$.
		\ENDFOR
  \STATE Obtain the estimates: $~~\overline{\nabla}_{\bL}
  \cG(\bK, \bL_l) = \frac{1}{M_1} \sum^{M_1-1}_{i=0}\frac{d_1}{r_1}\overline{\cG}(\bK, \bL^i_l) \bU^i_l$, \quad $\overline{\Sigma}_{\bK, \bL_l} = \frac{1}{M_1}\sum^{M_1-1}_{i=0}\overline{\Sigma}^i_{\bK, \bL_l}$.\vspace{0.3em}
			\STATE Execute one-step update:~~ \emph{PG}:~~ $\bL_{l+1} = \bL_{l} + \eta\overline{\nabla}_{\bL}\cG(\bK, \bL_l)$, \quad \emph{NPG}:~~ $\bL_{l+1} = \bL_{l} + \eta\overline{\nabla}_{\bL}\cG(\bK, \bL_l)\overline{\Sigma}^{-1}_{\bK, \bL_l}$.
		\ENDFOR
		\STATE Return $\bL_L$.
	\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{theorem:free_pg_L}(Inner-Loop Sample Complexity for PG)
	For a fixed $\bK\in \cK$ and an arbitrary $\bL_0$ that induces a finite $\cG(\bK, \bL_0)$, define a superlevel set $\cL_{\bK}(a)$ as in \eqref{eqn:levelset_L}, where $a \leq  \cG(\bK, \bL_0)$ is an arbitrary constant. Let  $\epsilon_1, \delta_1 \in (0, 1)$, and $M_1, r_1, \eta >0$ in Algorithm \ref{alg:model_free_inner_PG} satisfy
	\begin{align*}
		M_1 \geq \left(\frac{d_1}{r_1}\Big(\cG(\bK, \bL(\bK)) + \frac{l_{\bK, a}}{\rho_{\bK, a}}\Big)\sqrt{\log\Big(\frac{2d_1L}{\delta_1}\Big)}\right)^2\frac{1024}{\mu_{\bK}\epsilon_1},
		\end{align*}
		\vspace{-1.5em}
		\begin{align*}
		 r_1 \leq \min\bigg\{\frac{\theta_{\bK, a} \mu_{\bK}}{8\psi_{\bK, a}}\sqrt{\frac{\epsilon_1}{240}},~ \frac{1}{8\psi^2_{\bK,a}}\sqrt{\frac{\epsilon_{1}\mu_{\bK}}{30}},~\rho_{\bK, a}\bigg\}, \quad \eta \leq \min\left\{1, ~\frac{1}{8\psi_{\bK,a}}, ~\rho_{\bK, a}\cdot\Big[\frac{\sqrt{\mu_{\bK}}}{32} + \psi_{\bK, a} + l_{\bK, a}\Big]^{-1}\right\},
	\end{align*}
 	where $\theta_{\bK, a} = \min\big\{1/[2\psi_{\bK, a}], \rho_{\bK, a}/l_{\bK, a}\big\}$; $l_{\bK, a}, \psi_{\bK, a}, \mu_{\bK}$ are defined in Lemma \ref{lemma:landscape_L}; $\rho_{\bK, a}:=\min_{\bL\in\cL_{\bK}(a)}\rho_{\bK, \bL}>0$; and $d_1 = nmN$. Then, with probability at least $1 - \delta_1$ and a total number of iterations $L = \frac{8}{\eta \mu_{\bK}}\log(\frac{2}{\epsilon_1})$, the inner-loop ZO-PG update \eqref{eqn:pg_free_L} outputs some $\overline{\bL}(\bK) := \bL_L$ such that $\cG(\bK, \overline{\bL}(\bK)) \geq \cG(\bK, \bL(\bK)) - \epsilon_1$, and  $\|\bL(\bK) - \overline{\bL}(\bK)\|_F \leq \sqrt{\lambda^{-1}_{\min}(\bH_{\bK, \bL(\bK)}) \cdot \epsilon_1}$.
\end{theorem}

The proof of Theorem \ref{theorem:free_pg_L} is deferred to \S\ref{proof:free_pg_L}. The total sample complexity of the inner-loop ZO-PG algorithm scales as $M_1\cdot L \sim \tilde{\cO}(\epsilon_1^{-2}\cdot\log(\delta_1^{-1}))$, where the logarithmic dependence  on $\epsilon_1$ is suppressed. Next, we present the sample complexity of the inner-loop ZO-NPG algorithm \eqref{eqn:npg_free_L}, with its proof being provided in \S\ref{proof:free_npg_L}. 

 \begin{theorem}\label{theorem:free_npg_L}(Inner-Loop Sample Complexity for NPG)
 For a fixed $\bK\in \cK$ and an arbitrary $\bL_0$ that induces a finite $\cG(\bK, \bL_0)$, define a superlevel set $\cL_{\bK}(a)$ as in \eqref{eqn:levelset_L}, where $a \leq  \cG(\bK, \bL_0)$ is an arbitrary constant. Let  $\epsilon_1, \delta_1 \in (0, 1)$, and $M_1, r_1, \eta >0$ in Algorithm \ref{alg:model_free_inner_PG} satisfy
	\begin{align*}
	M_1 \geq \max\left\{\Big(\cG(\bK, \bL(\bK)) + \frac{l_{\bK, a}}{\rho_{\bK, a}}\Big)^2\cdot\frac{64d_1^2(\overline{\varkappa}_a+1)^2}{\phi^2r_{1}^2\mu_{\bK}\epsilon_1}, \frac{2\overline{\varkappa}_a^2}{\phi^2}\right\}\cdot\log\Big(\frac{4L\max\{d_1, d_{\Sigma}\}}{\delta_1}\Big), 
	\end{align*}
	\vspace{-1.5em}
	\begin{align*}
	r_{1} \leq \min\left\{\frac{\phi\sqrt{\mu_{\bK}\epsilon_1}}{16\overline{\varkappa}_a\psi_{\bK, a}}, \frac{\phi\mu_{\bK}\theta_{\bK, a}\sqrt{\epsilon_1/2}}{32\overline{\varkappa}_a\psi_{\bK, a}}, \rho_{\bK, a}\right\}, ~ \eta \leq \min\bigg\{\frac{\phi^2}{32\psi_{\bK, a}\overline{\varkappa}_a}, ~\frac{1}{2\psi_{\bK, a}}, ~\rho_{\bK, a}\cdot\Big[\frac{\sqrt{\mu_{\bK}}}{4(\underline{\varkappa}_a+1)} + \frac{2\psi_{\bK, a}}{\phi} + l_{\bK, a} +\frac{\phi l_{\bK, a}}{2}\Big]^{-1}\bigg\},
\end{align*}
 	where $\theta_{\bK, a} = \min\big\{1/[2\psi_{\bK, a}], \rho_{\bK, a}/l_{\bK, a}\big\}$; $l_{\bK, a}, \psi_{\bK, a}, \mu_{\bK}$ are defined in Lemma \ref{lemma:landscape_L}; $\rho_{\bK, a}, \overline{\varkappa}_a, \underline{\varkappa}_a$ are uniform constants over $\cL_{\bK}(a)$ defined in \S\ref{proof:free_npg_L}; $d_{\Sigma} = m^2(N+1)$; and $d_1 = nmN$. Then, with probability at least $1 - \delta_1$ and a total number of iterations $L = \frac{8\overline{\varkappa}_a}{\eta \mu_{\bK}}\log(\frac{2}{\epsilon_1})$, the inner-loop ZO-NPG update \eqref{eqn:npg_free_L} outputs some $\overline{\bL}(\bK) := \bL_L$ such that $\cG(\bK, \overline{\bL}(\bK)) \geq \cG(\bK, \bL(\bK)) - \epsilon_1$, and  $\|\bL(\bK) - \overline{\bL}(\bK)\|_F \leq \sqrt{\lambda^{-1}_{\min}(\bH_{\bK, \bL(\bK)}) \cdot \epsilon_1}$.
\end{theorem}
Similar to \eqref{eqn:pg_free_L}, the ZO-NPG algorithm \eqref{eqn:npg_free_L} also has a $\tilde{\cO}(\epsilon_1^{-2}\cdot\log(\delta_1^{-1}))$ total sample complexity. Different from \cite{fazel2018global}, our Algorithm \ref{alg:model_free_inner_PG} uses an \emph{unperturbed} pair of gain matrices to generate the state sequence for estimating the correlation matrix $\Sigma_{\bK, \bL}$. This modification avoids the estimation bias induced by the perturbations on the gain matrix, while only adding a constant factor of $2$ to the total sample complexity. 


\subsection{Outer-Loop ZO-NPG}
With the approximate inner-loop solution $\overline{\bL}(\bK)$ obtained from Algorithm \ref{alg:model_free_inner_PG}, the outer-loop ZO-NPG algorithm approximately solves the constrained minimization problem $\min_{\bK \in \cK}\cG(\bK, \overline{\bL}(\bK))$, with the following update rule:
\begin{align}
	\text{Zeroth-Order Natural PG: } \quad \bK_{k+1} &= \bK_k - \alpha \overline{\nabla}_{\bK}
   \cG(\bK_k,\overline{\bL}(\bK_k))\overline{\Sigma}^{-1}_{\bK_k, \overline{\bL}(\bK_k)},\label{eqn:npg_free_K} 
\end{align}
where $\alpha>0$ is the stepsize, $k \geq 0$ is the iteration index, and $\overline{\nabla}_{\bK} \cG(\bK,\overline{\bL}(\bK))$ and $\overline{\Sigma}_{\bK, \overline{\bL}(\bK)}$ are the estimated PG and state correlation matrices, obtained from Algorithm \ref{alg:model_free_outer_NPG}. Similar to the modification in \S\ref{sec:max_oracle}, we estimate the correlation matrix $\overline{\Sigma}(\bK, \bL(\bK))$ using the state sequence generated by the \emph{unperturbed} gain matrices, $(\bK, \overline{\bL}(\bK))$, to avoid the estimation bias induced by the perturbations on the gain matrices. In the following theorem, whose proof is deferred to \S\ref{proof:free_IR} and a short sketch is provided below, we first prove that the implicit regularization studied in Theorem \ref{theorem:ir_K} also holds in the derivative-free setting, with high probability. 

\begin{algorithm}[t]
	\caption{~Outer-Loop ZO-NPG with Maximization Oracle} 
	\label{alg:model_free_outer_NPG}
	\begin{algorithmic}[1]
		\STATE Input: initial gain matrix $\bK_0 \in \cK$, number of iterates $K$, batchsize $M_2$, problem horizon $N$, distribution $\cD$, smoothing radius $r_2$, dimension $d_2=mdN$, stepsize $\alpha$. 
		\FOR{$k = 0, \cdots, K-1$}
		\STATE Find $\overline{\bL}(\bK_k)$ such that $\cG(\bK_k, \overline{\bL}(\bK_k)) \geq \cG(\bK_k, \bL(\bK_k)) - \epsilon_1$.
		\FOR{$j = 0, \cdots, M_2-1$}
		\STATE Sample $\bK^j_k = \bK_k+r_2\bV^j_k$, where $\bV^j_k$ is uniformly drawn from $\cS(d, m, N)$ with $\|\bV^j_k\|_F = 1$.
        \STATE Find $\overline{\bL}(\bK^j_k)$ such that $\cG(\bK^j_k, \overline{\bL}(\bK^j_k)) \geq \cG(\bK^j_k, \bL(\bK^j_k)) - \epsilon_1$ using Algorithm \ref{alg:model_free_inner_PG}. 
		\STATE Simulate $(\bK^j_k, \overline{\bL}(\bK^j_k))$ and $(\bK_k, \overline{\bL}(\bK_k))$ for horizon $N$ starting from $x^{j, 0}_{k, 0}, x^{j, 1}_{k, 0}\sim \cD$, and collect $\overline{\cG}(\bK^j_k, \overline{\bL}(\bK^j_k)) = \sum_{t=0}^N c^{j, 0}_{k, t}$, $\overline{\Sigma}^j_{\bK_k, \overline{\bL}(\bK_k)} = diag\big[x^{j, 1}_{k, 0}(x^{j, 1}_{k, 0})^{\top}, \cdots, x^{j, 1}_{k, N}(x^{j, 1}_{k, N})^{\top}\big]$, where $\big\{c^{j, 0}_{k, t}\big\}$ is the sequence of stage costs following the trajectory generated by $(\bK^j_k, \overline{\bL}(\bK^j_k))$ and $\big\{x^{j, 1}_{k, t}\big\}$ is the sequence of states following the trajectory generated by $(\bK_k, \overline{\bL}(\bK_k))$, for $t\in\{0,\cdots,N\}$, under independently sampled noises $\xi^{j, 0}_{k, t}, \xi^{j, 1}_{k, t} \sim \cD$ for all $t \in\{0,\cdots,N-1\}$. 
		\ENDFOR
		\STATE Obtain the estimates: ~~$\overline{\nabla}_{\bK}
   \cG(\bK_k,\overline{\bL}(\bK_k)) = \frac{1}{M_2} \sum^{M_2-1}_{j=0}\frac{d_2}{r_2}\overline{\cG}(\bK^j_k, \overline{\bL}(\bK^j_k)) \bV^j_k$, \quad $\overline{\Sigma}_{\bK_k, \overline{\bL}(\bK_k)} = \frac{1}{M_2}\sum^{M_2-1}_{j=0}\overline{\Sigma}^j_{\bK_k, \overline{\bL}(\bK_k)}$.\vspace{0.3em}
\STATE Execute one step \emph{NPG} update:~~ 
		$\bK_{k+1} = \bK_k -\alpha \overline{\nabla}_{\bK}
   \cG(\bK_k,\overline{\bL}(\bK_k))\overline{\Sigma}^{-1}_{\bK_k, \overline{\bL}(\bK_k)}$.
		\ENDFOR
		\STATE Return $\bK_{K}$.	
		\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{theorem:free_IR}(Implicit Regularization: Derivative-Free Setting)
	For any $\bK_0 \in \cK$ and defining $\zeta:=\lambda_{\min}(\bH_{\bK_0, \bL(\bK_0)}) >0$,  introduce the following set $\widehat{\cK}$:
	\begin{align}\label{eqn:widehatck_main}
 	\widehat{\cK} := \Big\{\bK \mid \eqref{eqn:DARE_black_L} \text{ admits a solution } \bP_{\bK, \bL(\bK)}\geq 0, \text{~and } \bP_{\bK, \bL(\bK)} \leq \bP_{\bK_0, \bL(\bK_0)} + \frac{\zeta}{2\|\bD\|^2}\cdot\bI\Big\} \subset \cK. 
 \end{align}
 Let $\delta_2 \in (0, 1)$ and other parameters in Algorithm \ref{alg:model_free_outer_NPG} satisfy $\delta_1 \leq \delta_2/[6M_2K]$ and
  \small
  \begin{align}
    M_2  &\geq \max\left\{\frac{128d_2^2\alpha^2c_0^2\widehat{\cG}(\bK, \bL(\bK))^2}{r_2^2\phi^4\varpi^2}, \frac{512d_2^2\alpha^2(\widehat{\cG}(\bK, \bL(\bK)) + r_2\cB_{\bP}c_0)^2}{r_2^2\phi^2\varpi^2}, \frac{32\alpha^2(\widehat{c}_{5, \bK})^2(\widehat{c}_{\Sigma_{\bK, \bL(\bK)}})^2}{\phi^2\varpi^2}, \frac{8(\widehat{c}_{\Sigma_{\bK, \bL(\bK)}})^2}{\phi^2}\right\} \cdot\log\bigg(\frac{12K\max\{d_2, d_{\Sigma}\}}{\delta_2}\bigg), \nonumber\\
    \epsilon_1 &\leq \min\left\{\frac{\phi\varpi r_2}{16\alpha d_2}, \frac{\widehat{\cB}_{1, \bL(\bK)}^2\zeta}{2}, \frac{\phi^2\varpi^2 \zeta}{128\alpha^2(\widehat{c}_{5, \bK})^2\widehat{\cB}_{\Sigma, \bL(\bK)}^2}, \frac{\phi^2 \zeta}{32\widehat{\cB}_{\Sigma, \bL(\bK)}^2}\right\}, ~~~ r_2 \leq \min\Big\{\varpi, \frac{\phi\varpi}{64\alpha  \widehat{c}_{5, \bK}(\widehat{c}_{\Sigma_{\bK, \bL(\bK)}} +\widehat{\cB}_{\Sigma, \bK})}, \frac{\phi\varpi}{64\alpha \widehat{c}_{2, \bK}\widehat{\cB}_{\Sigma, \bK}}\Big\}, \nonumber\\
    \alpha &\leq \frac{1}{2}\cdot\big\|\bR^u + \bB(\overline{\bP} + \overline{\bP}\bD(\bR^w - \bD^{\top}\overline{\bP}\bD)^{-1}\bD^{\top}\overline{\bP})\bB\big\|^{-1}, \qquad \quad   \overline{\bP} := \bP_{\bK_0, \bL(\bK_0)} + \frac{\zeta}{2\|\bD\|^2}\cdot\bI, \label{eqn:ir_free_req}
\end{align}
\normalsize
where $\widehat{\cG}(\bK, \bL(\bK)), \widehat{c}_{2, \bK}, \widehat{c}_{5, \bK}, \widehat{c}_{\Sigma_{\bK, \bL(\bK)}}, \widehat{\cB}_{\Sigma, \bK}, \widehat{\cB}_{1, \bL(\bK)}, \widehat{\cB}_{\Sigma, \bL(\bK)}, \varpi >0$ are uniform constants over $\widehat{\cK}$ defined in \S\ref{proof:free_IR}. Then, it holds with probability at least $1-\delta_2$ that $\bK_k \in \widehat{\cK} \subset \cK$ for all $k \in \{1, \cdots, K\}$.
\end{theorem}

\begin{SCfigure}
 \centering
\includegraphics[width=0.45\textwidth]{plots/proof_sketch.png}
\hspace{1em}
\caption{Illustrating the proof idea for Theorem \ref{theorem:free_IR}. Starting with any $\bK_0\hspace{-0.1em}\in\hspace{-0.1em}\cK$, we can construct two compact sets $\widehat{\cK}$ and $\cK_0$ as shown in blue and red, respectively, that are independent of the contour lines of the objective function. Our analysis proves that the iterates following \eqref{eqn:npg_free_K} stay within $\widehat{\cK}$ with high probability, thus also uniformly separated from $\partial\cK$, with high probability.}
\label{fig:proof2}
\end{SCfigure}

\noindent \textit{Proof Sketch.} Due to lack of coercivity, the objective function of the outer loop can no longer act as a barrier function to guarantee that the iterates of PG updates stay in $\cK$ (cf. Figure \ref{fig:landscape}), and thus new candidates are needed. To this end, we construct two compact sets $\widehat{\cK}$ and $\cK_0$ for a given $\bK_0 \hspace{-0.15em}\in\hspace{-0.15em}\cK$, that are shown in blue and red in Figure \ref{fig:proof2}, respectively, where $\cK_0 \hspace{-0.1em}:=\hspace{-0.1em} \big\{\bK \hspace{-0.1em}\mid\hspace{-0.1em} \bK \in \cK, \text{~and } \bP_{\bK, \bL(\bK)} \hspace{-0.1em}\leq \hspace{-0.1em}\bP_{\bK_0, \bL(\bK_0)}\hspace{-0.1em}\big\}\hspace{-0.1em}\hspace{-0.1em}$. Clearly, $\bK_0 \hspace{-0.1em}\in\hspace{-0.1em} \partial \cK_0$ and a sequence of iterates $\{\bK_k\}$ that stays in $\widehat{\cK}$ or $\cK_0$ is also uniformly separated from $\partial\cK$ (dashed lines in Figure \ref{fig:proof2}). Denote the gain matrix after one step of the exact NPG update \eqref{eqn:npg_K} as $\tilde{\bK}_1$. Then, under the appropriate stepsize, the IR property in Theorem \ref{theorem:ir_K} demonstrates that $\bP_{\tilde{\bK}_1, \bL(\tilde{\bK}_1)}\hspace{-0.1em}\geq\hspace{-0.1em} 0$ exists and satisfies $\bP_{\tilde{\bK}_1, \bL(\tilde{\bK}_1)} \hspace{-0.1em}\leq \hspace{-0.1em}\bP_{\bK_0, \bL(\bK_0)}$ almost surely, which also means that $\tilde{\bK_1} \hspace{-0.1em}\in\hspace{-0.1em}\cK_0$ almost surely. In contrast, when the model is not known, one step of the ZO-NPG update \eqref{eqn:npg_free_K} using estimated gradients sampled through system trajectories could drive the gain matrix outside of $\cK_0$ (even worse, outside of $\cK$) due to the induced statistical errors. Moreover, these errors accumulate over all the iterations, raising significant challenges to find a uniform ``margin'' for safely selecting the parameters of Algorithm \ref{alg:model_free_outer_NPG}.

To overcome this challenge, we establish some argument stronger than that in Theorem \ref{theorem:ir_K}, i.e., $\bK_k$ stays in $\widehat{\cK}$, for all $k$, with high probability. We first show that with a finite number of samples, the estimated NPG could be accurate enough such that $\bK_1$, the iterate after applying one step of \eqref{eqn:npg_free_K}, is close to $\tilde{\bK}_1$, and thus stays in $\widehat{\cK}$, with high probability. The same arguments could be iteratively applied to all future iterations, because starting from any $\bK_k \in \cK$ and choosing an appropriate stepsize, Theorem \ref{theorem:ir_K} guarantees that 
%$\bP_{\tilde{\bK}_{k\hspace{-0.05em}+\hspace{-0.05em}1}, \bL(\tilde{\bK}_{k\hspace{-0.05em}+\hspace{-0.05em}1})} \hspace{-0.1em}\leq \hspace{-0.1em}\bP_{\bK_k, \bL(\bK_k)}$ almost surely. In other words, 
the iterates following the exact NPG direction are monotonically moving toward the interior of $\cK$. Also, there exist parameters of Algorithm \ref{alg:model_free_outer_NPG} such that the NPG estimates could be arbitrarily close to the exact ones. These two properties together imply that we can control, with high probability, the rate under which the iterates following  \eqref{eqn:npg_free_K} is moving ``outward'', i.e. toward $\partial\cK$. Therefore, we manage to demonstrate that even in the worse case, the iterates of the ZO-NPG update will not travel beyond $\partial\widehat{\cK}$ (the blue line), with high probability. Since $\widehat{\cK}$ is compact, we can then safely choose the parameters of Algorithm \ref{alg:model_free_outer_NPG} when analyzing the convergence rate of \eqref{eqn:npg_free_K}. This completes the proof. \hfill$\blacksquare$

Theorem \ref{theorem:free_IR} appears to be the first IR result of PO in robust control in the derivative-free setting, with previous work in the literature \cite{zhang2019policymixed} focusing only on the case with exact PG accesses. Also, \cite{zhang2019policymixed} studied the infinite-horizon LTI setting (mixed $\cH_2/\cH_{\infty}$ design problem), which has a more complicated constraint set (see \cite{zhang2019policymixed}; Lemma 2.7) compared to our $\cK$. Thus, it is still open whether implicit regularization property can be proved for derivative-free methods in this setting. In contrast, our finite-horizon time-varying setting leads to a simpler form of the robust controller set $\cK$. However, we note that a delicate control of the iterates is still needed when proving Theorem \ref{theorem:free_IR}. Specifically, in the  derivative-free setting, the iterates $\bK_k$ need to be \emph{uniformly} separated from the boundary of $\cK$, so that the algorithm parameters can be chosen appropriately, without driving $\bK_k$ out of $\cK$.  To this end, we manage to establish some argument stronger than that in Theorem \ref{theorem:ir_K}, i.e., $\bK_k$ stays in a \emph{strict subset} of $\cK$, denoted by $\widehat{\cK}$, with high probability. The exact-case  implicit regularization in Theorem \ref{theorem:ir_K} is important in this proof, which has to be carefully  adapted to account for the estimation error when sampling  the NPG direction using trajectories. Finally,  with Theorem \ref{theorem:free_IR} in hand, we present the sample complexity of the outer-loop ZO-NPG algorithm \eqref{eqn:npg_free_K}, deferring its proof to \S\ref{proof:free_npg_K}.


\begin{theorem}\label{theorem:free_npg_K}(Outer-Loop Sample Complexity for NPG) For any $\bK_0 \in \cK$, let $\epsilon_2 \leq \phi/2$, $\delta_2, \epsilon_1, \delta_1, M_2, r_2, \alpha$ in Algorithm \ref{alg:model_free_outer_NPG} satisfy the requirements in Theorem \ref{theorem:free_IR}, but with $\varpi$ therein replaced by $\varphi := \min\left\{\varpi, \alpha\phi\epsilon_2/[\sqrt{s}c_0\cB_{\bP}]\right\}$. Then, it holds with probability at least $1-\delta_2$ that the sequence $\{\bK_k\}$, $k \in \{0, \cdots, K\}$, converges with $\cO(1/K)$ rate such that $K^{-1}\sum^{K-1}_{k = 0} \|\bF_{\bK_k, \bL(\bK_k)}\|^2_F \\ \leq \epsilon_2$  with $K = \tr(\bP_{\bK_0, \bL(\bK_0)} - \bP_{\bK^*, \bL(\bK^*)})/[\alpha\phi\epsilon_2]$, which is also towards the unique Nash equilibrium.
 \end{theorem}

 Hence, ZO-NPG converges to the $\epsilon_2$-neighborhood of the Nash equilibrium with probability at least $1-\delta_2$, after using $M_2\cdot K \sim \tilde{\cO}(\epsilon_2^{-5}\cdot\log(\delta_2^{-1}))$ samples. Moreover, the convergent gain matrix $\bK_{K}$ also solves the LEQG and the LQ disturbance attenuation problems (cf. Lemma \ref{lemma:equivalent}).
 
 Compared with the $\tilde{\cO}(\epsilon^{-2})$ rate of PG methods for solving LQR \cite{malik2020derivative} and our inner-loop (cf. Theorem \ref{theorem:free_pg_L}), the $\tilde{\cO}(\epsilon^{-5})$ rate of ZO-NPG for solving our outer-loop is less efficient, due to the much richer landscape presented in Lemma \ref{lemma:landscape_K}. In particular, the objective function of LQR is coercive (leading to the ``compactness” of sub-level sets and the ``smoothness” over the sub-level sets, and enabling the use of “any” descent direction of the objective to ensure feasibility) and PL. In contrast, none of these properties hold true for the objective function of our outer loop, and a descent direction of the objective value may still drive the iterates out of $\cK$, which will lead to unbounded/undefined value.
 
 To guarantee that the ZO-NPG iterates will stay within $\cK$ (which is necessary for the iterates to be well-defined), we need to use large number of samples ($\tilde{\cO}(\epsilon^{-5})$ in $\epsilon$) to obtain a very accurate approximation of the exact NPG update \eqref{eqn:npg_K}, similar to what has been done in \cite{fazel2018global}, to ensure that $\bP_{\bK, \bL(\bK)}$ is monotonically non-increasing in the p.s.d. sense with a high probability along iterations. For LQR, any descent direction of the objective value, which is a scalar, suffices to guarantee that the PG iterates will stay in the feasible set. Therefore, for LQR, the $\tilde{\cO}(\epsilon^{-2})$ rate is expected for the smooth (since the iterates will not leave the feasible set, which is compact) and PL objective functions; while for our robust control setting, due to the more stringent requirements on the estimation accuracy and the non-PL objective function, the $\tilde{\cO}(\epsilon^{-5})$ rate is reasonable. In fact, to our knowledge, there is no sample complexity lower-bound applicable to our outer loop (stochastic nonconvex optimization with no global smoothness nor coercivity nor PL condition, with an inner-loop oracle).
 

==> Mixed Design Arxiv v3/sim.tex <==
In this section, we provide simulation results to complement our theories. In particular, we present convergence (divergence) results in the following four scenarios where we apply PG updates in Algorithms \ref{alg:model_free_inner_PG} and \ref{alg:model_free_outer_NPG} to solve a finite-horizon zero-sum LQ dynamic game with time-invariant system parameters: (i) double-loop update scheme with both the inner- and outer-loop solved exactly; (ii) double-loop scheme with the inner-loop solved in the derivative-free scheme by sampling system trajectories while the outer-loop solved exactly; (iii) double-loop scheme with the inner-loop solved exactly while the outer-loop solved in the derivative-free scheme by sampling system trajectories; (iv) descent-multi-step-ascent/AGDA/$\tau$-GDA with exact gradient accesses diverge. Subsequently, we extend our numerical experiments to a setting with \emph{time-varying} system parameters in \S\ref{sec:time_varying}, and demonstrate the convergence results of double-loop PG updates.

\textbf{Simulation Setup.} All the experiments are executed on a desktop computer equipped with a 3.7 GHz Hexa-Core Intel Core i7-8700K processor with Matlab R2019b. The device also has two 8GB 3000MHz DDR4 memories and a NVIDIA GeForce GTX 1080 8GB GDDR5X graphic card. In all settings except the one used in \S\ref{sec:time_varying}, we set the horizon of the problem to $N=5$ and test a linear time-invariant system with the set of system matrices being $A_t = A$, $B_t=B$, $D_t=D$, $Q_t =Q$, $R^u_t=R^u$, and $R^w_t = R^w$, where $R^w = 5\cdot \bI$ and
\small
\begin{align}\label{parameter}
	A = \begin{bmatrix} 1 & 0 & -5 \\ -1 & 1 & 0 \\ 0 & 0 & 1\end{bmatrix},
	~\ B = \begin{bmatrix} 1 & -10 & 0 \\ 0 & 3 & 1 \\ -1 & 0 & 2\end{bmatrix},
	~\ D = \begin{bmatrix} 0.5 & 0 & 0 \\ 0 & 0.2 & 0 \\ 0 & 0 & 0.2\end{bmatrix},
	~\ Q = \begin{bmatrix} 2 & -1 & 0 \\ -1 & 2 & -1 \\ 0 & -1 & 2\end{bmatrix},
	~\ R^u = \begin{bmatrix} 4 & -1 & 0 \\ -1 & 4 & -2 \\ 0 & -2 & 3\end{bmatrix}.
\end{align}
\normalsize

% \begin{figure}[t]
%\begin{center}
%\includegraphics[width=1\textwidth]{plots/exact_case1.png}
%\caption{Convergence of three sets of the exact double-loop updates starting from $\bK_{0}^1$. \emph{Top:} Convergence of the objective function and $\lambda_{\min}(\bH_{\bK, \bL})$. \emph{Bottom:} Convergence of $\{l^{-1}\sum_{\iota=0}^{l-1}\|\nabla_{\bL}(\bK, \bL_\iota)\|_F\}_{l\geq 1}$; and the convergence of $\{k^{-1}\sum_{\kappa=0}^{k-1}\|\nabla_{\bK}\cG(\bK_\kappa, \overline{\bL}(\bK_\kappa))\|_F\}_{k\geq 1}$, where $\overline{\bL}(\bK)$ is the approximate inner-loop solution with $\epsilon_1 = 0.001$. }
%\label{fig:exact_1}
%\end{center}
%\end{figure}
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=1\textwidth]{plots/exact_case2.png}
%\end{center}
%\caption{Two combinations of the exact double-loop updates following the initialization $\bK_{0}^2$. \emph{Left:} Convergence of the objective function and $\lambda_{\min}(\bH_{\bK, \bL(\bK)})$. \emph{Right:} Convergence of average gradient norms with respect to $\bL$ and $\bK$, respectively. }
%\label{fig:exact_2}
%\end{figure}
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.9\textwidth]{plots/case3.png}
%\end{center}
%\caption{Convergence of the objective function and $\lambda_{\min}(\bH_{\bK, \bL(\bK)})$ following two sets of the update rules and the initial gain matrix $\bK_{0}^3$. \emph{Left:}  The inner loop follows the ZO-PG update \eqref{eqn:pg_free_L} and the outer loop follows the exact NPG update \eqref{eqn:npg_K}. \emph{Right:} The inner loop follows the ZO-NPG update \eqref{eqn:npg_free_L} and the outer loop follows the exact NPG update \eqref{eqn:npg_K}. }
%\label{fig:exact_3}
%\end{figure}
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.9\textwidth]{plots/maincase.png}
%\end{center}
%\caption{Convergence behaviors of the objective function and the minimum eigenvalue of $\bH_{\bK, \bL}$, where the inner loop follows the exact NPG update \eqref{eqn:npg_L} and the outer loop follows the ZO-NPG update \eqref{eqn:npg_free_K}. \emph{Left: } The case where we assume accesses to the exact inner-loop solutions given by \eqref{eqn:l_k}. \emph{Right:} The case where Algorithm \ref{alg:model_free_outer_NPG} computes the approximate inner-loop solution using the exact NPG update \eqref{eqn:npg_L} until achieving the accuracy level of $\epsilon_1 = 10^{-4}$. }
%\label{fig:main_plot}
%\end{figure}
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.8\textwidth]{plots/gda.png}
%\end{center}
%\caption{Diverging patterns of the objective and average gradient norms with respect to $\bK$ and $\bL$. \emph{Top: } ANGDA with stepsizes $\eta = \alpha = 1.7319\times 10^{-11}$. \emph{Middle:} $\tau$-NGDA with stepsizes $\alpha = 1.7319\times 10^{-11}$ and $\eta = 10^3\cdot \alpha$. \emph{Bottom: } Descent-multi-step-ascent with update rules \eqref{eqn:npg_L}-\eqref{eqn:npg_K} and stepsizes $\eta = \alpha = 1.7319\times 10^{-9}$. For each iteration of the outer-loop NPG update \eqref{eqn:npg_K}, we run 10 iterations of the inner-loop NPG update \eqref{eqn:npg_L}.}
%\label{fig:gda}
%\end{figure}
%
%\subsection{Exact Double-Loop Updates}\label{sec:exact1}
%% We test a linear time-invariant system with the set of system matrices being $A_t = A$, $B_t=B$, $D_t=D$, $Q_t =Q$, $R^u_t=R^u$, and $R^w_t = R^w$, where $R^w = 5\cdot \bI$ and
%%\begin{align*}
%%	A = \begin{bmatrix} 1 & 0 & -5 \\ -1 & 1 & 0 \\ 0 & 0 & 1\end{bmatrix},
%%	\quad B = \begin{bmatrix} 1 & -10 & 0 \\ 0 & 3 & 1 \\ -1 & 0 & 2\end{bmatrix},
%%	\quad D = \begin{bmatrix} 0.5 & 0 & 0 \\ 0 & 0.2 & 0 \\ 0 & 0 & 0.2\end{bmatrix},
%%	\quad Q = \begin{bmatrix} 2 & -1 & 0 \\ -1 & 2 & -1 \\ 0 & -1 & 2\end{bmatrix},
%%	\quad R^u = \begin{bmatrix} 4 & -1 & 0 \\ -1 & 4 & -2 \\ 0 & -2 & 3\end{bmatrix}.
%%\end{align*}
%We set $\Sigma_0 = \bI$. Then, we present the convergence result following two different initializations, denoted as $\bK_{0}^1$ and $\bK_{0}^2$, where $\bK_{0}^2$ is closer to the boundary of $\cK$. Specifically, $\bK_{0}^i = \big[ diag((K_{0}^i)^5) ~~~ \bm{0}_{15\times 3}  \big]$, for $i \in \{1, 2\}$, where \small$K_{0}^1 =  \begin{bmatrix} -0.12 & -0.01 & 0.62 \\ -0.21 & 0.14 & 0.15 \\ -0.06 & 0.05 & 0.42\end{bmatrix}$ \normalsize and \small$K_{0}^2 =  \begin{bmatrix} -0.14 & -0.04 & 0.62 \\ -0.21 & 0.14 & 0.15 \\ -0.06 & 0.05 & 0.42\end{bmatrix}$\normalsize. Then, we can verify that $\lambda_{\min}(\bH_{\bK_{0}^1, \bL(\bK_{0}^1)}) = 0.5041$ and $\lambda_{\min}(\bH_{\bK_{0}^2, \bL(\bK_{0}^2)}) = 0.0199$. Moreover, we initialize $\bL = \bm{0}$ in both cases.
%
% \vspace{0.6em}
%\noindent\textbf{Case 1: } We demonstrate in Figure \ref{fig:exact_1} the convergence of three update combinations, namely PG-NPG, NPG-NPG, and GN-GN, for the inner and outer loop, respectively. The stepsizes are chosen to be $(\eta, \alpha) = (1\times 10^{-4}, 3\times 10^{-6})$ for PG-NPG, $(\eta, \alpha) = (0.1, 3\times 10^{-6})$ for NPG-NPG, and $(\eta, \alpha) = (0.5, 5\times 10^{-4})$ for GN-GN. Also, we require the approximate inner-loop solution to have the accuracy of $\epsilon_1 = 0.001$. As shown in the top of Figure \ref{fig:exact_1}, the double-loop algorithm with all three update combinations successfully converges to the unique Nash equilibrium of the game. Also, the sequence $\{\lambda_{\min}(\bH_{\bK_{k}, \bL(\bK_{k})})\}_{k\geq 0}$ is monotonically non-decreasing, which matches the implicit regularization property we introduced in Theorem \ref{theorem:ir_K} for the outer-loop NPG and GN updates. As $\bK_{0}^1 \in \cK$, we can guarantee that all future iterates will stay inside $\cK$. The convergences of the average gradient norms with respect to both $\bL$ and $\bK$ are also presented in the bottom of Figure \ref{fig:exact_1}.
%
% \vspace{0.6em}
% \noindent\textbf{Case 2: }When the initial gain matrix $\bK_{0}^2$ is closer to the boundary of $\cK$, one non-judicious update could easily drive the gain matrix outside of $\cK$. In this case, we present two combinations of updates, namely NPG-NPG and GN-GN, for the inner and outer loop, respectively. We use the stepsizes $(\eta, \alpha) = (0.1, 2.48\times 10^{-7})$ for NPG-NPG and $(\eta, \alpha) = (0.5, 2.5\times 10^{-4})$ for GN-GN. Similarly, we also set $\epsilon_1 = 0.001$. The convergence patterns presented in Figure \ref{fig:exact_2} are similar to those of \textbf{Case 1}.
%
%\subsection{Derivative-Free Inner-Loop Oracles}\label{sec:zo-fo}
%We provide two sets of experiments to validate Theorems \ref{theorem:free_pg_L} and \ref{theorem:free_npg_L}. We consider the same example as the one in \S\ref{sec:exact1}, but using derivative-free updates \eqref{eqn:pg_free_L}-\eqref{eqn:npg_free_L} by sampling system trajectories to approximately solve the inner-loop subproblem, as proposed in \S\ref{sec:max_oracle}. Note that the inner-loop subproblem is essentially an indefinite LQR, as introduced in \S\ref{sec:1st}. The outer-loop problem is solved using the exact NPG update \eqref{eqn:npg_K}. Note that according to Theorem \ref{theorem:free_npg_K}, one can also use the outer-loop ZO-NPG \eqref{eqn:npg_free_K} together with the inner-loop derivative-free updates to achieve the same convergence pattern. However, we use an exact outer-loop update, as it suffices to illustrate our idea here and also has better computational efficiency. In contrast to the example in \S\ref{sec:exact1}, we set $\Sigma_0 = 0.1\cdot\bI$ and initialize $\bK_{0}^3 = \big[ diag((K_{0}^3)^5) ~~~ \bm{0}_{15\times 3}  \big]$ with \small$K_{0}^3 =  \begin{bmatrix} -0.04 & -0.01 & 0.61 \\ -0.21 & 0.15 & 0.15 \\ -0.06 & 0.05 & 0.42\end{bmatrix}$\normalsize, where one can verify that $\lambda_{\min}(\bH_{\bK_{0}^3, \bL(\bK_{0}^3)}) = 1.8673>0$. That is, $\bK_{0}^3 \in \cK$.
% 
% \vspace{0.6em}
% \noindent\textbf{Inner-Loop ZO-PG: }When we use the inner-loop ZO-PG update \eqref{eqn:pg_free_L} in Algorithm \ref{alg:model_free_inner_PG}, we choose $M_1 = 10^6$ and $r_1 = 1$. Moreover, we set the stepsizes of the inner-loop ZO-PG and the outer-loop exact NPG to be $(\eta, \alpha) = (8\times 10^{-3}, 4.5756\times 10^{-4})$, respectively. The desired accuracy level of the double-loop algorithm is picked to be $(\epsilon_1, \epsilon_2) = (0.8, 0.5)$. As shown in the left of Figure \ref{fig:exact_3}, the inner-loop ZO-PG \eqref{eqn:npg_free_L} successfully converges for every fixed outer-loop update, validating our results in Theorem \ref{theorem:free_pg_L}. Also, the double-loop algorithm converges to the unique Nash equilibrium of the game. 
%  
%  \vspace{0.6em}
% \noindent\textbf{Inner-Loop ZO-NPG: }When the inner-loop subproblem is solved via the ZO-NPG update \eqref{eqn:npg_free_L}, we choose the same $M_1, r_1, \alpha, \epsilon_1, \epsilon_2$ as the ones used in the inner-loop ZO-PG update but in contrast we set $\eta = 5 \times 10^{-2}$. Similar convergence patterns can be observed in the right of Figure \ref{fig:exact_3}.
%
%\subsection{Derivative-Free Outer-Loop NPG}
%%We test a linear time-invariant system with the set of parameters being $A_t = A$, $B_t=B$, $D_t=D$, $Q_t =Q$, $R^u_t=R^u$, and $R^w_t = R^w$ for all $t$, where $R^w = 5\cdot \bI$ and
%%\begin{align*}
%%	A = \begin{bmatrix} 1 & 0 & -5 \\ -1 & 1 & 0 \\ 0 & 0 & 1\end{bmatrix},
%%	\quad B = \begin{bmatrix} 1 & -10 & 0 \\ 0 & 3 & 1 \\ -1 & 0 & 2\end{bmatrix},
%%	\quad D = \begin{bmatrix} 0.5 & 0 & 0 \\ 0 & 0.2 & 0 \\ 0 & 0 & 0.2\end{bmatrix},
%%	\quad Q = \begin{bmatrix} 2 & -1 & 0 \\ -1 & 2 & -1 \\ 0 & -1 & 2\end{bmatrix},
%%	\quad R^u = \begin{bmatrix} 4 & -1 & 0 \\ -1 & 4 & -2 \\ 0 & -2 & 3\end{bmatrix}.
%%\end{align*}
%We set $\Sigma_0 = 0.05\cdot\bI$. We present convergence results following the initial gain matrix $\bK_{0} = \big[ diag(K^5) ~~~ \bm{0}_{15\times 3} \big]$, where \small$K =  \begin{bmatrix}
%	-0.08 & 0.35 & 0.62 \\ -0.21 & 0.19 & 0.32 \\ -0.06 & 0.10 & 0.41\end{bmatrix}$ \normalsize and \small$\lambda_{\min}(\bH_{\bK_0, \bL(\bK_0)}) = 3.2325$\normalsize. The convergence of Algorithm \ref{alg:model_free_outer_NPG} is implemented for two cases, with the inner-loop oracle being implemented using (i) the exact solution as computed by \eqref{eqn:l_k}; and (ii) the approximate inner-loop solution following the exact NPG update \eqref{eqn:npg_L}. As proved by Theorems \ref{theorem:free_pg_L} and \ref{theorem:free_npg_L}, the inner loop can also be solved approximately using either ZO-PG or ZO-NPG updates, which has been verified via the simulation results presented in \S\ref{sec:zo-fo}. The parameters of Algorithm \ref{alg:model_free_outer_NPG} in both cases are set to $M_2 = 5\times 10^5$, ~ $r_2 = 0.08$, ~$(\eta, \alpha) = (0.1, 4.67\times 10^{-5})$, and $ (\epsilon_1, \epsilon_2) = (10^{-4}, 0.8)$. Figure \ref{fig:main_plot} illustrates the behaviors of the objective function and the smallest eigenvalue of $\bH_{\bK, \bL}$ following the double-loop update scheme. It is shown that iterates of the outer-loop gain matrix $\{\bK_k\}_{k\geq 0}$ stay within the feasible set $\cK$ along with the double-loop update, which preserves a certain disturbance attenuation level in the view of Remark \ref{remark:ir}.  Moreover, in both cases, we have Algorithm \ref{alg:model_free_outer_NPG} converging sublinearly to the unique Nash equilibrium. 
%
%
%
%\subsection{Divergent Cases}\label{sec:alternate}
%As noted in Remark \ref{remark:double}, it is unclear yet if descent-multi-step-ascent, AGDA, or $\tau$-GDA, where $\tau = \eta/\alpha$, can converge globally to the Nash equilibrium in our setting.  In this section, we present some scenarios where descent-multi-step-ascent, AGDA, and $\tau$-GDA diverges even with infinitesimal stepsizes. We use the same example as \S\ref{sec:exact1} and initialize $\bK_{0}^4, \bL_{0}^4$ to be time-invariant such that \small$K^4_{0, t} = K_{0}^4 = \begin{bmatrix} -0.1362 &   0.0934 &   0.6458 \\ -0.2717 &  -0.1134 &  -0.4534 \\ -0.6961 &  -0.9279 &  -0.6620 \end{bmatrix}$ \normalsize and \small$L_{0, t}^4 = L_{0}^4 = \begin{bmatrix}0.2887  & -0.2286 &   0.4588 \\ -0.7849 &  -0.1089 &  -0.3755 \\   -0.2935 &   0.9541 &   0.7895\end{bmatrix}$ \normalsize for all $t$. Note that in descent-multi-step-ascent/AGDA/$\tau$-GDA, the maximizing problem with respect to $\bL$ for a fixed $\bK$ is no longer solved to a high accuracy for each iteration of the updates on $\bK$. Thus, we can relax the constraint $\bK \in \cK$ since the maximizing player will not drive the cost to $\infty$ in such iterates under descent-multi-step-ascent/AGDA/$\tau$-GDA. Figure \ref{fig:gda} illustrates the behaviors of the objective and the gradient norms with respect to $\bK$ and $\bL$ when applying alternating natural GDA (ANGDA), $\tau$-natural GDA ($\tau$-NGDA), and descent-multi-step-ascent with updates \eqref{eqn:npg_L}-\eqref{eqn:npg_K} to our problem. The stepsizes for the ANGDA are chosen to be infinitesimal such that $\eta = \alpha = 1.7319\times 10^{-11}$. However, we can still observe the diverging patterns from the top row of Figure \ref{fig:gda}, even with such tiny stepsizes. Further, we test the same example with the same initialization but use $\tau$-NGDA with $\tau = 10^3$. That is, $\eta = 10^3\cdot\alpha$. In such case, it is shown in the middle row of Figure \ref{fig:gda} that diverging behaviors still appear. Whether there exists a finite timescale separation $\tau^*$, similar to the one proved in \cite{fiez2020gradient}, such that $\tau$-GDA type algorithms with $\tau \in (\tau^*, \infty)$ provably converge to the unique Nash equilibrium in our setting requires further investigation, and is left as our future work. Lastly, we present a case where descent-multi-step-ascent with updates following \eqref{eqn:npg_L}-\eqref{eqn:npg_K} diverges. The stepsizes are chosen to be $\eta = \alpha = 1.7319\times 10^{-9}$ and we run 10 iterations of \eqref{eqn:npg_L} for each iteration of \eqref{eqn:npg_K}. The bottom row of Figure \ref{fig:gda} demonstrates the diverging behaviors of this update scheme.
\subsection{Exact Double-Loop Updates}\label{sec:exact1}
% We test a linear time-invariant system with the set of system matrices being $A_t = A$, $B_t=B$, $D_t=D$, $Q_t =Q$, $R^u_t=R^u$, and $R^w_t = R^w$, where $R^w = 5\cdot \bI$ and
%\begin{align*}
%	A = \begin{bmatrix} 1 & 0 & -5 \\ -1 & 1 & 0 \\ 0 & 0 & 1\end{bmatrix},
%	\quad B = \begin{bmatrix} 1 & -10 & 0 \\ 0 & 3 & 1 \\ -1 & 0 & 2\end{bmatrix},
%	\quad D = \begin{bmatrix} 0.5 & 0 & 0 \\ 0 & 0.2 & 0 \\ 0 & 0 & 0.2\end{bmatrix},
%	\quad Q = \begin{bmatrix} 2 & -1 & 0 \\ -1 & 2 & -1 \\ 0 & -1 & 2\end{bmatrix},
%	\quad R^u = \begin{bmatrix} 4 & -1 & 0 \\ -1 & 4 & -2 \\ 0 & -2 & 3\end{bmatrix}.
%\end{align*}
We set $\Sigma_0 = \bI$. Then, we present the convergence result following two different initializations, denoted as $\bK_{0}^1$ and $\bK_{0}^2$, where $\bK_{0}^2$ is closer to the boundary of $\cK$. Specifically, $\bK_{0}^i = \big[ diag((K_{0}^i)^5) ~~~ \bm{0}_{15\times 3}  \big]$, for $i \in \{1, 2\}$, where \small$K_{0}^1 =  \begin{bmatrix} -0.12 & -0.01 & 0.62 \\ -0.21 & 0.14 & 0.15 \\ -0.06 & 0.05 & 0.42\end{bmatrix}$ \normalsize and \small$K_{0}^2 =  \begin{bmatrix} -0.14 & -0.04 & 0.62 \\ -0.21 & 0.14 & 0.15 \\ -0.06 & 0.05 & 0.42\end{bmatrix}$\normalsize. Then, we can verify that $\lambda_{\min}(\bH_{\bK_{0}^1, \bL(\bK_{0}^1)}) = 0.5041$ and $\lambda_{\min}(\bH_{\bK_{0}^2, \bL(\bK_{0}^2)}) = 0.0199$. Moreover, we initialize $\bL = \bm{0}$ in both cases.

 \begin{figure}[t]
 \vspace{2em}
\begin{center}
\includegraphics[width=0.95\textwidth]{plots/exact_case1.png}
\caption{Three exact double-loop PG updates with initial gain matrix being $\bK_{0}^1$. \emph{Top:} Convergence of $\cG(\bK, \bL)$ and $\lambda_{\min}(\bH_{\bK, \bL})$. \emph{Bottom:} Convergence of \small$\{l^{-1}\sum_{\iota=0}^{l-1}\|\nabla_{\bL}(\bK, \bL_\iota)\|_F\}_{l\geq 1}$\normalsize and \small$\{k^{-1}\sum_{\kappa=0}^{k-1}\|\nabla_{\bK}\cG(\bK_\kappa, \overline{\bL}(\bK_\kappa))\|_F\}_{k\geq 1}$\normalsize. $\overline{\bL}(\bK)$ is the approximate inner-loop solution with $\epsilon_1 = 10^{-3}$. }
\label{fig:exact_1}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=1\textwidth]{plots/exact_case2.png}
\end{center}
\caption{Two exact double-loop PG updates with initial gain matrix being $\bK_{0}^2$. \emph{Left:} Convergence of of $\cG(\bK, \bL)$ and $\lambda_{\min}(\bH_{\bK, \bL(\bK)})$. \emph{Right:} Convergence of \small$\{l^{-1}\sum_{\iota=0}^{l-1}\|\nabla_{\bL}(\bK, \bL_\iota)\|_F\}_{l\geq 1}$\normalsize and \small$\{k^{-1}\sum_{\kappa=0}^{k-1}\|\nabla_{\bK}\cG(\bK_\kappa, \overline{\bL}(\bK_\kappa))\|_F\}_{k\geq 1}$\normalsize. $\overline{\bL}(\bK)$ is the approximate inner-loop solution with $\epsilon_1 = 10^{-3}$. }
\label{fig:exact_2}
\end{figure}

 \vspace{0.6em}
\noindent\textbf{Case 1: } We demonstrate in Figure \ref{fig:exact_1} the convergence of three update combinations, namely PG-NPG, NPG-NPG, and GN-GN, for the inner and outer loop, respectively. The stepsizes are chosen to be $(\eta, \alpha) = (1\times 10^{-4}, 3\times 10^{-6})$ for PG-NPG, $(\eta, \alpha) = (0.0635, 3\times 10^{-6})$ for NPG-NPG, and $(\eta, \alpha) = (0.5, 5\times 10^{-4})$ for GN-GN. Also, we require the approximate inner-loop solution to have the accuracy of $\epsilon_1 = 0.001$. As shown in the top of Figure \ref{fig:exact_1}, the double-loop algorithm with all three update combinations successfully converges to the unique Nash equilibrium of the game. Also, the sequence $\{\lambda_{\min}(\bH_{\bK_{k}, \bL(\bK_{k})})\}_{k\geq 0}$ is monotonically non-decreasing, which matches the implicit regularization property we introduced in Theorem \ref{theorem:ir_K} for the outer-loop NPG and GN updates. As $\bK_{0}^1 \in \cK$, we can guarantee that all future iterates will stay inside $\cK$. The convergences of the average gradient norms with respect to both $\bL$ and $\bK$ are also presented in the bottom of Figure \ref{fig:exact_1}.

 \vspace{0.6em}
 \noindent\textbf{Case 2: }When the initial gain matrix $\bK_{0}^2$ is closer to the boundary of $\cK$, one non-judicious update could easily drive the gain matrix outside of $\cK$. In this case, we present two combinations of updates, namely NPG-NPG and GN-GN, for the inner and outer loop, respectively. We use the stepsizes $(\eta, \alpha) = (0.0635, 2.48\times 10^{-7})$ for NPG-NPG and $(\eta, \alpha) = (0.5, 2.5\times 10^{-4})$ for GN-GN. Similarly, we set $\epsilon_1 = 0.001$. The convergence patterns presented in Figure \ref{fig:exact_2} are similar to those of \textbf{Case 1}.

\subsection{Derivative-Free Inner-Loop Oracles}\label{sec:zo-fo}
We provide two sets of experiments to validate Theorems \ref{theorem:free_pg_L} and \ref{theorem:free_npg_L}. We consider the same example as the one in \S\ref{sec:exact1}, but using derivative-free updates \eqref{eqn:pg_free_L}-\eqref{eqn:npg_free_L} by sampling system trajectories to approximately solve the inner-loop subproblem, as proposed in \S\ref{sec:max_oracle}. Note that the inner-loop subproblem is essentially an indefinite LQR, as introduced in \S\ref{sec:1st}. The outer-loop problem is solved using the exact NPG update \eqref{eqn:npg_K}. Note that according to Theorem \ref{theorem:free_npg_K}, one can also use the outer-loop ZO-NPG \eqref{eqn:npg_free_K} together with the inner-loop derivative-free updates to achieve the same convergence pattern. However, we use an exact outer-loop update, as it suffices to illustrate our idea here and also has better computational efficiency. In contrast to the example in \S\ref{sec:exact1}, we set $\Sigma_0 = 0.1\cdot\bI$ and initialize $\bK_{0}^3 = \big[ diag((K_{0}^3)^5) ~~~ \bm{0}_{15\times 3}  \big]$ with \small$K_{0}^3 =  \begin{bmatrix} -0.04 & -0.01 & 0.61 \\ -0.21 & 0.15 & 0.15 \\ -0.06 & 0.05 & 0.42\end{bmatrix}$\normalsize, where one can verify that $\lambda_{\min}(\bH_{\bK_{0}^3, \bL(\bK_{0}^3)}) = 1.8673>0$. That is, $\bK_{0}^3 \in \cK$.
 
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\textwidth]{plots/case3.png}
\end{center}
\caption{Convergence of $\cG(\bK, \bL)$ and $\lambda_{\min}(\bH_{\bK, \bL(\bK)})$ with the initial gain matrix being $\bK_{0}^3$. \emph{Left:}  The inner loop follows the ZO-PG update \eqref{eqn:pg_free_L} and the outer loop follows the exact NPG update \eqref{eqn:npg_K}. \emph{Right:} The inner loop follows the ZO-NPG update \eqref{eqn:npg_free_L} and the outer loop follows the exact NPG update \eqref{eqn:npg_K}. }
\label{fig:exact_3}
\end{figure}

 \vspace{0.6em}
 \noindent\textbf{Inner-Loop ZO-PG: }When we use the inner-loop ZO-PG update \eqref{eqn:pg_free_L} in Algorithm \ref{alg:model_free_inner_PG}, we choose $M_1 = 10^6$ and $r_1 = 1$. Moreover, we set the stepsizes of the inner-loop ZO-PG and the outer-loop exact NPG to be $(\eta, \alpha) = (8\times 10^{-3}, 4.5756\times 10^{-4})$, respectively. The desired accuracy level of the double-loop algorithm is picked to be $(\epsilon_1, \epsilon_2) = (0.8, 0.5)$. As shown in the left of Figure \ref{fig:exact_3}, the inner-loop ZO-PG \eqref{eqn:npg_free_L} successfully converges for every fixed outer-loop update, validating our results in Theorem \ref{theorem:free_pg_L}. Also, the double-loop algorithm converges to the unique Nash equilibrium of the game. 
  
  \vspace{0.6em}
 \noindent\textbf{Inner-Loop ZO-NPG: }When the inner-loop subproblem is solved via the ZO-NPG update \eqref{eqn:npg_free_L}, we choose the same $M_1, r_1, \alpha, \epsilon_1, \epsilon_2$ as the ones used in the inner-loop ZO-PG update but in contrast we set $\eta = 5 \times 10^{-2}$. Similar convergence patterns can be observed in the right of Figure \ref{fig:exact_3}.

\subsection{Derivative-Free Outer-Loop NPG}
%We test a linear time-invariant system with the set of parameters being $A_t = A$, $B_t=B$, $D_t=D$, $Q_t =Q$, $R^u_t=R^u$, and $R^w_t = R^w$ for all $t$, where $R^w = 5\cdot \bI$ and
%\begin{align*}
%	A = \begin{bmatrix} 1 & 0 & -5 \\ -1 & 1 & 0 \\ 0 & 0 & 1\end{bmatrix},
%	\quad B = \begin{bmatrix} 1 & -10 & 0 \\ 0 & 3 & 1 \\ -1 & 0 & 2\end{bmatrix},
%	\quad D = \begin{bmatrix} 0.5 & 0 & 0 \\ 0 & 0.2 & 0 \\ 0 & 0 & 0.2\end{bmatrix},
%	\quad Q = \begin{bmatrix} 2 & -1 & 0 \\ -1 & 2 & -1 \\ 0 & -1 & 2\end{bmatrix},
%	\quad R^u = \begin{bmatrix} 4 & -1 & 0 \\ -1 & 4 & -2 \\ 0 & -2 & 3\end{bmatrix}.
%\end{align*}
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\textwidth]{plots/maincase.png}
\end{center}
\caption{Convergence of $\cG(\bK, \bL)$ and $\lambda_{\min}(\bH_{\bK, \bL})$ when the outer loop follows the ZO-NPG update \eqref{eqn:npg_free_K}. \emph{Left: } The inner-loop solutions are computed by \eqref{eqn:l_k}. \emph{Right:} The inner-loop solutions are approximated by the exact NPG update \eqref{eqn:npg_L} with an accuracy level of $\epsilon_1 = 10^{-4}$. }
\label{fig:main_plot}
\end{figure}

We set $\Sigma_0 = 0.05\cdot\bI$. We present convergence results following the initial gain matrix $\bK_{0} = \big[ diag(K^5) ~~~ \bm{0}_{15\times 3} \big]$, where \small$K =  \begin{bmatrix}
	-0.08 & 0.35 & 0.62 \\ -0.21 & 0.19 & 0.32 \\ -0.06 & 0.10 & 0.41\end{bmatrix}$ \normalsize and \small$\lambda_{\min}(\bH_{\bK_0, \bL(\bK_0)}) = 3.2325$\normalsize. The convergence of Algorithm \ref{alg:model_free_outer_NPG} is implemented for two cases, with the inner-loop oracle being implemented using (i) the exact solution as computed by \eqref{eqn:l_k}; and (ii) the approximate inner-loop solution following the exact NPG update \eqref{eqn:npg_L}. As proved by Theorems \ref{theorem:free_pg_L} and \ref{theorem:free_npg_L}, the inner loop can also be solved approximately using either ZO-PG or ZO-NPG updates, which has been verified via the simulation results presented in \S\ref{sec:zo-fo}. The parameters of Algorithm \ref{alg:model_free_outer_NPG} in both cases are set to $M_2 = 5\times 10^5$, ~ $r_2 = 0.08$, ~$(\eta, \alpha) = (0.1, 4.67\times 10^{-5})$, and $ (\epsilon_1, \epsilon_2) = (10^{-4}, 0.8)$. Figure \ref{fig:main_plot} illustrates the behaviors of the objective function and the smallest eigenvalue of $\bH_{\bK, \bL}$ following the double-loop update scheme. It is shown that iterates of the outer-loop gain matrix $\{\bK_k\}_{k\geq 0}$ stay within the feasible set $\cK$ along with the double-loop update, which preserves a certain disturbance attenuation level in the view of Remark \ref{remark:ir}.  Moreover, in both cases, we have Algorithm \ref{alg:model_free_outer_NPG} converging sublinearly to the unique Nash equilibrium. 



\subsection{Divergent Cases}\label{sec:alternate}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\textwidth]{plots/gda.png}
\end{center}
\caption{Divergence of $\cG(\bK, \bL)$, \small$\{l^{-1}\sum_{\iota=0}^{l-1}\|\nabla_{\bL}(\bK, \bL_\iota)\|_F\}_{l\geq 1}$\normalsize, and \small$\{k^{-1}\sum_{\kappa=0}^{k-1}\|\nabla_{\bK}\cG(\bK_\kappa, \overline{\bL}(\bK_\kappa))\|_F\}_{k\geq 1}$\normalsize. \emph{Top: } ANGDA with stepsizes $\eta = \alpha = 1.7319\times 10^{-11}$. \emph{Middle:} $\tau$-NGDA with stepsizes $\alpha = 1.7319\times 10^{-11}$ and $\eta = 10^3\cdot \alpha$. \emph{Bottom: } Descent-multi-step-ascent with update rules \eqref{eqn:npg_L} and \eqref{eqn:npg_K} and stepsizes $\eta = \alpha = 1.7319\times 10^{-9}$. For each iteration of the outer-loop update \eqref{eqn:npg_K}, we run 10 iterations of the inner-loop update \eqref{eqn:npg_L}.}
\label{fig:gda}
\end{figure}

As noted in Remark \ref{remark:double}, it is unclear yet if descent-multi-step-ascent, AGDA, or $\tau$-GDA, where $\tau = \eta/\alpha$, can converge globally to the Nash equilibrium in our setting.  In this section, we present some scenarios where descent-multi-step-ascent, AGDA, and $\tau$-GDA diverges even with infinitesimal stepsizes. We use the same example as \S\ref{sec:exact1} and initialize $\bK_{0}^4, \bL_{0}^4$ to be time-invariant such that \small$K^4_{0, t} = K_{0}^4 = \begin{bmatrix} -0.1362 &   0.0934 &   0.6458 \\ -0.2717 &  -0.1134 &  -0.4534 \\ -0.6961 &  -0.9279 &  -0.6620 \end{bmatrix}$ \normalsize and \small$L_{0, t}^4 = L_{0}^4 = \begin{bmatrix}0.2887  & -0.2286 &   0.4588 \\ -0.7849 &  -0.1089 &  -0.3755 \\   -0.2935 &   0.9541 &   0.7895\end{bmatrix}$ \normalsize for all $t$. Note that in descent-multi-step-ascent/AGDA/$\tau$-GDA, the maximizing problem with respect to $\bL$ for a fixed $\bK$ is no longer solved to a high accuracy for each iteration of the updates on $\bK$. Thus, we can relax the constraint $\bK \in \cK$ since the maximizing player will not drive the cost to $\infty$ in such iterates under descent-multi-step-ascent/AGDA/$\tau$-GDA. Figure \ref{fig:gda} illustrates the behaviors of the objective and the gradient norms with respect to $\bK$ and $\bL$ when applying alternating natural GDA (ANGDA), $\tau$-natural GDA ($\tau$-NGDA), and descent-multi-step-ascent with updates \eqref{eqn:npg_L} and \eqref{eqn:npg_K} to our problem. The stepsizes for the ANGDA are chosen to be infinitesimal such that $\eta = \alpha = 1.7319\times 10^{-11}$. However, we can still observe the diverging patterns from the top row of Figure \ref{fig:gda}, even with such tiny stepsizes. Further, we test the same example with the same initialization but use $\tau$-NGDA with $\tau = 10^3$. That is, $\eta = 10^3\cdot\alpha$. In such case, it is shown in the middle row of Figure \ref{fig:gda} that diverging behaviors still appear. Whether there exists a finite timescale separation $\tau^*$, similar to the one proved in \cite{fiez2020gradient}, such that $\tau$-GDA type algorithms with $\tau \in (\tau^*, \infty)$ provably converge to the unique Nash equilibrium in our setting requires further investigation, and is left as our future work. Lastly, we present a case where descent-multi-step-ascent with updates following \eqref{eqn:npg_L} and \eqref{eqn:npg_K} diverges. The stepsizes of the inner-loop and the outer-loop updates are chosen to be $\eta = \alpha = 1.7319\times 10^{-9}$ and we run 10 iterations of \eqref{eqn:npg_L} for each iteration of \eqref{eqn:npg_K}. The bottom row of Figure \ref{fig:gda} demonstrates the diverging behaviors of this update scheme.

\subsection{Time-Varying Systems}\label{sec:time_varying}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.62\textwidth]{plots/time_vary}
	\caption{Convergence of the exact double-loop NPG updates with initial gain matrix being $\bK_{0}^5$. \emph{Top:} Convergence of $\cG(\bK, \bL)$ and $\lambda_{\min}(\bH_{\bK, \bL})$. \emph{Bottom:} Convergence of $\{k^{-1}\sum_{\kappa=0}^{k-1}\|\nabla_{\bK}\cG(\bK_\kappa, \overline{\bL}(\bK_\kappa))\|_F\}_{k\geq 1}$ and $\{l^{-1}\sum_{\iota=0}^{l-1}\|\nabla_{\bL}(\bK, \bL_\iota)\|_F\}_{l\geq 1}$. The stepsizes of the inner-loop and the outer-loop NPG updates are chosen to be 0.0097 and  $3.0372\times 10^{-5}$, respectively. For each iteration of the outer-loop NPG update, we solve the inner-loop subproblem to the accuracy of $\epsilon_1 = 0.001$.}
	\label{fig:time_vary}
\end{figure}

Instead of setting $A_t = A$, $B_t = B$, and $D_t = D$ for all $t$, we now choose
\begin{align*}
	A_t = A + \frac{(-1)^t tA}{10}, \quad  B_t = B + \frac{(-1)^t tB}{10}, \quad D_t = D + \frac{(-1)^t tD}{10},
\end{align*} 
and set $R^w = 10\cdot\bI$. Rest of the parameters are set to the same as in \eqref{parameter}. The horizon of the problem is again set to $N=5$ and we initialize our algorithm using \small$K_{0, t}^5 = K_{0}^5 = \begin{bmatrix} -0.0984 & -0.7158 & -0.1460\\ -0.1405 & 0.0039 & 0.4544 \\ -0.1559 & -0.7595 & 0.7403\end{bmatrix}$. \normalsize

We demonstrate in Figure \ref{fig:time_vary} the convergence of exact double-loop NPG updates. The stepsizes of the inner-loop and the outer-loop updates are chosen to be $(\eta, \alpha) = (0.0097, 3.0372\times 10^{-5})$. Also, we require the approximate inner-loop solution to have the accuracy of $\epsilon_1 = 0.001$. As shown at the top of Figure \ref{fig:time_vary}, the double-loop NPG updates successfully converge to the unique Nash equilibrium of the game. Also, the minimum eigenvalue of $\bR^w - \bD^{\top}\bP_{\bK, \bL}\bD$ is monotonically non-decreasing along the iterations of the outer-loop NPG update, which matches the implicit regularization property we introduced in Theorem \ref{theorem:ir_K}. This guarantees that all future iterates of $\bK$ will stay in the interior of $\cK$ given that the initial $\bK$ does. The convergences of the average gradient norms with respect to both $\bL$ and $\bK$ are presented at the bottom of Figure \ref{fig:time_vary}.


==> auxiliary.tex <==
\subsection{Hessians} \label{sec:Hessian}
\xznote{consider not using this... looks stupid, see how Zhengyang proves smoothness}
\begin{lemma}(Hessian of The Inner Loop Problem)
For $X \in \RR^{mN\times n(N+1)}$, and with $(\bP'_{\bL})[X]$ representing the action of differential of the mapping 
$\bL \rightarrow \bP_{\bL}$, the Hessian of the inner loop problem is expressed as
\begin{align}\label{eqn:exact_hessian_L}
	\nabla^2 \cG(\bL)[X, X] = 2\big\langle \bF_{\bL}X\Sigma_{\bL} , X\big\rangle - 4 \big\langle (\bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL})\Sigma_{\bL}, X\big\rangle
\end{align}	
\begin{proof}
	Let $\bE_{\bL}'$ and $\Sigma_{\bL}'$ denote the derivatives with respect to $\bL$ of, respectively, $\bE_{\bL}$ and $\Sigma_{\bL}$. Then, the Hessian of the inner loop problem can be characterized as $\nabla^2\cG(\bL) = 2\bE_{\bL}'\Sigma_{\bL} + 2\bE_{\bL}\Sigma_{\bL}'$, and for $X \in \RR^{mN\times n(N+1)}$, the action of $\nabla^2\cG(\bL)[X, X]$ is given by 
	\begin{align*}
	\nabla^2\cG(\bL)[X, X] &= 2\Big\langle \big((\bR^w + \bD^T\bP_{\bL}\bD)X - \bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL}\big)\Sigma_{\bL}, X\Big\rangle + 2 \Big\langle \bE_{\bL}\big(\Sigma_{\bL}'[X]\big), X\Big\rangle,
%		\frac{d(P_t)}{d(K_t)} = 2(RK_t-B^TP_{t+1}(A-BK_t))
	\end{align*}
 where
	\begin{align*}
		\bP_{\bL}'[X] &= \tilde{\bA}^T_{\bL}(\bP_{\bL}'[X])\tilde{\bA}_{\bL} + 2X^T\bE_{\bL} \\
		\Sigma_{\bL}'[X] &= \tilde{\bA}_{\bL}(\Sigma_{\bL}'[X])\tilde{\bA}^T_{\bL} - \bD X\Sigma_{\bL}\tilde{\bA}^T_{\bL} - \tilde{\bA}_{\bL}\Sigma_{\bL} X^T\bD.
	\end{align*}
	Note that $\bP_{\bL}'[X]$ and $\Sigma_{\bL}'[X]$ can be solved by
	\begin{align}\label{eqn:pk_gradient}
		\bP_{\bL}'[X] &= \sum^N_{i = 0} \big(\tilde{\bA}^T_{\bL}\big)^i\big(2X^T\bE_{\bL}\big)\big(\tilde{\bA}_{\bL}\big)^i \\
		\Sigma_{\bL}'[X] &= \sum^N_{i = 0} \big(\tilde{\bA}_{\bL}\big)^i\big(- \bD X\Sigma_{\bL}\tilde{\bA}^T_{\bL} - \tilde{\bA}_{\bL}\Sigma_{\bL} X^T\bD\big)\big(\tilde{\bA}^T_{\bL}\big)^i.
	\end{align}
	Therefore, the action of the Hessian of the inner loop problem can be represented as
	\begin{align*}
		\nabla^2\cG(\bL)[X, X] &= 2\big\langle (\bR^w + \bD^T\bP_{\bL}\bD)X\Sigma_{\bL} , X\big\rangle - 4 \big\langle (\bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL})\Sigma_{\bL}, X\big\rangle \\
		&= 2\big\langle \bF_{\bL}X\Sigma_{\bL} , X\big\rangle - 4 \big\langle (\bD^T(\bP_{\bL}'[X])\tilde{\bA}_{\bL})\Sigma_{\bL}, X\big\rangle.
	\end{align*}
	This completes the proof of \eqref{eqn:exact_hessian_L}.
\end{proof}
	
\end{lemma}
\begin{lemma}(Hessian of The Outer Loop Problem)
For $X \in \RR^{mN\times d(N+1)}$, and with $(\bE'_{\bK, \bL(\bK)})[X]$ representing the action of differential of the mapping $\bK \rightarrow \bE_{\bK}$, the Hessian of the outer loop problem is expressed as
	\begin{align}\label{eqn:exact_hessian_K}
		\nabla^2\cG(\bK)[X, X] &= 2\big\langle \bE_{\bK}'[X]\Sigma_{\bK} , X\big\rangle + 2 \big\langle \bE_{\bK}\Sigma_{\bK}'[X], X\big\rangle.
	\end{align}
For ease of expositions, we further define : $\Sigma := \Sigma_{\bK}$, $\bP:=\bP_{\bK}$, $\Lambda := \bR^w - \bD^T\bP_{\bK}\bD$, and $\tilde{\bP} := \tilde{\bP}_{\bK}$. Then, $\bE'[X]$ is defined as follows
 \small
 \begin{align}
 	\hspace{-1em}\bE_{\bK}'[X] &= \bF_{\bK} X  - \bB^T\bP'[X]\bA_{\bK} \nonumber\\
 	&\hspace{1em} + \bK\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB + \bK\bD^T\bP\bB\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} + \bK\bD^T\bP\bB\Lambda^{-1}\bB^T\bP'[X]\bD \nonumber\\
 	&\hspace{1em} -\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB\bA - \bD^T\bP\bB\bA\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} - \bD^T\bP\bB\bA\Lambda^{-1}\bB^T\bP'[X]\bD,\label{eqn:E'}
 \end{align}
 \normalsize
 where the definitions of $\bP'[X]$ and $\Sigma'[X]$ are represented, respectively, as
 \begin{align}
		\bP'[X] &= \bA_{\bK}^T(\bP'[X])\bA_{\bK} + 2X^T\bE_{\bK} \label{eqn:pk'}\\
		\Sigma'[X] &= \bA_{\bK}(\Sigma'[X])\bA_{\bK}^T - \bB X\Sigma\bA_{\bK}^T - \bA_{\bK}\Sigma X^T\bB. \label{eqn:sigmak'}
\end{align}
\end{lemma}

\begin{proof}
Let $\bE_{\bK}'$ and $\Sigma_{\bK}'$ denote the derivatives with respect to $\bK$ of, respectively, $\bE_{\bK}$ and $\Sigma_{\bK}$. Then, by the gradient form reported in Lemma \ref{lemma:exact_PG_K}, the Hessian can be characterized as $\nabla^2\cG(\bK) = 2\bE_{\bK}'\Sigma_{\bK} + 2\bE_{\bK}\Sigma_{\bK}'$, and for $X \in \RR^{mN\times d(N+1)}$, the action of $\nabla^2\cG(\bK)[X, X]$ is given by 
	\begin{align*}
	\nabla^2\cG(\bK)[X, X] &= 2\big\langle \bE_{\bK}'[X]\Sigma_{\bK} , X\big\rangle + 2 \big\langle \bE_{\bK}\Sigma_{\bK}'[X], X\big\rangle.
%	&= 2\Big\langle \big((\bR^u+ \bB^T\tilde{\bP}_{\bK, \bL(\bK)}\bB)X - \bB^T(\tilde{\bP}_{\bK, \bL(\bK)}'[X])(\bA-\bB\bK)\big)\Sigma_{\bK, \bL(\bK)} , X\Big\rangle + 2 \Big\langle \bE_{\bK, \bL(\bK)}\big(\Sigma_{\bK, \bL(\bK)}'[X]\big), X\Big\rangle,
%		\frac{d(P_t)}{d(K_t)} = 2(RK_t-B^TP_{t+1}(A-BK_t))
	\end{align*}
 To further simplify the notations, we let $\bP:=\bP_{\bK}$, $\Lambda := \bR^w - \bD^T\bP_{\bK}\bD$, and $\tilde{\bP} := \tilde{\bP}_{\bK}$. Then, 
 \small
 \begin{align*}
 	\bE_{\bK}'[X] &= \bF_{\bK} X  - \bB^T\bP'[X]\bA_{\bK} \nonumber\\
 	&\hspace{1em} + \bK\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB + \bK\bD^T\bP\bB\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} + \bK\bD^T\bP\bB\Lambda^{-1}\bB^T\bP'[X]\bD \nonumber\\
 	&\hspace{1em} -\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bB\bA - \bD^T\bP\bB\bA\bB^T\bP\bD\Lambda^{-1}\bD^T\bP'[X]\bD\Lambda^{-1} - \bD^T\bP\bB\bA\Lambda^{-1}\bB^T\bP'[X]\bD,
 \end{align*}
 \normalsize
 where
 \begin{align*}
		\bP'[X] &= \bA_{\bK}^T(\bP'[X])\bA_{\bK} + 2X^T\bE_{\bK} \\
		\Sigma'[X] &= \bA_{\bK}(\Sigma'[X])\bA_{\bK}^T - \bB X\Sigma\bA_{\bK}^T - \bA_{\bK}\Sigma X^T\bB.
\end{align*}
	Note that $\bP'[X]$ and $\Sigma'[X]$ can be solved by the iterative equations
	\begin{align*}
		\bP'[X] &= \sum^N_{i = 0} \big( \bA_{\bK}^T\big)^i\big(2X^T\bE_{\bK}\big)\big( \bA_{\bK}\big)^i \nonumber\\
		\Sigma'[X] &= \sum^N_{i = 0} \big(\bA_{\bK}\big)^i\big(- \bB X\Sigma\bA_{\bK}^T - \bA_{\bK}\Sigma X^T\bB\big)\big(\bA_{\bK}^T\big)^i. 
	\end{align*}
	Therefore, the action of the Hessian can be represented as
	\begin{align*}
		\nabla^2\cG(\bK)[X, X] &= 2\big\langle \bE_{\bK}'[X]\Sigma , X\big\rangle + 2 \big\langle \bE_{\bK}\Sigma'[X], X\big\rangle,
	\end{align*}
	where $\bE_{\bK}'[X]$ and $\Sigma'[X]$ follow the definitions in \eqref{eqn:E'} and \eqref{eqn:sigmak'}, respectively. This completes the proof of \eqref{eqn:exact_hessian_K}.
\end{proof}

\subsection{Auxiliary Bounds: The Inner Loop Problem}\label{sec:bounds_L}
\begin{lemma}
	For a fixed outer loop control gain matrix $\bK$ and for any $\bL \in \cS_{\bL}(a)$, there exist positive auxiliary constants reported in the left column of Table \ref{table:L}, such that the bounds in the right column of Table \ref{table:L} hold.
\end{lemma}
\begin{table}[!h]

\begin{tabular*}{\textwidth}{
  @{\extracolsep{\fill}}
  l
  >{$\displaystyle}c<{\vphantom{\sum_{1}{N}}$}
  >{\refstepcounter{equation}(\theequation)}r
  @{}
}
\toprule
\textbf{Auxiliary Constants} & \multicolumn{1}{c}{\textbf{Auxiliary Bounds: The Inner Loop Problem}} & \multicolumn{1}{c}{} \\
\midrule
$c_{\iota_1} := c_{\bP_{\bL}, a}$  &
  	\|\bP_{\bL}\| \leq  c_{\iota_1} &
  \label{bound:P_L}
\\
$c_{\iota_2} := sNC_m$ & 
  \|\Sigma_{\bL}\| \leq  c_{\iota_2} & \label{bound:sigma_L}
\\
$c_{\iota_3} :=$\small $\sqrt{(\|\bR^w\| + \|\bD\|^2c_{\iota_1})(a - \cG(\bL^*)))}$\normalsize &
  \|\bE_{\bL}\| \leq c_{\iota_3} & \label{bound:E_L}
\\
 $c_{\iota_4} := \frac{c_{\iota_3}+\|\bB\|\|\tilde{\bA}\|c_{\iota_1}}{\lambda_{\min}(\bR^w)}$&
  \|\nabla\cG(\bL)\| \leq c_{\iota_2}c_{\iota_3} & \label{bound:grad_L}
\\
& 
  \|\bL\| \leq c_{\iota_4} & \label{bound:L}
\\
&
  \|\cT_{\bL}\| \leq c_{\iota_2} & \label{bound:TL}
\\
\bottomrule
\end{tabular*}
\caption{Auxiliary constants and bounds for the Inner loop problem.}\label{table:L}
\end{table}

\begin{proof}
	First, due to the finite-horizon setting that is considered in this paper, mappings $\bL \rightarrow \bP_{\bL}$ is continuous for a fixed outer loop control gain matrix $\bK$. Thus, there exist uniform upper bounds such that for $\bL \in \cS_{\bL}(a)$,
	\begin{align*}
		\|\bP_{\bL}\| \leq c_{\bP_{\bL}, a} = c_{\iota_1}.
	\end{align*}
	This proves \eqref{bound:P_L}. Next, because that $\Sigma_{\bL}$ is the solution of the Lyapunov equation
	\begin{align*}
		\Sigma_{\bL} = \tilde{\bA}_{\bL}\Sigma_{\bL}\tilde{\bA}_{\bL}^T + \Sigma_0,
	\end{align*} 
	where $\Sigma_0 = \EE[\bm{\xi}\bm{\xi}^T]$ and $\|\bm{\xi}\|^2 \leq sC_m$ almost surely due to the assumption on the distribution $\cD$. Since $\Sigma_{\bL}$ can be solved iteratively via 
	\begin{align*}
		\Sigma_{\bL} = \sum^{N}_{t=0}\big(\tilde{\bA}_{\bL}\big)^{t}\Sigma_{0} \big((\tilde{\bA}_{\bL})^T\big)^t,
	\end{align*}
	we can bound $\|\Sigma_{\bL}\|$ by $\|\Sigma_{\bL}\| \leq sNC_m = c_{\iota_1}$. This proves \eqref{bound:sigma_L}. Next, we prove \eqref{bound:E_L} by deriving a lower bound that provides counterparts of the results in Lemma \ref{lemma:gd_L}. Specifically, under the assumption that $\cG(\bL') \geq \cG(\bL^*)$, we have
	\begin{align*}
		\cG(\bL) - \cG(\bL^*) &\geq \cG(\bL) - \cG(\bL') \geq \Tr\big(\Sigma_{\bL'} \bE^T_{\bL}\bF^{-1}_{\bL}\bE_{\bL} \big) \\
			&\geq \frac{\lambda_{\min}(\Sigma_{\bL'})}{\|\bF_{\bL}\|}\Tr\big(\bE^T_{\bL}\bE_{\bL} \big) \geq \frac{1}{\|\bF_{\bL}\|}\Tr\big(\bE^T_{\bL}\bE_{\bL} \big).
	\end{align*}
	The last inequality is because of $\Sigma_{\bL'} \geq \Sigma_0 = \textbf{I}$. By utilizing \eqref{bound:P_L}, it leads to 
	\begin{align*}
		\Tr\big(\bE^T_{\bL}\bE_{\bL} \big) \leq \|\bF_{\bL}\|(\cG(\bL) - \cG(\bL^*)) \leq (\|\bR^w\| + \|\bD\|^2c_{\iota_1})(a - \cG(\bL^*)) = c_{\iota_3}^2.
	\end{align*}
Then, \eqref{bound:E_L} can be concluded. Furthermore, invoking Lemma 25 of \cite{fazel2018global} and applying \eqref{bound:sigma_L} yields
\begin{align*}
	\|\nabla\cG(\bL)\|^2 \leq \Tr(\Sigma_{\bL}\bE^T_{\bL}\bE_{\bL}\Sigma_{\bL}) \leq \|\Sigma_{\bL}\|^2\Tr(\bE^T_{\bL}\bE_{\bL}) \leq \big(c_{\iota_2}c_{\iota_3} \big)^2.
\end{align*}
Taking square-root of both sides proves \eqref{bound:grad_L}. Next, Lemma 25 of \cite{fazel2018global} suggests that
\begin{align*}
	\|\bL\| \leq \frac{\sqrt{(\|\bR^w\| + \|\bD\|^2c_{\iota_1})(a - \cG(\bL^*))}}{\lambda_{\min}(\bR^w)} + \frac{\|\bD\|\|\tilde{\bA}\|c_{\iota_1}}{\lambda_{\min}(\bR^w)} = \frac{c_{\iota_3}+\|\bB\|\|\tilde{\bA}\|c_{\iota_1}}{\lambda_{\min}(\bR^w)} = c_{\iota_4}, 
\end{align*}
yielding \eqref{bound:L}. Lastly, combining the results from Lemma 17 of \cite{fazel2018global} with \eqref{bound:sigma_L} yields \eqref{bound:TL} as follows
	\begin{align*}
		\|\cT_{\bL}\| \leq \|\Sigma_{\bL}\| \leq c_{\iota_2}.
	\end{align*}
	This completes the proof.
\end{proof}


\subsection{Auxiliary Bounds: The Outer Loop Problem}\label{sec:bounds_K}
\begin{lemma}
	For $\bK \in \cS_{\bK}(a)$, there exist positive auxiliary constants reported in the left column of Table \ref{table:K}, such that the bounds in the right column of Table \ref{table:K} hold.
\end{lemma}

\begin{table}[!h]

\begin{tabular*}{\textwidth}{
  @{\extracolsep{\fill}}
  l
  >{$\displaystyle}c<{\vphantom{\sum_{1}{N}}$}
  >{\refstepcounter{equation}(\theequation)}r
  @{}
}
\toprule
\textbf{Auxiliary Constants} & \multicolumn{1}{c}{\textbf{Auxiliary Bounds: The Outer Loop Problem}} & \multicolumn{1}{c}{} \\
\midrule
$c_{\kappa_1} := c_{\bP_{\bK}, a}$  &
  	\|\bP_{\bK}\| \leq  c_{\kappa_1} &
  \label{bound:P_K}
\\
$c_{\kappa_2} := sNC_m$ & 
  \|\Sigma_{\bK}\| \leq  c_{\kappa_2} & \label{bound:sigma_K}
\\
$c_{\kappa_3} := c_{\kappa_1} + \|\bR^w\|\|\bD\|^2c^2_{\kappa_1}$ &
  \|\tilde{\bP}_{\bK}\| \leq c_{\kappa_3} & \label{bound:barP_K}
\\
$c_{\kappa_4} :=$\small $\sqrt{(\|\bR^u\| + \|\bB\|^2c_{\kappa_3})(a - \cG(\bK^*))}$\normalsize &
  \|\bE_{\bK}\| \leq c_{\kappa_4} & \label{bound:E_K}
\\
 $c_{\kappa_5} := \frac{c_{\kappa_4}+\|\bB\|\|\bA\|c_{\kappa_3}}{\lambda_{\min}(\bR^u)}$&
  \|\nabla\cG(\bK)\| \leq c_{\kappa_2}c_{\kappa_4} & \label{bound:grad_K}
\\
$c_{\kappa_6} :=$ \small$2\|\bB\|c_{\kappa_2}c_{\kappa_4}(\|\bA\| + \|\bB\|c_{\kappa_5})$\normalsize& 
  \|\bK\| \leq c_{\kappa_5} & \label{bound:K}
\\
\hspace{2em}\small$+(4 + 2\|\bR^w\|\|\bD\|^2c_{\kappa_1})\|\bR^w\|\|\bB\|^2\|\bD\|^2$\normalsize&
  \|\cT_{\bK}\| \leq c_{\kappa_2} & \label{bound:TK}
\\
\hspace{2em}\small$c_{\kappa_1}c_{\kappa_2}c_{\kappa_4}(c_{\kappa_5}+\|\bA\|) + \|\bR^u\| + \|\bB\|^2c_{\kappa_3}$\normalsize&
  \|\bE'_{\bK}\| \leq c_{\kappa_6} & \label{bound:EK'}
\\
\bottomrule
\end{tabular*}
\caption{Auxiliary constants and bounds for the outer loop problem.}\label{table:K}
\end{table}


\begin{proof}
First, due to the finite-horizon setting that is considered in this paper, mappings $\bK \rightarrow \bP_{\bK}$ is continuous. Thus, there exist an uniform upper bound such that for $\bK \in \cS_{\bK}(a)$,
	\begin{align*}
		\|\bP_{\bK}\| \leq c_{\bP_{\bK}, a} = c_{\kappa_1}.
    \end{align*}
	This proves \eqref{bound:P_K}. Next, because that $\Sigma_{\bK}$ is the solution of the Lyapunov equation
	\begin{align*}
		\Sigma_{\bK} = \bA_{\bK, \bL}\Sigma_{\bK} \bA_{\bK, \bL}^T + \Sigma_0,
	\end{align*} 
	where $\Sigma_0 = \EE[\bm{\xi}\bm{\xi}^T]$ and $\|\bm{\xi}\|^2 \leq sC_m$ almost surely due to the assumption on the distribution $\cD$. Since $\Sigma_{\bK}$ can be solved iteratively via 
	\begin{align*}
		\Sigma_{\bK} = \sum^{N}_{t=0}\big(\bA_{\bK, \bL}\big)^{t}\Sigma_{0} \big(\bA_{\bK, \bL}^T\big)^t,
	\end{align*}
	we can bound $\|\Sigma_{\bK}\|$ by $\|\Sigma_{\bK}\| \leq sNC_m = c_{\kappa_1}$. This proves \eqref{bound:sigma_K}. Furthermore, by the definition of $\tilde{\bP}_{\bK}$, we can prove \eqref{bound:barP_K} by
	\begin{align*}
		\|\tilde{\bP}_{\bK}\| \leq c_{\kappa_1} + \|\bR^w - \bD^T\bP_{\bK}\bD\|\|\bD\|^2c^2_{\kappa_1} \leq c_{\kappa_1} + \|\bR^w\|\|\bD\|^2c^2_{\kappa_1} := c_{\kappa_3}.
	\end{align*}
	Subsequently, we consider $\bK' = \bK - \bF_{\bK}^{-1}\bE_{\bK}$, which is the Gauss-Newton update \eqref{eqn:gn_K} with stepsize $1/2$. Under the assumption that $\cG(\bK^*) \leq \cG(\bK')$, we have
	\begin{align*}
		\cG(\bK) - \cG(\bK^*) &\geq \cG(\bK) - \cG(\bK') \geq \Tr(\bE^T_{\bK}\bF_{\bK}^{-1}\bE_{\bK}) \geq \frac{1}{\|\bF_{\bK}\|}\Tr(\bE^T_{\bK}\bE_{\bK}).
	\end{align*}
	This yields
	\begin{align*}
		\Tr(\bE^T_{\bK}\bE_{\bK}) &\leq \|\bF_{\bK}\|(\cG(\bK) - \cG(\bK^*)) \leq (\|\bR^u\| + \|\bB\|^2c_{\kappa_3})(a - \cG(\bK^*)) = c_{\kappa_4}^2.
	\end{align*}
	Therefore, we prove \eqref{bound:E_K}. Also, by invoking Lemma 25 of \cite{fazel2018global}, we can derive that
	\begin{align*}
		\|\nabla\cG(\bK)\|^2 &\leq \Tr(\Sigma_{\bK}\bE^T_{\bK}\bE_{\bK}\Sigma_{\bK}) \leq \|\Sigma_{\bK}\|^2 \Tr(\bE^T_{\bK}\bE_{\bK}) \leq (c_{\kappa_2}c_{\kappa_4})^2.
	\end{align*}
	Taking square root of both sides proves \eqref{bound:grad_K}. Next, Lemma 25 of \cite{fazel2018global} suggests that
\begin{align*}
	\|\bK\| \leq \frac{\sqrt{(\|\bR^u\| + \|\bB\|^2c_{\kappa_3})(a - \cG(\bK^*))}}{\lambda_{\min}(\bR^u)} + \frac{\|\bB\|\|\bA\|c_{\kappa_3}}{\lambda_{\min}(\bR^u)} = \frac{c_{\kappa_4}+\|\bB\|\|\bA\|c_{\kappa_3}}{\lambda_{\min}(\bR^u)} = c_{\kappa_5}, 
\end{align*}
yielding \eqref{bound:K}. Furthermore,  combining Lemma 17 of \cite{fazel2018global} with \eqref{bound:sigma_K} yields \eqref{bound:TK} as follows
	\begin{align*}
		\|\cT_{\bK}\| \leq \|\Sigma_{\bK}\| \leq c_{\kappa_2}.
	\end{align*}
Lastly, we focus on proving the upper bound for $\|\bE'_{\bK}\|$. To start with, by the definition of $\bP_{\bK}'$ in \eqref{eqn:pk'}, we can show that
\begin{align*}
	\|\bP_{\bK}'\| \leq 2\|\cT_{\bK}\|\|\bE_{\bK}\| \leq 2c_{\kappa_2}c_{\kappa_4}.
\end{align*}
Then, by the definition of $\bE'_{\bK}$ in \eqref{eqn:E'}, we can show that
\begin{align*}
	\|\bE'_{\bK}\| &\leq \|\bR^u\| + \|\bB\|^2c_{\kappa_3} + 2\|\bB\|c_{\kappa_2}c_{\kappa_4}(\|\bA\| + \|\bB\|c_{\kappa_5}) \\
	&\hspace{1em} + 4\|\bR^w\|\|\bB\|^2\|\bD\|^2c_{\kappa_1}c_{\kappa_2}c_{\kappa_4}c_{\kappa_5} + 2\|\bR^w\|^2\|\bB\|^2\|\bD\|^4c^2_{\kappa_1}c_{\kappa_2}c_{\kappa_4}c_{\kappa_5}\\
	&\hspace{1em} + 4\|\bR^w\|\|\bA\|\|\bB\|^2\|\bD\|^2c_{\kappa_1}c_{\kappa_2}c_{\kappa_4} + 2\|\bR^w\|^2\|\bA\|\|\bB\|^2\|\bD\|^4c^2_{\kappa_1}c_{\kappa_2}c_{\kappa_4} \\
	&= \|\bR^u\| + \|\bB\|^2c_{\kappa_3} + 2\|\bB\|c_{\kappa_2}c_{\kappa_4}(\|\bA\| + \|\bB\|c_{\kappa_5})\\
	&\hspace{1em} + (4 + 2\|\bR^w\|\|\bD\|^2c_{\kappa_1})\|\bR^w\|\|\bB\|^2\|\bD\|^2c_{\kappa_1}c_{\kappa_2}c_{\kappa_4}(c_{\kappa_5}+\|\bA\|) = c_{\kappa_6}.
\end{align*}
This completes the proof of \eqref{bound:EK'}
\end{proof}

%\subsection{Proof of Theorem \ref{theorem:free_pg_L}}
% \begin{proof}
% 	For ease of notation, we define $\Delta_l = \cG(\bL_l) - \cG(\bL^*)$ as the optimality gap between the control gain matrix $\bL_l$ at iteration $l$ and the optimal control gain matrix $\bL^*$. Also, we define
% 	\begin{align*}
% 		G_{\infty} := \sup_{\bL}~ \|\nabla\cG(\bL)\|, \quad G_2 := \sup_{\bL}~ \EE~\Big[\big\|\nabla\cG(\bL) - \EE~\big[\nabla\cG(\bL) \mid \bL\big]\big\|^2\Big]
% 	\end{align*}
% 	as the uniform bounds on the gradient norm and its variance, respectively.  Suppose that the algorithm parameters are chosen to satisfy \eqref{eqn:one_point_req}, we first focus on proving that for any iteration index $l$, inequality
% \begin{align}\label{eqn:delta_bound}
% 	\EE_l[\Delta_{l+1}] \leq (1-\frac{\eta c_g}{4})\Delta_l + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta c_g \frac{\epsilon_{\bL}\delta}{20}
% \end{align}
% holds, where $\EE_l[\Delta_{l}]$ denotes the expectation of the optimality gap at iteration $l$. From page 24 of \cite{malik2020derivative}, we can apply Markov's inequality to obtain
% 	\begin{align*}
% 		\EE_l[\Delta_{l+1} - \Delta_l] \leq - \frac{\eta c_g}{2}\Delta_l + \frac{\eta c_g}{4}\Delta_l + 4\frac{\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta^2\psi_{\bL}^3r_{\bL}^2,
% 	\end{align*}
% 	where $\theta_{\bL} = \min\{\frac{1}{2\psi_{\bL}}, \frac{1}{l_{\bL}}\}$. Since \eqref{eqn:one_point_req} is satisfied, we can derive that $\frac{4\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$ and $\eta^2\psi_{\bL}^3r_{\bL}^2 \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$. This completes the proof of \eqref{eqn:delta_bound}. Subsequently, we want to show that if \eqref{eqn:one_point_req} is satisfied, then we will have 
% 	\begin{align}\label{eqn:intermediate_E}
% 		\EE[\Delta_{\cL}] \leq \epsilon_{\bL}\delta.
% 	\end{align}
% 	with probability $1$. Suppose $\eta \leq \frac{\epsilon_{\bL} c_g\delta}{40\psi_{\bL} G_2}$, we have
% 	\begin{align*}
% 		\EE [\Delta_{l+1}] &\leq \Big(1-\frac{\eta c_g}{4}\Big)^{l+1}\Delta_0 + \Big(\frac{\psi_{\bL}\eta^2G_2}{2} + \frac{\eta c_g \epsilon_{\bL}\delta}{20}\Big)\sum^{l}_{i=0}\Big(1 - \frac{\eta c_g}{4}\Big)^i \\
% 		&\leq \Big(1-\frac{\eta c_g}{4}\Big)^{l+1}\Delta_0 + \frac{2\psi_{\bL}\eta G_2}{c_g} + \frac{\epsilon_{\bL}\delta}{5} \\
% 		& \leq \Big(1-\frac{\eta c_g}{4}\Big)^{l+1}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4}.
%  	\end{align*}
%  	Let $\cL = l+1$, we can verify that if $\cL = \frac{4}{\eta c_g}\log(\frac{4\Delta_0}{3\delta\epsilon_{\bL}})$, then
%  	\begin{align*}
%  		\Big(1-\frac{\eta c_g}{4}\Big)^{\cL}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4} \leq \epsilon_{\bL}\delta.
%  	\end{align*}
%  	This leads to $\EE[\Delta_{\cL}] \leq \epsilon_{\bL}\delta$.  Moreover, applying Markov's inequality leads to
% 	\begin{align*}
% 		P\{\Delta_\cL \geq \epsilon_{\bL}\} \leq \frac{1}{\epsilon_{\bL}}\EE[\Delta_{\cL}] \leq \delta,
% 	\end{align*}
% 	which implies $P\{\Delta_\cL \leq \epsilon_{\bL}\} > 1- \delta$. Lastly, we provide bounds for $G_2$ and $G_{\infty}$. By definition of the estimated cost function, their exists an absolute constant $c_1$ such that 
% 	\begin{align*}
% 		\cG(\bL + U, \bm{\xi}) = \bm{\xi}^T\bP_{\bL + U}\bm{\xi} \leq sC_m \EE_{\bm{\xi}} [\bm{\xi}^T\bm{\xi}]~ \|\bP_{\bL + U}\| \leq sC_mc_{1}.
% 	\end{align*}
% 	Therefore, as $\|U\|_F = r_{\bL}$, we can prove the following bound
% 	\begin{align*}
% 		G_{\infty} = \frac{\tilde{d}_{\bL}}{r_{\bL}}~\sup_{\bL+U}~ \overline{\cG} \leq \frac{sC_m\tilde{d}_{\bL}c_{1}}{r_{\bL}}, \quad G_2 \leq G^2_{\infty} \leq \Big(\frac{sC_m\tilde{d}_{\bL}c_{1}}{r_{\bL}}\Big)^2.
% 	\end{align*}
% 	Substitute the bounds into the requirements of $\eta$ completes the proof of the theorem. 
% \end{proof}
 
% \begin{lemma}
% 	For an initial control gain matrix $\bK_0 \in \cK$, there exists a smoothing radius 
% 	\begin{align}
% 		r_{\bK} \leq \min \Big\{ \bB_{\bK}, \frac{\lambda_{\min}(\bR^w - \bD^T\bP_{\bK_0}\bD)}{\|\bD\|_F^2\bB_{\bP}} \Big\}
% 	\end{align} 
% 	such that $\bK_0 + r_{\bK}U_i \in \cK$, $\|U_i\|_F = 1$.
% \end{lemma}
% \begin{proof}
% 	For $\bK_0$ initialized within the set $\cK$, we have $\lambda_{\min}(\bR^w - \bD^T\bP_{\bK_0}\bD) :=X > 0$. Then, suppose $\bK' = \bK_0 + r_{\bK}U$, where $\|U\|_F = 1$, Lemma \ref{lemma:riccati_perturb} suggests that if 
% 	\begin{align*}
% 		\|\bK' - \bK_0\|_F = r_{\bK} \leq \min \Big\{ \bB_{\bK}, \frac{X}{\|\bD\|_F^2\bB_{\bP}} \Big\}, 
% 	\end{align*}
% 	then $\|\bP_{\bK'} - \bP_{\bK_0}\|_F \leq \frac{X}{\|\bD\|_F^2}$ holds, which leads to the condition
% 	\begin{align*}
% 		\|\bD^T(\bP_{\bK'} - \bP_{\bK_0})\bD\| \leq \|\bD^T(\bP_{\bK'} - \bP_{\bK_0})\bD\|_F \leq \|\bD\|_F^2\|\bP_{\bK'} - \bP_{\bK_0}\|_F \leq  X.
% 	\end{align*}
% 	This condition is sufficient to derive 
% 	\begin{align*}
% 		\bD^T(\bP_{\bK'} - \bP_{\bK_0})\bD \leq X\bI \Rightarrow \bD^T\bP_{\bK'}\bD \leq \bD^T\bP_{\bK_0}\bD +X\bI\Rightarrow \bR^w - \bD^T\bP_{\bK'}\bD >0.
% 	\end{align*}
% 	Therefore, $\bK' \in \cK$ is guaranteed, which completes the proof.
% \end{proof}
% 
% \begin{lemma}(Riccati Perturbation)\label{lemma:riccati_perturb}
% 	For any control gain matrix $\bK, \bK' \in \cK$, there exists some constant $\cB_{\bK} > 0$ such that if $\|\bK' - \bK\|_F \leq \cB_{\bK}$, the inequlity
% 	\begin{align}
% 		\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \cB_{\bP}\|\bK'-\bK\|_F
% 	\end{align}
% 	holds for some constant $\cB_{\bP}>0$.
% \end{lemma}
%% \xzedit{Whether Sun98 can be applied. Here, the inner loop player solves a Riccati equation with indefinite Q matrix. but for a given $\bK$, $\bP_{\bK} > 0$.}
% \begin{proof}
% 	The proof mostly follows from Proposition B.1 of \cite{zhang2019policy}. First of all, for a given $\bK \in \cK$, there exists $\bP_{\bK} \geq 0$ that solves the Riccati equation for the inner loop minimization problem with transition matrix $\tilde{\bA}_{\bK} = \bA-\bB\bK$ and state-weighting matrix $\tilde{\bQ} = -\bQ - \bK^T\bR^u\bK$. Recall that $\bL(\bK) = (-\bR^w + \bD\bP_{\bK}\bD)^{-1}\bD^T\bP_{\bK}\tilde{\bA}_{\bK}$, we have
% 	\begin{align*}
% 		\tilde{\bA}_{\bK} - \bD\bL(\bK) = \tilde{\bA}_{\bK} + \bD(\bR^w - \bD^T\bP_{\bK}\bD)^{-1}\bD^T\bP_{\bK}\tilde{\bA}_{\bK} = [\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\tilde{\bA}_{\bK},
% 	\end{align*}
% 	where the last equality comes from the matrix inversion lemma. Then, we let $\Delta = \bK'-\bK$ and follow page 44 of \cite{zhang2019policy} to define the following quantities
% 	\begin{align*}
% 		&\delta = \|\tilde{\bA}_{\bK'} - \tilde{\bA}_{\bK}\| = \|\bB\Delta\|_F, \quad f = \|[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\|_F, \quad g = \|\bD(\bR^w)^{-1}\bD\|_F \\
% 		&\phi = \|[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\tilde{\bA}_{\bK}\|_F, \quad \gamma = f\delta(2\phi + f\delta), \quad \psi = \|\bP_{\bK}[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\|_F \\
% 		&T_{\bK} = \bI - \big[\tilde{\bA}_{\bK} - \bD\bL(\bK)\big]^T\otimes\big[\tilde{\bA}_{\bK} - \bD\bL(\bK)\big]^T, \quad l = \|T_{\bK}^{-1}\|^{-1}_F, \quad H = \bP_{\bK}[\bI - \bD(\bR^w)^{-1}\bD\bP_{\bK}]^{-1}\tilde{\bA}_{\bK} \\
% 		&p = \big\|T_{\bK}^{-1}\big[\bI \otimes H^T + (H^T \otimes \bI)\Pi\big]\big\|_F, \quad \epsilon = \frac{1}{l}\big\|\Delta^T\bR^u\bK + \bK^T\bR^u\Delta + \Delta^T\bR^u\Delta\big\|_F + \big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \\
% 		&\alpha = f(\|\tilde{\bA}_{\bK}\|_F + \|\bB\Delta\|_F), \quad \theta = \frac{l}{\phi + \sqrt{\phi^2 + l}},
% 	\end{align*}
% 	where $\Pi$ is the vec-perturbation matrix. Here, $l$ is finite and uniformly bounded above zero because $\tilde{\bA}_{\bK} - \bD\bL(\bK)$ is actually concatenation of blocks. Then, we require the following sufficient conditions to hold \cite{sun1998perturbation, zhang2019policy}
% 	\begin{align}\label{eqn:perturb_conditions}
% 		1-fg\xi_* \geq 0, \quad \frac{f\delta+\phi fg\xi_*}{1-fg\xi_*} \leq \theta
% 	\end{align}
% 	where $\xi_* = (2l\epsilon)\cdot(l/2 + lfg\epsilon)^{-1}$. Additionally, we require
% 	\begin{align}\label{eqn:gamma}
% 		\gamma = f\delta(2\phi + f\delta) &\leq f\|\bB\Delta\|_F(2\phi+2l+f\|\bB\Delta\|_F) \nonumber\\
% 		&\leq 2f(\phi+l)\|\bB\|_F\|\Delta\|_F + f^2\|\bB\|_F^2\|\Delta\|_F^2 \leq l/2
% 	\end{align}
% 	and 
% 	\begin{align}\label{eqn:epsilon}
% 		\epsilon &= \frac{1}{l}\big\|\Delta^T\bR^u\bK + \bK^T\bR^u\Delta + \Delta^T\bR^u\Delta\big\|_F + \big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \nonumber\\
% 		&\leq \frac{1}{l}\big(2\|\bR^u\bK\|_F\|\Delta\|_F + \|\bR^u\|_F\|\Delta\|_F^2\big) + \big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \leq \frac{(l/2)^2}{2lfg(l+2a)} = \frac{l}{8fg(l+2a)}.
% 	\end{align}
% 	Then, as $\gamma \leq l/2$, we can further have
% 	\begin{align}
% 		\frac{(l/2)^2}{2lfg(l+2a)} \leq \frac{(l-\gamma)^2}{lfg(l-\gamma+2\alpha + \sqrt{(l-\gamma+2\alpha)^2-(l-\gamma)^2})}.
% 	\end{align}
% 	This implies the condition (4.41) of \cite{sun1998perturbation} holds. Therefore, Theorem 4.1 of \cite{sun1998perturbation} suggests that 
% 	\begin{align}\label{eqn:pk_bound}
% 		\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \xi_* &= \frac{2l\epsilon}{l/2 + lfg\epsilon} \leq 4\epsilon = \frac{4}{l}\big\|\Delta^T\bR^u\bK + \bK^T\bR^u\Delta + \Delta^T\bR^u\Delta\big\|_F+ 4\big(p + \frac{\psi\delta}{l}\big)\|\bB\Delta\|_F \nonumber\\
% 		&\leq \frac{8}{l}\|\bR^u\bK\|_F\|\Delta\|_F + \frac{4}{l}\|\bR^u\|_F\|\Delta\|_F^2 + 4p\|\bB\|_F\|\Delta\|_F +4\frac{\psi}{l}\|\bB\|_F^2\|\Delta\|_F^2
%    \end{align}
%    Then, following the proof of Proposition 1 in \cite{zhang2019policy}, we can have the sufficient conditions of \eqref{eqn:perturb_conditions}, \eqref{eqn:gamma}, and \eqref{eqn:epsilon} such that \eqref{eqn:pk_bound} is satisfied. This sufficient condition can be represented as
%%    \begin{align}
%%    	fg\frac{2\epsilon}{1/2 + fg\epsilon} \leq \Rightarrow fg\epsilon \leq 1/2, \quad f\delta + (\phi+\theta)fg\xi_* \leq \theta
%%    \end{align}
%%    where one sufficient condition for the second one to hold is 
%%    \begin{align}\label{eqn:condition1}
%%    	f\delta + 4(\phi+\theta)fg\epsilon \leq \theta,
%%    \end{align}
%%    as $\xi_* \leq 2\epsilon/(1/2) = 4\epsilon$. Since $f\delta\geq 0$ and $fg\epsilon \geq 0$, \eqref{eqn:condition1} implies that $fg\epsilon \leq 1/2$. For \eqref{eqn:condition1} to hold, we can let
%%    \begin{align}
%%    	f\|\bB\|\|\Delta\| + 4(\phi+\theta)fg\big(\frac{2}{l}\|\bR^u\bK\|\|\Delta\| + \frac{1}{l}\|\bR^u\|\|\Delta\|^2 + p\|\bB\|\|\Delta\| + \frac{\psi}{l}\|\bB\|^2\|\Delta\|^2\big) \leq \theta,
%%    \end{align}
%%    which can be satisfied by choosing $\|\Delta\|$ such that
%%    \begin{align}
%%    	\hspace{-0.5em}\|\Delta\| \leq \min\Big\{\frac{\|\bB\| + 4(\phi+\theta)g(2\|\bR^u\bK\|/l + p\|\bB\|)}{4(\phi+\theta)g(\|\bR^u\|/l + \psi\|\bB\|^2/l)}, \frac{\theta}{2f\|\bB\|+8f(\phi+\theta)g(2\|\bR^u\bK\|/l + p\|\bB\|)}\Big\}
%%    \end{align}
%%    Subsequently, \eqref{eqn:gamma} gives
%%    \begin{align}
%%    	2f(\phi + l)\|\bB\|\|\Delta\| + f^2\|\bB\|^2\|\Delta\|^2 \leq l/2,
%%    \end{align}
%%    which can be satisfied by choosing $\|\Delta\|$ such that
%%     \begin{align}
%%    	\|\Delta\| \leq \min\Big\{\frac{2(\phi+l)}{f\|\bB\|}, \frac{l}{8f(\phi+l)\|\bB\|}\Big\}
%%    \end{align}
%%    \xzedit{maybe should just cite the result}
%%    The three conditions can be satisfied by choosing
%    \begin{align}
%    	\hspace{-0.5em}\|\Delta\|_F \leq \min\Big\{1, \frac{2\|\bR^u\bK\|_F + (p+1)l\|\bB\|_F}{\|\bR^u\|_F + \psi\|\bB\|_F^2}, \frac{l}{16fg[l+2f(\|\tilde{\bA}_{\bK}\|_F + \|\bB\|_F)](\|\bR^u\bK\|_F/l + 2(p+1)\|\bB\|_F)}\Big\}
%    \end{align}
%    Under this condition, the perturbation of the Riccati equation can be bounded by
%    \begin{align}
%    	\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \Big[\frac{\|\bB\|_F}{(\psi+\theta)g} + \frac{16\|\bR^u\bK\|_F}{l} + 8p\|\bB\|_F\Big] \cdot\|\Delta\|_F
%    \end{align}
%    Therefore, there exists some $\cB_{\bK} >0$ and $\cB_{\bP} = \frac{\|\bB\|_F}{(\psi+\theta)g} + \frac{16\|\bR^u\bK\|_F}{l} + 8p\|\bB\|_F$ such that $\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \cB_{\bP}\|\bK'-\bK\|_F$ for $\bK', \bK \in \cK$ and $\|\bK' - \bK\|_F \leq \cB_{\bK}$. This completes the proof.
% \end{proof}
 
% \begin{lemma}(Local Lipschitz and Smooth)
% 	For $\bK, \bK' \in \cK$ and let the inequality  \xznote{Do we actually need smoothness}
% 	\begin{align}\label{eqn:lipschitz_bound}
% 		\|\bK' - \bK\|_F \leq \cB_{\bK}
% 	\end{align}
% 	holds. Then, we have
% 	\begin{align}\label{eqn:out_lipschitz}
% 		|\cG(\bK') - \cG(\bK)| &\leq l_{\bK}\|\bK'-\bK\|_F \\
% 		\|\nabla\cG(\bK') -\nabla\cG(\bK)\|_F &\leq \psi_{\bK}\|\bK'-\bK\|_F \label{eqn:out_smooth} 
% 	\end{align}
% \end{lemma}
% \begin{proof}
% 	By definition, 
% 	\begin{align}
% 		|\cG(\bK') - \cG(\bK)| = \Tr(\bP_{\bK'}) - \Tr(\bP_{\bK}) \leq s\|\bP_{\bK'} - \bP_{\bK}\| \leq s\|\bP_{\bK'} - \bP_{\bK}\|_F.
% 	\end{align}
% 	Applying Lemma \ref{lemma:riccati_perturb} and the condition \eqref{eqn:lipschitz_bound} yields
% 	\begin{align}
% 		\|\bP_{\bK'} - \bP_{\bK}\|_F \leq \bB_{\bP}\|\bK'-\bK\|_F.
% 	\end{align}
% 	Therefore, substituting $l_{\bK} = s\cB_{\bP}$ completes the proof of \eqref{eqn:out_lipschitz}. Next, we focus on showing \eqref{eqn:out_smooth}. First, we invoke Lemma 13 of \cite{fazel2018global} to obtain
% 	\begin{align}
% 		\|\bP_{\bK}\| \leq \cG(\bK).
% 	\end{align}
% 	Next, because that $\Sigma_{\bK}$ is the solution of the Lyapunov equation
%	\begin{align*}
%		\Sigma_{\bK} = \bA_{\bK, \bL}\Sigma_{\bK} \bA_{\bK, \bL}^T + \Sigma_0,
%	\end{align*} 
%	where $\Sigma_0 = \EE[\bm{\xi}\bm{\xi}^T]$ and $\|\bm{\xi}\|^2 \leq sC_m$ almost surely due to the assumption on the distribution $\cD$. Since $\Sigma_{\bK}$ can be solved iteratively via 
%	\begin{align*}
%		\Sigma_{\bK} = \sum^{N}_{t=0}\big(\bA_{\bK, \bL}\big)^{t}\Sigma_{0} \big(\bA_{\bK, \bL}^T\big)^t,
%	\end{align*}
%	we can bound $\|\Sigma_{\bK}\|$ by $\|\Sigma_{\bK}\| \leq sNC_m$. Subsequently, by the gradient formula in Lemma \ref{lemma:exact_PG_K} and suppose \eqref{eqn:lipschitz_bound} is enforced, we have
%	\begin{align}
%		\|\nabla\cG(\bK') - \nabla\cG(\bK)\|_F &= \|(\bE_{\bK'} - \bE_{\bK})\Sigma_{\bK'} + \bE_{\bK}(\Sigma_{\bK'} - \Sigma_{\bK})\|_F \\
%		&\leq \|\bE_{\bK'} - \bE_{\bK}\|_F\|\Sigma_{\bK'}\| + \|\bE_{\bK}\|_F\|\Sigma_{\bK'} - \Sigma_{\bK}\| \\
%		&\leq 
%	\end{align}
%	
%	\begin{align*}
%		\|\bE_{\bK'} - \bE_{\bK}\|_F &= 2\|(\bR^u + \bB^T\tilde{\bP}_{\bK'}\bB)\bK -\bB^T\tilde{\bP}_{\bK'}\bA - (\bR^u + \bB^T\tilde{\bP}_{\bK}\bB)\bK + \bB^T\tilde{\bP}_{\bK}\bA\|_F \\
%		&\hspace{-2em}\leq 2\|\bR^u(\bK'-\bK) + \bB^T(\tilde{\bP}_{\bK'} - \tilde{\bP}_{\bK})\bB\bK' + \bB^T\tilde{\bP}_{\bK}\bB(\bK'-\bK) - \bB^T(\tilde{\bP}_{\bK'} -\tilde{\bP}_{\bK})\bA\|_F\\
%		&\hspace{-2em}\leq 2\|\bR^u\|_F\|\bK'-\bK\|_F + 2\|\bB^T(\tilde{\bP}_{\bK'}- \tilde{\bP}_{\bK})\bB\bK'\|_F + 2\|\bB^T\tilde{\bP}_{\bK}\bB(\bK'-\bK)\|_F + 2\|\bB^T(\tilde{\bP}_{\bK'} -\tilde{\bP}_{\bK})\bA\|_F
%	\end{align*}
%	\begin{align*}
%		\|\tilde{\bP}_{\bK'}- \tilde{\bP}_{\bK}\|_F &= \|\bP_{\bK'} - \bP_{\bK} + \bP_{\bK'}\bD(\bR^w - \bD^T\bP_{\bK'}\bD)^{-1}\bD^T\bP_{\bK'}  - \bP_{\bK}\bD(\bR^w - \bD^T\bP_{\bK}\bD)^{-1}\bD^T\bP_{\bK}\|_F\\
%		&\leq \|\bP_{\bK'} - \bP_{\bK}\|_F + \|\|_F
%	\end{align*}
% \end{proof}

 
 % Backup
% \begin{proof}
% 	For the ease of notation, we first define the set $\cS_{\bL_{10}} := \big\{\bL \mid \cG(\bL) - \cG(\bL^*) \leq 10\delta^{-1}\Delta_0\big\}$, where $\Delta_l = \cG(\bL_l) - \cG(\bL^*)$ is the optimality gap between the control gain matrix $\bL_l$ at iteration $l$ and the optimal control gain matrix $\bL^*$. Also, we define
% 	\begin{align*}
% 		G_{\infty} := \sup_{\bL \in \cS_{\bL_{10}}} \|\nabla\cG(\bL)\|, \quad G_2 := \sup_{\bL \in \cS_{\bL_{10}}} \EE~\Big[\big\|\nabla\cG(\bL) - \EE~\big[\nabla\cG(\bL) \mid \bL\big]\big\|^2\Big]
% 	\end{align*}
% 	as the uniform bounds on the gradient norm and its variance, respectively. Subsequently, let $\iota := \min\big\{l\mid \Delta_{l} > 10\delta^{-1}\Delta_0\big\}$ to denote the first iteration index where the iterates exits the sublevel set $\cS_{\bL_{10}}$. Then, we provide the following helper lemma with its proof deferred for smoother reading.
% \begin{lemma}\label{lemma:Deltabound}
% Let the algorithm parameters are chosen to satisfy \eqref{eqn:one_point_req}. Then, for any iteration index $l$ such that $\bL_l \in \cS_{\bL_{10}}$, we have
% \begin{align*}
% 	\EE_l[\Delta_{l+1}] \leq (1-\frac{\eta c_g}{4})\Delta_l + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta c_g \frac{\epsilon_{\bL}\delta}{20},
% \end{align*}
% where $\EE_l[\Delta_{l}]$ denotes the expectation of the optimality gap at iteration $l$. 
% \end{lemma}
%
% With the helper lemma above, we first show that if \eqref{eqn:one_point_req} is satisfied, then we will have 
% 	\begin{align}\label{eqn:intermediate_E}
% 		\EE[\Delta_{\cL} 1_{\iota > \cL}] \leq \frac{\epsilon_{\bL}\delta}{2}.
% 	\end{align}
% 	and $\iota > \cL$ with probability greater than $1-\frac{\delta}{2}$. To start with, we separate the proof into two cases. In the case where $\iota > \cL$, Lemma \ref{lemma:Deltabound} can be applied to to bound $\EE_l[\Delta_{l+1}]$. In the case where $\iota \leq \cL$, it is straightforward to see that $\EE_{l}[\Delta_{l+1}]1_{\iota > \cL} = 0$. Combining these two case with $\eta \leq \frac{\epsilon_{\bL} c_g\delta}{40\psi_{\bL} G_2}$ yields
% 	\begin{align*}
% 		\EE [\Delta_{l+1}1_{\iota > l+1}] &\leq \Big(1-\frac{\eta}{ c_g}\Big)^{l+1}\Delta_0 + \Big(\frac{\psi_{\bL}\eta^2G_2}{2} + \frac{\eta c_g \epsilon_{\bL}\delta}{20}\Big)\sum^{l}_{i=0}\Big(1 - \frac{\eta c_g}{4}\Big)^i \\
% 		&\leq \Big(1-\frac{\eta}{ c_g}\Big)^{l+1}\Delta_0 + \frac{2\psi_{\bL}\eta G_2}{c_g} + \frac{\epsilon_{\bL}\delta}{5} \\
% 		& \leq \Big(1-\frac{\eta}{ c_g}\Big)^{l+1}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4}.
%  	\end{align*}
%  	Let $\cL = l+1$, we can verify that if $\cL = \frac{4}{\eta c_g}\log(\frac{4\Delta_0}{\delta\epsilon_{\bL}})$, then
%  	\begin{align*}
%  		\Big(1-\frac{\eta}{ c_g}\Big)^{\cL}\Delta_0 + \frac{\epsilon_{\bL}\delta}{4} \leq \frac{\epsilon_{\bL}\delta}{2}.
%  	\end{align*}
%  	This leads to $\EE[\Delta_{\cL} 1_{\iota > \cL}] \leq \frac{\epsilon_{\bL}\delta}{2}$. It remains to show that the event $\iota \leq \cL$ happens with a probability lower than $\frac{\delta}{2}$. Then, for $l \in [\cL]$, we denote the stopped process
% 	\begin{align*}
% 		Y_l = \Delta_{\min(\iota, l)} + (\cL - l)\big(\frac{\eta^2\psi_{\bL}}{2}G_2 + \frac{\eta c_g\epsilon_{\bL}\delta}{20}\big).
% 	\end{align*}
% 	Following from \cite{malik2020derivative}, the stopped process sequence $Y_l$ is a super-martingale such that
% 	 \begin{align*}
% 		\EE_l[Y_{l+1}] \leq Y_{l}.
% 	\end{align*}
% 	Then, if $\epsilon_{\bL}$ is small enough to satisfy $\epsilon_{\bL} \log(\frac{4\Delta_0}{\delta\epsilon_{\bL}}) \leq \frac{16}{\delta}\Delta_0$, we can obtain
% 	\begin{align*}
% 		P \big\{\max_{l \in [\cL]} Y_l \geq 10\delta^{-1}\Delta_0\big\} &\leq \frac{\EE[Y_0]}{10\delta^{-1}\Delta_0} \\
% 		& = \frac{1}{10\delta^{-1}\Delta_0}\bigg(\Delta_0 + \cL\Big(\frac{\psi_{\bL}\eta^2}{2}G_2 + \frac{\eta\epsilon_{\bL} c_g \delta}{20}\Big)\bigg) \\
% 		& \leq \frac{1}{10\delta^{-1}\Delta_0}\bigg(\Delta_0 + \frac{2}{c_g}\log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big)\psi_{\bL}\eta G_2 + \log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big)\frac{\epsilon_{\bL}\delta}{5}\bigg)\\
% 		& \leq \frac{1}{10\delta^{-1}\Delta_0}\bigg(\Delta_0 + \frac{\delta\epsilon_{\bL}}{20}\log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big) + \frac{\epsilon_{\bL}\delta}{5}\log\big(\frac{4\Delta_0}{\delta\epsilon_{\bL}}\big)\bigg) \\
% 		&\leq \frac{\delta}{10\Delta_0}(5\Delta_0) = \frac{\delta}{2}.
% 	\end{align*}
% 	This completes the proof of \eqref{eqn:intermediate_E}. Moreover, this leads to
% 	\begin{align*}
% 		P\{\Delta_\cL \geq \epsilon_{\bL}\} &\leq P\{\Delta_{\cL}1_{\iota>\cL} \geq \epsilon_{\bL}\} + P\{1_{\iota \leq \cL}\}  \leq \frac{1}{\epsilon_{\bL}}\EE[\Delta_{\cL}1_{\iota>\cL}] + P\{1_{\iota \leq \cL}\} \leq \delta,
% 	\end{align*}
% 	which implies $P\{\Delta_\cL \leq \epsilon_{\bL}\} > 1- \delta$. Lastly, we provide bounds for $G_2$ and $G_{\infty}$. By definition of the cost function, if $r \leq \frac{10\delta^{-1}\cG(\bL_0)}{l_{\bL}}$ and $\|U\|_F = r_{\bL}$, then we will have
% 	\begin{align*}
% 		\cG(\bL + U, \bm{\xi}) = \bm{\xi}^T\bP_{\bL + U}\bm{\xi} \leq sC_m \EE_{\bm{\xi}} [\bm{\xi}^T\bP_{\bL + U}\bm{\xi}] &= sC_m\cG(\bL + U)\leq 20\delta^{-1}sC_m\cG(\bL_0).
% 	\end{align*}
% 	Therefore, 
% 	\begin{align*}
% 		G_{\infty} = \frac{\tilde{d}_{\bL}}{r_{\bL}}\sup_{\bL+U \in \cS_{\bL_{10}}} \overline{\cG} \leq \frac{20\delta^{-1}\tilde{d}_{\bL}sC_m}{r_{\bL}}\cG(\bL_0), \quad G_2 \leq G^2_{\infty} \leq \Big(\frac{20\delta^{-1}\tilde{d}_{\bL}sC_m}{r_{\bL}}\cG(\bL_0)\Big)^2.
% 	\end{align*}
% 	Substitute the bounds into the requirements of $\eta$ completes the proof of the theorem. Lastly, we focus on proving the helper Lemma \eqref{lemma:Deltabound}.
% 	From page 24 of \cite{malik2020derivative}, we have
% 	\begin{align*}
% 		\EE_l[\Delta_{l+1} - \Delta_l] \leq - \frac{\eta c_g}{2}\Delta_l + \frac{\eta c_g}{4}\Delta_l + 4\frac{\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} + \frac{\psi_{\bL}\eta^2}{2}G_2 + \eta^2\psi_{\bL}^3r_{\bL}^2,
% 	\end{align*}
% 	where $\theta_{\bL} = \min\{\frac{1}{2\psi_{\bL}}, \frac{1}{\lambda}\}$. Since \eqref{eqn:one_point_req} is satisfied, we can derive that $\frac{4\eta\psi_{\bL}^2r_{\bL}^2}{c_g\theta_{\bL}} \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$ and $\eta^2\psi_{\bL}^3r_{\bL}^2 \leq \frac{\eta c_g\epsilon_{\bL} \delta}{40}$. This completes the proof.
% \end{proof}


==> landscape.tex <==

\xznote{note that it is different from LQR, don't overclaim}


%Moreover, we can show that whenever $\bK \in \cK$, the cost function of the outer loop is smooth.
% 
% \begin{lemma}(``Smoothness'')\label{lemma:smooth_K} For $\bK \in \cK$, the cost function $\cG(\bK, \bL(\bK))$ of the outer loop is $\psi_2$-smooth. That is,
% \begin{align*}
% 	\|\nabla_{\bK}\cG(\bK', \bL(\bK')) - \nabla_{\bK}\cG(\bK, \bL(\bK))\|_F &\leq \psi_2 \|\bK'-\bK\|_F, \ \forall \bK \in \cK, 
% \end{align*}
% where $\psi_2$ is an absolute constant.
% \end{lemma}
 

%By Lemma \ref{assumption_game}, for any fixed $\bK_i \in \overline{\cK}$, the maximization problem in terms of $\bL$ is a well-defined indefinite LQR that is $\psi_i$-smooth and $p_i$-PL. Also, for any $\bK \in \overline{\cK}$, the Hessian is a polynomial and $\overline{\cK}$ is compact, there exists a uniform upper bound for the Hessian. Combining the above two conditions yields that there exists a constant parameter $L_1$ such that   
%\begin{align*}
%	\|\nabla_{\bK}\cG(\bK', \bL') - \nabla_{\bK}\cG(\bK, \bL)\| \leq L_1 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bK \in \overline{\cK}	
%\end{align*}
%Similarly, we can show that $\overline{\cL}$ is a compact set and for any fixed $\bL \in \overline{\cL}$, the minimization problem in terms of $\bK$ is a well-defined indefinite LQR that is $\psi_j$-smooth and $p_j$-PL. Thus, we can also derive the condition such that there exists a constant parameter $L_2$  that 
%\begin{align*}
%	\|\nabla_{\bL}\cG(\bK', \bL') - \nabla_{\bL}\cG(\bK, \bL)\| \leq L_2 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bL \in \overline{\cL}.
%\end{align*}
%This proves the two-sided smoothness property, similar to Assumption 1 of \cite{yang2020global}, but restricted to the region where $(\bK, \bL) \in  \overline{\cK} \times \overline{\cL}$.  Finally, invoking Lemma A.2 of \cite{yang2020global} yields that the outer loop is $L$-smooth with $L:=\max\{L_1, L_2\} + \frac{\max\{L_1, L_2\}}{\max_i{p_i}}$ for any $\bK \in \overline{\cK}$.
% \begin{lemma}(Lemma A.3 of \cite{nouiehed2019solving})
% 	Assume that $\{\cG(\bK, \bL) \mid \bK \in \cK\}$ is a class of $\Upsilon$-PL functions in $\bL$, where $\Upsilon$ is an absolute constant. Then, if $\bL(\bK) = \argmax_{\bL}\cG(\bK, \bL)$, we have for any $\bK_1, \bK_2 \in \cK$ and their corresponding $\bL(\bK_1), \bL(\bK_2)$, 
% 	\begin{align*}
% 		\|\bK_1 - \bK_2\| \leq \frac{\textcolor{red}{L}}{2\Upsilon}\|\bL(\bK_1) - \bL(\bK_2)\| 
% 	\end{align*}  
% \end{lemma}
%
%\begin{lemma}(Lemma A.5 of \cite{nouiehed2019solving})
%	For $\bK \in \cK$, the outer loop is $\psi_{2}$-smooth.
%\end{lemma}
%Meisam Lemma A.5: outer loop is smooth, for $\bK \in \cK$.
% \end{proof}
% 
% 
% \begin{lemma}(Two-Sided Smoothness)\label{lemma:two_side_smooth}
% There exists a positive constant $l >0$ such that
% \begin{align*}
% 	\|\nabla_{\bK}\cG(\bK', \bL') - \nabla_{\bK}\cG(\bK, \bL)\| \leq l \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \\
% 	\|\nabla_{\bL}\cG(\bK', \bL') - \nabla_{\bL}\cG(\bK, \bL)\| \leq l \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big],
% \end{align*}	
% holds for all pairs of $(\bK, \bL)$ such that $\bK \in \cK$ and $\bL \in \cL$.
%\end{lemma}
%
%\begin{proof}
%First, define the auxiliary sets 
%\begin{align*}
%	\overline{\cK}:= \{\bK \mid \bR^w-\bD^{\top}\bP_{\bK, \bL(\bK)}\bD \geq \zeta\bI\}, \quad \overline{\cL} := \{\bL \mid \bR^u + \bB^{\top}\bP_{\bK(\bL), \bL}\bB \geq \zeta\bI \}, 
%\end{align*}
%where $\bL(\bK) = \argmax_{\bL}\cG(\bK, \bL)$ and $\bK(\bL) = \argmin_{\bK}\cG(\bK, \bL)$ for whenever $\bL(\bK)$ and $\bK(\bL)$ exist and $\zeta>0$ is a small constant such that $\overline{\cK}$ and $\overline{\cL}$ are nonempty. We first claim that $\overline{\cK}$ is a compact set. First, we show that $\overline{\cK}$ is closed. Since $\bP_{\bK, \bL(\bK)}$ is the unique solution of the Riccati equation
%\begin{align*}
%	\bP_{\bK, \bL(\bK)} = \bQ + \bK^{\top}\bR^u\bK - \bL(\bK)^{\top}\bR^w\bL(\bK) +(\bA-\bB\bK-\bD\bL(\bK))^{\top}\bP_{\bK, \bL(\bK)}(\bA-\bB\bK-\bD\bL(\bK))
%\end{align*}
%where the uniqueness is due to the fact that it is actually an iterative linear equation in terms of the blocks. Thus, $\overline{\cK}$ is closed. Then, it remains to show that $\overline{\cK}$ is bounded. Since $\bQ \geq 0, \bR^u, \bR^w > 0$ and $\bL$ is the control gain matrix of the maximizing player, we have $\bQ + \bK^{\top}\bR^u\bK - \bL(\bK)^{\top}\bR^w\bL(\bK) \geq 0$. This leads to $\bP_{\bK, \bL(\bK)} \geq 0$. Moreover, for any $\bK \in \overline{\cK}$,
%\begin{align*}
%	\bD^{\top}\bP_{\bK, \bL(\bK)}\bD \leq \bR^w \Rightarrow \|\bD^{\top}\bP_{\bK, \bL(\bK)}\bD\| \leq \|\bR^w\| \Rightarrow \|\bP_{\bK, \bL(\bK)}\| \leq C
%\end{align*}
%where $C>0$ is a finite absolute constant. This results in the condition that $\sup_{\bK}\|\bK\| < \infty$. Therefore, the set $\overline{\cK}$ is bounded and thus compact. By Lemma \ref{assumption_game}, for any fixed $\bK_i \in \overline{\cK}$, the maximization problem in terms of $\bL$ is a well-defined indefinite LQR that is $\psi_i$-smooth and $p_i$-PL. Also, for any $\bK \in \overline{\cK}$, the Hessian is a polynomial and $\overline{\cK}$ is compact, there exists a uniform upper bound for the Hessian. Combining the above two conditions yields that there exists a constant parameter $L_1$ such that   
%\begin{align*}
%	\|\nabla_{\bK}\cG(\bK', \bL') - \nabla_{\bK}\cG(\bK, \bL)\| \leq L_1 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bK \in \overline{\cK}	
%\end{align*}
%Similarly, we can show that $\overline{\cL}$ is a compact set and for any fixed $\bL \in \overline{\cL}$, the minimization problem in terms of $\bK$ is a well-defined indefinite LQR that is $\psi_j$-smooth and $p_j$-PL. Thus, we can also derive the condition such that there exists a constant parameter $L_2$  that 
%\begin{align*}
%	\|\nabla_{\bL}\cG(\bK', \bL') - \nabla_{\bL}\cG(\bK, \bL)\| \leq L_2 \big[\|\bK'-\bK\| + \|\bL'-\bL\|\big], \forall \bL \in \overline{\cL}.
%\end{align*}
%This proves the two-sided smoothness property, similar to Assumption 1 of \cite{yang2020global}, but restricted to the region where $(\bK, \bL) \in  \overline{\cK} \times \overline{\cL}$.  Finally, invoking Lemma A.2 of \cite{yang2020global} yields that the outer loop is $L$-smooth with $L:=\max\{L_1, L_2\} + \frac{\max\{L_1, L_2\}}{\max_i{p_i}}$ for any $\bK \in \overline{\cK}$.
 
%	We prove the two-sided smoothness property by showing that when fixing either $\bK$ or $\bL$, the cost function of the remaining single-player optimization problem is smooth. That is, there exists constants $l_{\bK}, l_{\bl}$ such that
%	\begin{align}\label{eqn:fixed_L}
%	 	\|\nabla_{\bK}\cG(\bK', \bL) - \nabla_{\bK}\cG(\bK, \bL)\| &\leq l_{\bK} \|\bK'-\bK\|, \\
% 	\|\nabla_{\bL}\cG(\bK, \bL') - \nabla_{\bL}\cG(\bK, \bL)\| &\leq l_{\bL}  \|\bL'-\bL\|, \label{eqn:fixed_K}
%	\end{align}
%	holds for all $\bK$ and $\bL$. If \eqref{eqn:fixed_K} and \eqref{eqn:fixed_L} hold, Lemma \ref{lemma:two_side_smooth} is proved by setting $l = \max(l_{\bK}, l_{\bL})$. Now, we focus on proving \eqref{eqn:fixed_K} and \eqref{eqn:fixed_L}. Notice that for any fixed $\bK$, the maximization problem in terms of $\bL$ is essentially an indefinite LQR with state weighting matrix $-\bQ-\bK^{\top}\bR^u\bK$ and state transition matrix $\bA - \bB\bK$. Similarly, for any fixed $\bL$, the minimization problem in terms of $\bK$ is also an indefinite LQR with state-weighting matrix $\bQ - \bL^{\top}\bR^w\bL$ and state transition matrix $\bA-\bD\bL$. \xznote{expand}Then, we can conclude coerciveness properties and thus compact level sets. This leads to \eqref{eqn:fixed_K} and \eqref{eqn:fixed_L} and thus proves the two-sided smoothness property.


\subsection{Global Convergence}\label{sec:convergence}



 

%	There are a few intuitions behind the initialization process that we would like to point out. Firstly, when initializing with any $\bK_0$,  there exists a finite disturbance attenuation level $\gamma_{\bK_0} > \gamma^*$ associated with the initial controller $\bK_0$. By Lemma \ref{lemma:game-game} and \ref{lemma:game-inf}, we can formulate a corresponding stochastic game parametrized by $\gamma_{\bK_0}$ that is well-defined, in the sense that the upper value of the game is finite. Then, as we shown in Theorem \ref{theorem:ir_K}, this initial disturbance attenuation level is preserved on-the-fly along two PG methods. Finally, Theorem \ref{theorem:Mbased_conv_K} proves that starting with any $\bK_0$, two PG methods converge to the saddle-point policies of the associated game. According to Lemma \ref{lemma:game-game} and \ref{lemma:game-inf}, the saddle point policy of the minimizing player is equivalent to the controller that minimizes the objective \eqref{eqn:ckl} and also attains a the disturbance attenuation level of $\gamma_{\bK_0}$ in the original disturbance attenuation problem. 
%	
%	Further, for any $\tilde{\bK}_0$ that satisfies a prescribed disturbance attenuation level $\gamma_{\tilde{\bK}_0} > \gamma^*$, Theorem \ref{theorem:Mbased_conv_K}, Lemma \ref{lemma:game-game}, and Lemma \ref{lemma:game-inf} demonstrate that two PG methods automatically preserve the a $\gamma_{\tilde{\bK}_0}$-level of disturbance attenuation on-the-fly while converging globally to the saddle point. Lastly, searching for such a feasible initial control gain matrix $\tilde{\bK}_0$ that satisfies $\gamma_{\tilde{\bK}_0} > \gamma^*$ is empirically permissible through a ``robustification'' process without the knowledge of model parameters \cite{zhang2020rarl}. 


==> mixfree.tex <==
\xznote{need perturbation analaysis for K, Pk, L(K), and SigmaK.}
In this section, we analyze the sample complexity of random search algorithms for the outer loop problem. 





\begin{theorem}
	Let the stepsize and smoothing radius to satisfy $\alpha = \cO(M^{-2/3})$ and $r_{\bK} = \cO(M^{-1/6})$ and run the algorithm for $M = \cO(\epsilon_{\bK}^{-3}\Lambda^{-3})$ iterations. Then, the random search algorithm reaches the stationary point, such that $\|\nabla\cG(\bK_{M})\|^2 \leq \epsilon_{\bK}$, with probability greater than $1-\Lambda$. $\epsilon_{\bK} >0$ is the desired accuracy level and $\Lambda \in (0, 1)$.  
\end{theorem}
\begin{proof}
	Following from \cite{nesterov2017random}, the following properties holds for Gaussian-smoothed version of function $\cG(\bK)$, denoted as $\cG_{r_{\bK}}(\bK) := \EE[\cG(\bK+r_{\bK}U)]$,
	\begin{align}
		|\cG_{r_{\bK}}(\bK) - \cG(\bK)| &\leq r_{\bK}^2\psi_{\bK}\tilde{d}_{\bK} \label{eqn:cost_bound}\\
		\|\nabla\cG_{r_{\bK}}(\bK) - \nabla\cG(\bK)\| &\leq r_{\bK}\psi_{\bK}(\tilde{d}_{\bK} + 3)^{3/2} \label{eqn:grad_bound}
	\end{align}
	Also, the noisy gradient estimate $\overline{\nabla}\cG_{r_{\bK}}(\bK)$ satisfies that for all $\bK_k$,
	\begin{align}\label{eqn:unbiased_est}
		\EE~[\overline{\nabla}\cG_{r_{\bK}}(\bK_k)] = \nabla\cG_{r_{\bK}}(\bK_k)
	\end{align}
	where the expectation is taken over both the random process noise $\bm{\xi}$ and the Gaussian smoothing on the control gain matrix, $U$. Let the function $\cG_{r_{\bK}}(\bK, \bm{\xi}) \in C^{1, 1}$ with Lipschitz constant $\psi_{\bK}(\bm{\xi})$, we assume $\psi_{\bK}(\bm{\xi}) \leq \psi_{\bK}$. Then, we have
	\begin{align}
		\EE~[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2] &\leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + \|\nabla\cG_{r_{\bK}}(\bK_k)\|^2\nonumber\\
		&\leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + 2\|\nabla\cG(\bK_k)\|^2 + 2\|\nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\|\nonumber\\
		&\leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + 2\|\nabla\cG(\bK_k)\|^2 + 2r_{\bK}^2\psi_{\bK}^2(\tilde{d}_{\bK}+3)^3. \label{eqn:step2}
	\end{align}
	Following Lemma 1.2.3 of \cite{nesterov2013introductory}, we can obtain the following inequality
	\begin{align*}
		\cG_{r_{\bK}}(\bK_{k+1}) &\leq \cG_{r_{\bK}}(\bK_{k}) + \big\langle\nabla\cG_{r_{\bK}}(\bK_{k}), \bK_{k+1}-\bK_k \big\rangle + \frac{\psi_{\bK}}{2}\|\bK_{k+1} - \bK_k\|^2 \\
		&= \cG_{r_{\bK}}(\bK_{k}) -\alpha\big\langle\nabla\cG_{r_{\bK}}(\bK_{k}), \overline{\nabla}\cG_{r_{\bK}}(\bK_{k}) \big\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2 \\
		&=\cG_{r_{\bK}}(\bK_{k}) -\alpha\big\langle\nabla\cG_{r_{\bK}}(\bK_{k}), \overline{\nabla}\cG_{r_{\bK}}(\bK_{k})-\nabla\cG_{r_{\bK}}(\bK_{k}) \big\rangle -\alpha\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2 + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2
	\end{align*}
	By \eqref{eqn:unbiased_est},  we take expectation on both sides and rearrange terms. This leads to
	\begin{align*}
		\alpha\EE\big[\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big] \leq \EE\big[\cG_{r_{\bK}}(\bK_{k})\big] - \EE\big[\cG_{r_{\bK}}(\bK_{k+1})\big] + \frac{\psi_{\bK}\alpha^2}{2}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big]
	\end{align*}
	Summing the above inequality from 0 to $M-1$ and dividing both sides by $\alpha$ yields
	\begin{align}
		\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big] \leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \EE\big[\cG_{r_{\bK}}(\bK_{M})\big]}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] \nonumber\\
		\leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] \label{eqn:step1}
	\end{align}
	where $\cG_{r_{\bK}}(\bK^*)$ is the lower bound of the smoothed function $\cG_{r_{\bK}}(\bK)$, for which the existence is ensured because of the boundness of the original function $\cG(\bK)$ and \eqref{eqn:cost_bound}. Since
	\begin{align}
		\frac{1}{2}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \EE\big[\|\nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big] + \EE\big[\|\nabla\cG(\bK_{k}) - \nabla\cG_{r_{\bK}}(\bK_{k})\|^2\big],
	\end{align}
	we can combine \eqref{eqn:step1} and \eqref{eqn:grad_bound} to obtain
	\begin{align*}
		\frac{1}{2}\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] + r^2_{\bK}\psi^2_{\bK}(\tilde{d}_{\bK} + 3)^{3}M
	\end{align*}
	Also, from \eqref{eqn:step2}, we can derive 
	\begin{align}
		\sum^{M-1}_{k=0}\EE~[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2]  \leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k))M + 2\|\nabla\cG(\bK_k)\|^2M + 2r_{\bK}^2\psi_{\bK}^2(\tilde{d}_{\bK}+3)^3M.
	\end{align}
	Therefore, 
	\begin{align*}
		&\frac{1}{2}\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} + \frac{\psi_{\bK}\alpha}{2}\sum^{M-1}_{k=0}\EE\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_{k})\|^2\big] + r^2_{\bK}\psi^2_{\bK}(\tilde{d}_{\bK} + 3)^{3}M \\
		&\hspace{1em}\leq \frac{\EE\big[\cG_{r_{\bK}}(\bK_{0})\big] - \cG_{r_{\bK}}(\bK^*)}{\alpha} +\frac{\psi_{\bK}\alpha \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k))M}{2} + \psi_{\bK}\alpha\|\nabla\cG(\bK_0)\|^2M + (\psi_{\bK}\alpha+1)r^2_{\bK}\psi^2_{\bK}(\tilde{d}_{\bK} + 3)^{3}M 
	\end{align*}
	\xzedit{As the variance term can be bounded by 
	\begin{align*}
		\Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) \leq \Big(\frac{1}{r_{\bK}}~\sup_{\bK_k}~ (\overline{\cG}_{r_{\bK}}(\bK_k) + \epsilon_{\bL})\Big)^2
	\end{align*}
	almost surely, we can conclude that $\Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) = \cO(r_{\bK}^{-2}\epsilon_{\bL}^2)$}. Then, let the stepsize and the perturbation radius chosen to satisfy the order of $\alpha = \cO(M^{-2/3})$ and $r_{\bK} = \cO(M^{-1/6})$, we have
 	\begin{align}
 		\sum^{M-1}_{k=0}\EE\big[\|\nabla\cG(\bK_{k})\|^2\big] \leq \cO(M^{2/3}) + \cO(M^{2/3}\xzedit{\epsilon_{\bL}^2}) + \cO(M^{1/3}) + \cO(M^{2/3}) + \cO(1)
 	\end{align}
 	Dividing both sides by $M$, we can observe when $M = \cO(\epsilon_{\bK}^{-3}\Lambda^{-3})$ \xzedit{and $ \epsilon_{\bL} = o( \sqrt{\epsilon_{\bK}\Lambda})$ almost surely}, $\EE\big[\|\nabla\cG(\bK_{M})\|^2\big] \leq \epsilon_{\bK}\Lambda$. Applying Markov's inequality leads to 
 	\begin{align}
 		P\big\{\|\nabla\cG(\bK_{M})\|^2 \geq \epsilon_{\bK}\big\} \leq \frac{1}{\epsilon_{\bK}}\EE\big[\|\nabla\cG(\bK_{M})\|^2\big] \leq \Lambda.
 	\end{align}
 	This implies $P\big\{\|\nabla\cG(\bK_{M})\|^2 \leq \epsilon_{\bK}\big\} > 1-\Lambda$. The proof is completed.
\end{proof}

\xzedit{The total sample complexity scales as $\cO\big(\frac{1}{\epsilon_{\bK}^{3}\epsilon_{\bL}^2\Lambda^{3}\delta^{2}}\log(\frac{1}{\epsilon_{\bL}\delta})\big)$, where $ \epsilon_{\bL} = o( \sqrt{\epsilon_{\bK}\Lambda})$ almost surely.}
%\begin{proof}
%	For a positive smoothing radius $r_{\bK} > 0$, the smoothed function $\cG_{r_{\bK}}(\bK) := \EE[\cG(\bK+U)]$ with $\|U\|_F = r_{\bK}$ and the expectation is taken with respect to the combined randomness. The estimate of the gradient $\overline{\nabla}\cG_{r_{\bK}}$ at the point $\bK$ is given by $\overline{\nabla}\cG_{r_{\bK}}(\bK) = \frac{\tilde{d}_{\bL}}{r^2_{\bK}}\cG(\bK+U; \bm{\xi})U$, where each of the randomness $\{x_0, \xi_0, \dots, \xi_{N-1}\}$ of the system is sampled independently from the distribution $\cD$. Then, \cite{flaxman2005online, agarwal2010optimal, shamir2017optimal, malik2020derivative} suggests the following properties of the gradient estimate $\overline{\nabla}\cG_{r_{\bK}}$.
%	\begin{itemize}
%		\item $\nabla\cG_{r_{\bK}}(\bK) = \EE[\overline{\nabla}\cG_{r_{\bK}}(\bK)]$
%		\item $\|\nabla\cG_{r_{\bK}}(\bK) - \nabla\cG(\bK)\| \leq \psi_{\bK}r_{\bK}$
%%		\item  \quad $\|\nabla\cG_{r_{\bK}}(\bK)\|^2 \leq \|\nabla\cG(\bK)\|^2 +  \psi_{\bK}^2r_{\bK}^2$.
%	\end{itemize}
%	The proof is omitted for simplicity and we refer the readers to Appendix $C$ of \cite{malik2020derivative} for a complete justification. Since the gradient of the outer loop problem is $\psi_{\bK}$-Lipschitz, we have
%	\begin{align*}
%		\cG(\bK_{k+1}) - \cG(\bK_{k}) &\leq \big\langle \nabla\cG(\bK_k), \cG(\bK_{k+1}) - \cG(\bK_k)\big\rangle + \frac{\psi_{\bK}}{2}\|\cG(\bK_{k+1}) - \cG(\bK_k)\|^2 \\
%		&= - \alpha\big\langle \nabla\cG(\bK_k), \nabla\cG_{r_{\bK}}(\bK_k)\big\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2\\
%		&= -\alpha\|\nabla\cG(\bK_k)\|^2 - \alpha \langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2
%	\end{align*}
%	where the first equality follows from the first property above. Rearranging the terms yields
%	\begin{align*}
%		\alpha\|\nabla\cG(\bK_k)\|^2 &\leq \cG(\bK_{k}) - \cG(\bK_{k+1}) - \alpha \langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2
%	\end{align*}
%%	Then, utilizing the assumption of $\cG(\bK^*) \leq \cG(\bK_{k+1})$ leads to 
%%	\begin{align}
%%		\alpha \|\nabla\cG(\bK_k)\|^2 \leq \big(\cG(\bK_{k}) - \cG(\bK^*)\big) - \alpha \langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle + \frac{\psi_{\bK}\alpha^2}{2}\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2
%%	\end{align}
%	Taking expectation of the randomness up to iteration $k$ on both sides yields
%	\small
%	\begin{align*}
%		\alpha \EE_k~\big[\|\nabla\cG(\bK_k)\|^2\big] \leq \cG(\bK_{k}) - \cG(\bK_{k+1}) - \alpha \EE_{k}~\big[\langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle\big] + \frac{\psi_{\bK}\alpha^2}{2}\EE_{k}~\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2\big]
%	\end{align*}
%	\normalsize
%	Also, similar to equation (3.20) of \cite{ghadimi2013stochastic} and the second to last equation on page 23 of \cite{malik2020derivative}, we can observe the following two conditions
%	\begin{align*}
%		&\EE_{k}~\big[\langle \nabla\cG_{r_{\bK}}(\bK_k),  \nabla\cG_{r_{\bK}}(\bK_k) - \nabla\cG(\bK_k)\rangle\big] = 0\\
%		&\EE_{k}~\big[\|\overline{\nabla}\cG_{r_{\bK}}(\bK_k)\|^2\big] = \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + \EE_{k}~\big[\|\nabla\cG_{r_{\bK}}(\bK_k)\|^2\big] \\
%%		&\hspace{2em} \leq \Var(\overline{\nabla}\cG_{r_{\bK}}(\bK_k)) + 2\|\nabla\cG(\bK_k)\|^2 + 2\|\nabla\cG_{r_{\bK}}(\bK_k)- \nabla\cG(\bK_k)\|^2\\
%		&\hspace{2em} \leq G_2 + 2\EE_{k}~\|\nabla\cG(\bK_k)\|^2 + 2(\psi_{\bK}r_{\bK})^2.
%	\end{align*}
%	Therefore, applying the conditions leads to
%	\begin{align*}
%		\alpha \EE_k~\big[\|\nabla\cG(\bK_k)\|^2\big] &\leq \cG(\bK_{k}) - \cG(\bK_{k+1}) + \frac{\psi_{\bK}\alpha^2}{2}\big(G_2 + 2\EE_{k}~\|\nabla\cG(\bK_k)\|^2 + 2(\psi_{\bK}r_{\bK})^2\big) \\
%		(\alpha - \psi_{\bK}\alpha^2)\EE_k~\big[\|\nabla\cG(\bK_k)\|^2\big] & \leq \cG(\bK_{k}) - \cG(\bK_{k+1}) +  \frac{\psi_{\bK}\alpha^2}{2}\big(G_2 + 2(\psi_{\bK}r_{\bK})^2\big)
%	\end{align*}
%	Since $\alpha \leq \frac{1}{2\psi_{\bK}}$, we have $\sum^{\cK}_{k=0}(\alpha - \psi_{\bK}\alpha^2) = \cK\alpha(1-\psi_{\bK}\alpha) \geq \frac{\cK\alpha}{2}$. Then, summing over $\cK$ and dividing both sides by $\sum^{\cK}_{k=0}(\alpha - \psi_{\bK}\alpha^2)$ yields
%	\begin{align*}
%		 (\alpha - \psi_{\bK}\alpha^2)\sum^{\cK}_{k=0}\EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] &\leq \Delta_0  + \frac{\psi_{\bK}\alpha^2}{2}\sum^{\cK}_{k=0}\big(G_2 + 2(\psi_{\bK}r_{\bK})^2\big) \\
%		\Rightarrow \EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] &\leq \frac{2\Delta_0}{\cK\alpha}  + \psi_{\bK}\alpha\big(G_2 + 2(\psi_{\bK}r_{\bK})^2\big)\\
%		 &\leq \frac{2\Delta_0}{\cK\alpha}  + \psi_{\bK}\alpha G_2 + 2\psi^3_{\bK}r_{\bK}^2\alpha\\
%		 &\leq \frac{2\Delta_0}{\cK}\max\big\{2\psi_{\bK}, G_2\psi_{\bK}\sqrt{\cK}\big\}  + \frac{1}{\sqrt{\cK}}  + \frac{1}{\sqrt{\cK}} + \psi^2_{\bK}r_{\bK}^2 
%	\end{align*}
%	where the last inequality follows from the requirements of $\alpha$ in \eqref{eqn:one_point_req_K}. Then, since $r_{\bK} \leq \frac{1}{\psi_{\bK}\sqrt{\cK}}$, 
%	\begin{align*}
%		\frac{2\Delta_0}{\cK}\max\big\{2\psi_{\bK}, G_2\psi_{\bK}\sqrt{\cK}\big\}  + \frac{1}{\sqrt{\cK}} + \psi^2_{\bK}r_{\bK}^2 &\leq \frac{2\Delta_0}{\cK}\big[2\psi_{\bK}+  G_2\psi_{\bK}\sqrt{\cK}\big]  + \frac{1}{\sqrt{\cK}} + \frac{1}{\cK}\\
%		&= \frac{4\Delta_0\psi_{\bK}+1}{\cK} + \frac{G_2\psi_{\bK}}{\sqrt{\cK}} + \frac{1}{\sqrt{\cK}}.
%	\end{align*}
%	Subsequently, we provide a bound for $G_2$. By definition of the estimated cost function, their exists an absolute constant $c_2$ such that \xznote{in two point, G2 is a constant, in one point, G2 is more complicated, and needs to depend on epsilon, thus ck}
% 	\begin{align*}
% 		\cG(\bK + U, \bm{\xi}) = \bm{\xi}^T\bP_{\bK + U}\bm{\xi} \leq s\sigma^2 \EE_{\bm{\xi}} [\bm{\xi}^T\bm{\xi}]~ \|\bP_{\bK + U}\| \leq s\sigma^2c_{2}.
% 	\end{align*}
% 	Therefore, as $\|U\|_F = r_{\bK}$, we can prove the following bound
% 	\begin{align*}
% 		G_{\infty} = \frac{\tilde{d}_{\bK}}{r_{\bK}}~\sup_{\bK+U}~ \overline{\cG} \leq \frac{s\sigma^2\tilde{d}_{\bK}c_{2}}{r_{\bK}}, \quad G_2 \leq G^2_{\infty} \leq \Big(\frac{s\sigma^2\tilde{d}_{\bK}c_{2}}{r_{\bK}}\Big)^2 \leq \Big(\frac{s\sigma^2\tilde{d}_{\bK}c_{2}}{r_{\bK}}\Big)^2
% 	\end{align*}
%	Then, it can be seen that choosing a $\cK$ with the order of $\cO(\epsilon^{2}_{\bK})$. Then, the 
%	 ensures that $\EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] \leq \epsilon_{\bK}\Lambda$. Then, applying Markov's inequality yields 
%	\begin{align}
%		P\big\{\|\nabla\cG(\bK_{\cK})\|^2 \geq \epsilon_{\bK}\big\} \leq \frac{1}{\epsilon_{\bK}}\EE~\big[\|\nabla\cG(\bK_{\cK})\|^2\big] \leq \Lambda.
%	\end{align}
%	This implies $P\big\{\|\nabla\cG(\bK_{\cK})\|^2 \leq \epsilon_{\bK}\big\} > 1-\Lambda$.  	Substitute the bounds into the requirements of $\alpha$ completes the proof of the theorem.
%%	Also, as the cost function of the outer loop problem is smooth, we have
%%	\begin{align}
%%		(\theta_{\bK} - \theta_{\bK}^2\psi_{\bK}/2)\|\nabla\cG(\bK_k)\|^2 \leq \cG(\bK_k) - \cG(\bK_k - \theta_{\bK}\nabla\cG(\bK_k)) \leq \cG(\bK_k) - \cG(\bK^*),
%%	\end{align}
%%	for $\theta_{\bK} = \min\{\frac{1}{2\psi_{\bK}}, \frac{1}{l_{\bK}}\}$. Then, define $\Delta_k := \cG(\bK_k) - \cG(\bK^*)$ to be the optimality gap at iteration $k$. Then, 
%%	\begin{align}
%%	\EE_k[\Delta_{k+1} - \Delta_k] &\leq -\alpha\|\nabla\cG(\bK_k)\|^2 + \frac{2\alpha\psi_{\bK}r_{\bK}}{\theta_{\bK}}\Delta^{1/2}_k + \frac{\psi_{\bK}\alpha^2}{2}G_2 +  \psi_{\bK}\alpha^2\big(\|\nabla\cG(\bK_k)\|^2 + (\psi_{\bK}r_{\bK})^2\big) \\
%%	&\leq -\frac{\alpha}{2}\|\nabla\cG(\bK_k)\|^2+ \frac{2\alpha\psi_{\bK}r_{\bK}}{\theta_{\bK}}\Delta^{1/2}_k + \frac{\psi_{\bK}\alpha^2}{2}G_2 + \alpha^2\psi_{\bK}^3r_{\bK}^2 \\
%%	&\leq -\frac{\alpha}{2}\|\nabla\cG(\bK_k)\|^2+\Delta_k + \frac{\alpha^2\psi^2_{\bK}r_{\bK}^2}{\theta^2_{\bK}} + \frac{\psi_{\bK}\alpha^2}{2}G_2 + \alpha^2\psi_{\bK}^3r_{\bK}^2
%%	\end{align}
%%	\xznote{alsdhfliashdgfashdfoah}
%%	where the second inequality follows from $\alpha \leq \frac{1}{2\psi_{\bK}}$ and the last inequality follows from the inequality $2ab \leq a^2+b^2$ for any pair of $(a, b)$. 
%\end{proof}
